Teacher Demonstrations in a BabyLM's Zone of Proximal Development for Contingent Multi-Turn Interaction

Multi-turn dialogues between a child and a caregiver are characterized by a property called contingency - that is, prompt, direct, and meaningful exchanges between interlocutors. We introduce ContingentChat, a teacher-student framework that benchmarks and improves multi-turn contingency in a BabyLM trained on 100M words. Using a novel alignment dataset for post-training, BabyLM generates responses that are more grammatical and cohesive. Experiments with adaptive teacher decoding strategies show limited additional gains. ContingentChat demonstrates the benefits of targeted post-training for dialogue quality and indicates that contingency remains a challenging goal for BabyLMs.

==> _CONTRIBUTING <==
Simple guideline to give the paper consistency (WITH THANKS TO PIETRO LESCI FOR THIS STYLE GUIDE):
- Use British English

- When using number use \integer{}, \float[num_digits]{}, or \q{}{unit} as macros. For example, \integer{1}, \float[2][0.22], or \q{100}{\thousand}

- In the bib file (IMPORTANT FOR REFERENCE CONSISTENCY):

    - use `zhai2022scaling` or `zhai-etal-2022-scaling` kind of keys so it's easier to cite.
    
    - In titles, upper case after ":", e.g. "Some things: {O}ther things"
 
    - For arxiv papers, use the article class and in the journal entry use the format `journal = {arXiv preprint 2404.06395}`

- Instead of \texttt{} , use \myemph{}

- Let's define and use macros for common stuff we might change later, e.g., \bpe. Look at macros at the bottom of the preamble.tex file

- Use \enquote{} for quotations instead of manually using ``''

- Format links without the "http" prefix and formatting using \myemph for helvetica, e.g., `\href{https://github.com/huggingface/tokenisers}{\myemph{github.com/huggingface/tokenisers}}`

==> _scratchpad.tex <==


\section{Background and Motivation}

\subsection{Interactive Language Learning}

NeLLCom-X  \cite{lian-etal-2024-nellcom} 

\subsection{Pedagogically-Inspired Heuristics for Feedback}
Some possibilities include: minimal Edits and Corrections (v rewording). 

What are the textual signals for teacher intervention? For e.g., grammatical mistakes, questions. We could generate synthetic data based on these signals.

Non-textual signals (e.g., pause, hesitation): consider multi-modal setting. Need to differentiate English as an L1 vs L2. Datlog dataset (originally recordings that were then transcribed).

\subsubsection{Teaching Through Interactions (TTI)}

\textit{Quoting \citet{downer_measuring_2015}'s work below.}

The Teaching Through Interactions (TTI; \citeauthor{hamre_learning_2007}, \citeyear{hamre_learning_2007}) framework conceptualises classroom interactions as representing
these three broad, interrelated domains:
\begin{enumerate}
    \item \textbf{Emotional Support}, which is subdivided into three dimensions: Positive Climate, Teacher Sensitivity, and Regard for Student Perspectives.
    \item\textbf{Classroom Organisation}, which is subdivided into three dimensions: Negative Climate (the absence of), Productivity, and Behaviour Management. This domain draws from previous study and theory regarding the importance of \textbf{self-regulation and executive functioning} in promoting students' learning and achievement, and the role that \textbf{clear and consistent routines} play in the development of these skills.
    \item \textbf{Instructional Support}, which consists of five dimensions: Instructional Learning Formats, Content Understanding, Analysis and Problem Solving, Quality of Feedback, and Instructional Dialogue. Extant research has shown that providing children with opportunities to express existing knowledge and \textbf{scaffolded support} in learning new skills, providing \textbf{immediate and specific feedback} \citep{kulik_timing_1988}, and \textbf{linking new information to existing knowledge and real-world examples} all support cognitive and/or language development.
\end{enumerate}


Of these \#3 is probably the most appropriate for our use:
\begin{itemize}
    \item \textbf{feedback timing} \citep{kulik_timing_1988}: immediate feedback was found to be more effective than delayed feedback in enhancing long-term retention, and research by ``\citet{moreno_decreasing_2004} [...] indicates that feedback providing the correct answer or more detailed information tends to be more effective than merely indicating whether an answer is right or wrong '' \citep{aljabri_timing_2024}. \citet{mingzhe_relationship_2023} identified five types: verification feedback, directive feedback, scaffolding feedback, teacher praise, and teacher criticism. 
\end{itemize}



\section{Interactive Zone of Proximal Development}

We build on the trial and demonstration framework of \citet{ma2024babysit}, specifically aiming to introduce techniques that simulate a student BabyLM's Zone of Proximal Development (ZPD).  

\textit{Interactive Learning (Trial-and-Demonstration): The student model generates a response based on a partial input. A reward function evaluates the generated response. The teacher model provides an expert demonstration. Both responses (student and teacher) are used for policy optimization, refining the student's learning process.
}       

Research Question 1: \textbf{What are the benefits of combining Trial-and-Demonstration Interaction with ZPD-based Curriculum Learning to control how BabyLMs benefit from demonstrations?}



Research Question 2: 

Take a set of queries given some demonstrations to identify optimal demonstrations: IMPROVE, NOT IMPROVE (Retrieve and Rank, Greedy Scoring) --> IRT for ICL-assisted prompting via adding a skill vector for ICL and ICL discrimination vector. 

\section{Pre-training and Post-Training Distribution}

\section{Methods}

\subsection{BabyLM Architecture}

Knowledge Distillation

\textbf{Baseline:} BabyLlama-2, a 345M parameter model distilled from two teachers \cite{tastet-timiryasov-2024-babyllama}. 

Advantage-Guided Distillation for Preference Alignment (ADPA), which leverages an advantage function from the aligned teacher to deliver more nuanced, distribution-level reward signals for the student's alignment \cite{gao2025advantage}.  This uses a Dual-Constrained Knowledge Distillation (DCKD) employs knowledge distillation with two KL-divergence constraints from the aligned teacher to the unaligned student. \footnote{Implementation available here: \url{https://github.com/SLIT-AI/ADPA/tree/main/alignment}}


\subsection{Reward Function}

Token-Level Reward Functions – note from Zheng, these are very noisy and may not actually improve performance.  


==> tables/llama_age_metrics_reduced.tex <==
\begin{table*}[t]
\centering
\footnotesize
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lccccccc}
\toprule
\textbf{Age} & \makecell{\textbf{Student\_Teacher} \\ \textbf{Turn}} & \textbf{AoA} & \textbf{CEFR} & \textbf{TTR} & \textbf{Rep.} & \textbf{Overlap} & \textbf{Norm. Avg} \\ \midrule
6-11months & 1 & 5.080 & 1.390 & 0.483 & 0.844 & 0.201 & 0.664 \\
6-11months & 3 & 5.008 & 1.381 & 0.232 & 0.837 & 0.250 & 0.562 \\
6-11months & 5 & 4.940 & 1.381 & 0.163 & 0.815 & 0.286 & 0.523 \\
6-11months & all & 4.860 & 1.354 & 0.107 & 0.849 & 0.324 & 0.523 \\
\midrule
18-23months & 1 & 4.734 & 1.296 & 0.454 & 0.659 & 0.307 & 0.440 \\
18-23months & 3 & 4.689 & 1.277 & 0.234 & 0.698 & 0.330 & 0.373 \\
18-23months & 5 & 4.689 & 1.272 & 0.164 & 0.732 & 0.352 & 0.383 \\
18-23months & all & 4.609 & 1.241 & 0.099 & 0.766 & 0.411 & 0.391 \\
\midrule
2-3years & 1 & 4.534 & 1.209 & 0.554 & 0.674 & 0.112 & 0.277 \\
2-3years & 3 & 4.460 & 1.197 & 0.330 & 0.734 & 0.178 & 0.255 \\
2-3years & 5 & 4.428 & 1.192 & 0.246 & 0.776 & 0.202 & 0.261 \\
2-3years & all & 4.390 & 1.159 & 0.150 & 0.833 & 0.240 & 0.269 \\
\midrule
3-4years & 1 & 5.446 & 1.500 & 0.539 & 0.818 & 0.182 & 0.787 \\
3-4years & 3 & 5.348 & 1.485 & 0.297 & 0.821 & 0.251 & 0.702 \\
3-4years & 5 & 5.357 & 1.493 & 0.211 & 0.838 & 0.296 & 0.716 \\
3-4years & all & 5.270 & 1.449 & 0.114 & 0.878 & 0.360 & 0.708 \\
\midrule
4-5years & 1 & 4.943 & 1.350 & 0.443 & 0.650 & 0.260 & 0.466 \\
4-5years & 3 & 4.880 & 1.315 & 0.295 & 0.878 & 0.203 & 0.531 \\
4-5years & 5 & 4.842 & 1.306 & 0.223 & 0.869 & 0.183 & 0.465 \\
4-5years & all & 4.778 & 1.280 & 0.146 & 0.858 & 0.191 & 0.399 \\
\bottomrule
\end{tabular*}
\caption{Average metrics by age and number of turns between student and teachers (turns ordered as 1, 3, 5, all). Normalized average uses min–max normalization across all outputs per metric.}
\label{tab:age-segment-metrics-reduced}
\end{table*}


==> tables/main-table-v3.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lrrrrrrrrr}
\toprule
\textbf{BabyLM} & \textbf{Turns} & \textbf{Length} & \textbf{AoA} & \textbf{CEFR} & \textbf{Overlap} & \textbf{TTR} & \textbf{Rep.} & \textbf{NumCon} & \textbf{NormAvg} \\
\midrule
Talking-Babies-cpo\_opt\_100M\_2048\_preprocess & 4 & 50 & 5.087 & 1.373 & 0.068 & 0.620 & 0.851 & 13.300 & 0.503 \\
Talking-Babies-cpo\_opt\_base & 4 & 50 & 5.214 & 1.468 & 0.074 & 0.590 & 0.881 & 13.100 & 0.556 \\
Talking-Babies-cpo\_opt\_cosmos & 4 & 50 & 5.067 & 1.383 & 0.052 & 0.638 & 0.912 & 14.200 & 0.530 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 50 & 5.011 & 1.408 & 0.044 & 0.624 & 0.946 & 15.600 & 0.536 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 4 & 50 & 4.813 & 1.325 & 0.044 & 0.627 & 0.803 & 16.100 & 0.402 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 4 & 50 & 4.802 & 1.371 & 0.053 & 0.610 & 0.870 & 16.500 & 0.460 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 4 & 50 & 4.782 & 1.305 & 0.082 & 0.606 & 0.904 & 13.600 & 0.497 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 4 & 50 & 4.951 & 1.328 & 0.062 & 0.599 & 0.887 & 13.400 & 0.485 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 4 & 50 & 4.819 & 1.328 & 0.056 & 0.572 & 0.909 & 13.800 & 0.467 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 4 & 50 & 4.948 & 1.331 & 0.062 & 0.620 & 0.942 & 14.400 & 0.529 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 4 & 50 & 4.929 & 1.322 & 0.063 & 0.596 & 0.867 & 15.000 & 0.469 \\
Talking-Babies-cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 50 & 4.523 & 1.219 & 0.046 & 0.464 & 0.797 & 18.100 & 0.286 \\
Talking-Babies-mamba-sam-seqlen-2048-original & 4 & 50 & 4.770 & 1.353 & 0.048 & 0.609 & 0.945 & 15.700 & 0.494 \\
Talking-Babies-opt-sam-orpo-mamba-2048-step448 & 4 & 50 & 4.887 & 1.376 & 0.072 & 0.617 & 0.918 & 16.800 & 0.529 \\
Talking-Babies-opt-sam-orpo-seqlen-2048-step559 & 4 & 50 & 4.948 & 1.365 & 0.052 & 0.615 & 0.866 & 15.100 & 0.474 \\
Talking-Babies-opt-sam-seqlen-2048-original & 4 & 50 & 4.843 & 1.318 & 0.052 & 0.618 & 0.942 & 17.000 & 0.503 \\
Talking-Babies-orpo\_opt\_100M\_2048\_preprocess & 4 & 50 & 5.123 & 1.415 & 0.078 & 0.582 & 0.777 & 14.300 & 0.467 \\
Talking-Babies-orpo\_opt\_cosmos & 4 & 50 & 5.200 & 1.459 & 0.067 & 0.624 & 0.822 & 10.300 & 0.514 \\
Talking-Babies-orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 50 & 4.813 & 1.343 & 0.066 & 0.604 & 0.898 & 17.900 & 0.488 \\
Talking-Babies-orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 50 & 4.487 & 1.228 & 0.075 & 0.473 & 0.879 & 11.500 & 0.371 \\
babylm-seqlen-opt-1024-warmup-v2 & 4 & 50 & 4.864 & 1.343 & 0.057 & 0.594 & 0.925 & 16.500 & 0.496 \\
babylm-seqlen-opt-4096-warmup-v2 & 4 & 50 & 4.487 & 1.172 & 0.030 & 0.449 & 0.867 & 17.100 & 0.291 \\
Talking-Babies-cpo\_opt\_100M\_2048\_preprocess & 4 & 100 & 5.028 & 1.417 & 0.121 & 0.508 & 0.931 & 23.400 & 0.590 \\
Talking-Babies-cpo\_opt\_base & 4 & 100 & 5.075 & 1.404 & 0.088 & 0.496 & 0.847 & 21.000 & 0.491 \\
Talking-Babies-cpo\_opt\_cosmos & 4 & 100 & 5.196 & 1.458 & 0.075 & 0.540 & 0.876 & 25.100 & 0.540 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 100 & 4.921 & 1.353 & 0.062 & 0.537 & 0.955 & 35.900 & 0.524 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 4 & 100 & 4.974 & 1.391 & 0.069 & 0.548 & 0.879 & 29.800 & 0.498 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 4 & 100 & 4.888 & 1.374 & 0.082 & 0.523 & 0.817 & 31.700 & 0.453 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 4 & 100 & 4.900 & 1.365 & 0.083 & 0.522 & 0.903 & 33.600 & 0.511 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 4 & 100 & 4.934 & 1.350 & 0.045 & 0.526 & 0.906 & 26.400 & 0.463 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 4 & 100 & 4.984 & 1.395 & 0.063 & 0.524 & 0.905 & 25.700 & 0.499 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 4 & 100 & 4.954 & 1.367 & 0.076 & 0.513 & 0.844 & 21.900 & 0.458 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 4 & 100 & 4.847 & 1.353 & 0.092 & 0.513 & 0.884 & 27.400 & 0.492 \\
Talking-Babies-cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 100 & 4.532 & 1.224 & 0.058 & 0.391 & 0.891 & 33.300 & 0.349 \\
Talking-Babies-mamba-sam-seqlen-2048-original & 4 & 100 & 4.770 & 1.406 & 0.118 & 0.501 & 0.956 & 40.900 & 0.578 \\
Talking-Babies-opt-sam-orpo-mamba-2048-step448 & 4 & 100 & 4.797 & 1.390 & 0.099 & 0.514 & 0.799 & 42.100 & 0.458 \\
Talking-Babies-opt-sam-orpo-seqlen-2048-step559 & 4 & 100 & 4.728 & 1.304 & 0.077 & 0.512 & 0.893 & 40.100 & 0.463 \\
Talking-Babies-opt-sam-seqlen-2048-original & 4 & 100 & 4.917 & 1.439 & 0.089 & 0.523 & 0.904 & 35.500 & 0.538 \\
Talking-Babies-orpo\_opt\_100M\_2048\_preprocess & 4 & 100 & 5.021 & 1.419 & 0.085 & 0.524 & 0.862 & 20.300 & 0.503 \\
Talking-Babies-orpo\_opt\_cosmos & 4 & 100 & 5.211 & 1.443 & 0.091 & 0.532 & 0.866 & 26.100 & 0.549 \\
Talking-Babies-orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 100 & 4.953 & 1.365 & 0.068 & 0.534 & 0.909 & 35.200 & 0.507 \\
Talking-Babies-orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 100 & 4.711 & 1.262 & 0.062 & 0.419 & 0.870 & 19.600 & 0.371 \\
babylm-seqlen-opt-1024-warmup-v2 & 4 & 100 & 4.878 & 1.342 & 0.110 & 0.493 & 0.847 & 38.800 & 0.492 \\
babylm-seqlen-opt-4096-warmup-v2 & 4 & 100 & 4.378 & 1.189 & 0.067 & 0.341 & 0.770 & 35.000 & 0.238 \\
Talking-Babies-cpo\_opt\_100M\_2048\_preprocess & 4 & 150 & 5.057 & 1.441 & 0.115 & 0.469 & 0.828 & 33.400 & 0.518 \\
Talking-Babies-cpo\_opt\_base & 4 & 150 & 5.153 & 1.433 & 0.082 & 0.458 & 0.883 & 34.500 & 0.519 \\
Talking-Babies-cpo\_opt\_cosmos & 4 & 150 & 5.174 & 1.460 & 0.076 & 0.488 & 0.894 & 33.800 & 0.539 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 150 & 4.912 & 1.360 & 0.104 & 0.445 & 0.959 & 52.600 & 0.560 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 4 & 150 & 4.893 & 1.360 & 0.092 & 0.469 & 0.896 & 43.200 & 0.502 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 4 & 150 & 4.923 & 1.418 & 0.105 & 0.467 & 0.936 & 45.100 & 0.562 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 4 & 150 & 4.949 & 1.353 & 0.109 & 0.439 & 0.901 & 40.200 & 0.519 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 4 & 150 & 5.055 & 1.350 & 0.083 & 0.448 & 0.889 & 33.300 & 0.490 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 4 & 150 & 4.989 & 1.379 & 0.114 & 0.443 & 0.870 & 34.600 & 0.514 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 4 & 150 & 4.983 & 1.375 & 0.081 & 0.499 & 0.894 & 35.000 & 0.507 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 4 & 150 & 4.901 & 1.380 & 0.070 & 0.470 & 0.862 & 40.900 & 0.457 \\
Talking-Babies-cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 150 & 4.385 & 1.256 & 0.128 & 0.302 & 0.749 & 49.200 & 0.311 \\
Talking-Babies-mamba-sam-seqlen-2048-original & 4 & 150 & 4.918 & 1.435 & 0.075 & 0.470 & 0.906 & 55.800 & 0.516 \\
Talking-Babies-opt-sam-orpo-mamba-2048-step448 & 4 & 150 & 4.880 & 1.384 & 0.073 & 0.470 & 0.870 & 64.800 & 0.481 \\
Talking-Babies-opt-sam-orpo-seqlen-2048-step559 & 4 & 150 & 4.910 & 1.371 & 0.069 & 0.473 & 0.921 & 47.300 & 0.500 \\
Talking-Babies-opt-sam-seqlen-2048-original & 4 & 150 & 4.998 & 1.416 & 0.117 & 0.466 & 0.913 & 45.500 & 0.570 \\
Talking-Babies-orpo\_opt\_100M\_2048\_preprocess & 4 & 150 & 5.169 & 1.432 & 0.109 & 0.473 & 0.766 & 33.300 & 0.483 \\
Talking-Babies-orpo\_opt\_cosmos & 4 & 150 & 5.284 & 1.489 & 0.102 & 0.507 & 0.847 & 27.000 & 0.561 \\
Talking-Babies-orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 150 & 5.077 & 1.395 & 0.076 & 0.474 & 0.825 & 69.600 & 0.487 \\
Talking-Babies-orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 150 & 4.732 & 1.301 & 0.078 & 0.391 & 0.855 & 37.700 & 0.395 \\
babylm-seqlen-opt-1024-warmup-v2 & 4 & 150 & 4.778 & 1.351 & 0.098 & 0.441 & 0.903 & 55.800 & 0.497 \\
babylm-seqlen-opt-4096-warmup-v2 & 4 & 150 & 4.473 & 1.222 & 0.032 & 0.355 & 0.900 & 50.300 & 0.316 \\
Talking-Babies-cpo\_opt\_100M\_2048\_preprocess & 4 & 200 & 5.171 & 0.932 & 0.108 & 0.432 & 0.904 & 40.300 & 0.453 \\
Talking-Babies-cpo\_opt\_base & 4 & 200 & 5.378 & 1.506 & 0.099 & 0.433 & 0.882 & 41.500 & 0.580 \\
Talking-Babies-cpo\_opt\_cosmos & 4 & 200 & 5.191 & 1.270 & 0.130 & 0.435 & 0.933 & 50.800 & 0.585 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 200 & 4.960 & 1.394 & 0.105 & 0.427 & 0.891 & 67.500 & 0.533 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 4 & 200 & 4.827 & 1.345 & 0.113 & 0.430 & 0.946 & 59.900 & 0.547 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 4 & 200 & 4.952 & 1.391 & 0.061 & 0.419 & 0.874 & 58.100 & 0.457 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 4 & 200 & 5.184 & 1.474 & 0.115 & 0.434 & 0.873 & 60.400 & 0.576 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 4 & 200 & 4.899 & 1.337 & 0.071 & 0.469 & 0.872 & 44.300 & 0.458 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 4 & 200 & 5.025 & 1.387 & 0.093 & 0.441 & 0.904 & 50.500 & 0.527 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 4 & 200 & 5.006 & 1.444 & 0.068 & 0.454 & 0.887 & 43.300 & 0.494 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 4 & 200 & 5.163 & 1.257 & 0.083 & 0.453 & 0.875 & 50.100 & 0.488 \\
Talking-Babies-cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 200 & 4.367 & 1.188 & 0.082 & 0.245 & 0.770 & 102.700 & 0.269 \\
Talking-Babies-mamba-sam-seqlen-2048-original & 4 & 200 & 4.967 & 1.547 & 0.108 & 0.430 & 0.819 & 73.800 & 0.529 \\
Talking-Babies-opt-sam-orpo-mamba-2048-step448 & 4 & 200 & 5.049 & 1.435 & 0.095 & 0.438 & 0.853 & 76.100 & 0.525 \\
Talking-Babies-opt-sam-orpo-seqlen-2048-step559 & 4 & 200 & 4.825 & 1.152 & 0.090 & 0.456 & 0.829 & 62.500 & 0.410 \\
Talking-Babies-opt-sam-seqlen-2048-original & 4 & 200 & 4.947 & 1.384 & 0.073 & 0.456 & 0.841 & 59.800 & 0.462 \\
Talking-Babies-orpo\_opt\_100M\_2048\_preprocess & 4 & 200 & 5.080 & 1.198 & 0.100 & 0.463 & 0.928 & 39.000 & 0.516 \\
Talking-Babies-orpo\_opt\_cosmos & 4 & 200 & 5.417 & 1.546 & 0.074 & 0.478 & 0.854 & 43.100 & 0.562 \\
Talking-Babies-orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 200 & 5.047 & 0.888 & 0.094 & 0.438 & 0.948 & 71.000 & 0.463 \\
Talking-Babies-orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 200 & 4.533 & 1.340 & 0.122 & 0.306 & 0.808 & 65.100 & 0.391 \\
babylm-seqlen-opt-1024-warmup-v2 & 4 & 200 & 5.010 & 1.410 & 0.072 & 0.436 & 0.952 & 75.800 & 0.550 \\
babylm-seqlen-opt-4096-warmup-v2 & 4 & 200 & 4.418 & 1.164 & 0.042 & 0.268 & 0.750 & 70.400 & 0.193 \\
Talking-Babies-cpo\_opt\_100M\_2048\_preprocess & 4 & 250 & 5.054 & 1.393 & 0.125 & 0.396 & 0.950 & 57.700 & 0.590 \\
Talking-Babies-cpo\_opt\_base & 4 & 250 & 5.655 & 1.647 & 0.108 & 0.411 & 0.835 & 47.300 & 0.622 \\
Talking-Babies-cpo\_opt\_cosmos & 4 & 250 & 5.124 & 1.435 & 0.104 & 0.419 & 0.855 & 61.500 & 0.531 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 250 & 4.932 & 1.391 & 0.103 & 0.411 & 0.819 & 80.200 & 0.482 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 4 & 250 & 5.149 & 1.467 & 0.104 & 0.399 & 0.910 & 60.400 & 0.569 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 4 & 250 & 4.927 & 1.378 & 0.099 & 0.396 & 0.840 & 55.800 & 0.465 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 4 & 250 & 4.898 & 1.375 & 0.140 & 0.409 & 0.805 & 60.800 & 0.497 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 4 & 250 & 5.029 & 1.427 & 0.092 & 0.387 & 0.887 & 66.900 & 0.516 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 4 & 250 & 5.183 & 1.434 & 0.095 & 0.419 & 0.838 & 59.000 & 0.514 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 4 & 250 & 5.007 & 1.391 & 0.101 & 0.409 & 0.839 & 48.600 & 0.480 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 4 & 250 & 5.016 & 0.910 & 0.155 & 0.370 & 0.911 & 68.100 & 0.489 \\
Talking-Babies-cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 250 & 4.632 & 1.245 & 0.094 & 0.286 & 0.891 & 78.300 & 0.405 \\
Talking-Babies-mamba-sam-seqlen-2048-original & 4 & 250 & 4.836 & 1.413 & 0.100 & 0.411 & 0.869 & 100.300 & 0.519 \\
Talking-Babies-opt-sam-orpo-mamba-2048-step448 & 4 & 250 & 4.777 & 1.140 & 0.126 & 0.388 & 0.778 & 108.300 & 0.421 \\
Talking-Babies-opt-sam-orpo-seqlen-2048-step559 & 4 & 250 & 5.091 & 1.454 & 0.092 & 0.407 & 0.861 & 67.500 & 0.520 \\
Talking-Babies-opt-sam-seqlen-2048-original & 4 & 250 & 4.997 & 1.439 & 0.116 & 0.401 & 0.907 & 71.200 & 0.565 \\
Talking-Babies-orpo\_opt\_100M\_2048\_preprocess & 4 & 250 & 5.160 & 1.247 & 0.101 & 0.424 & 0.897 & 47.700 & 0.510 \\
Talking-Babies-orpo\_opt\_cosmos & 4 & 250 & 5.386 & 1.497 & 0.120 & 0.436 & 0.844 & 47.600 & 0.585 \\
Talking-Babies-orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 250 & 5.073 & 1.197 & 0.096 & 0.412 & 0.888 & 90.700 & 0.502 \\
Talking-Babies-orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 250 & 4.741 & 1.391 & 0.117 & 0.318 & 0.810 & 49.500 & 0.416 \\
babylm-seqlen-opt-1024-warmup-v2 & 4 & 250 & 4.977 & 1.426 & 0.077 & 0.429 & 0.905 & 71.000 & 0.520 \\
babylm-seqlen-opt-4096-warmup-v2 & 4 & 250 & 4.549 & 1.223 & 0.070 & 0.266 & 0.922 & 79.400 & 0.374 \\
Talking-Babies-cpo\_opt\_100M\_2048\_preprocess & 6 & 50 & 5.071 & 1.423 & 0.065 & 0.564 & 0.830 & 19.000 & 0.479 \\
Talking-Babies-cpo\_opt\_base & 6 & 50 & 5.022 & 1.355 & 0.057 & 0.549 & 0.891 & 18.400 & 0.483 \\
Talking-Babies-cpo\_opt\_cosmos & 6 & 50 & 5.123 & 1.457 & 0.049 & 0.560 & 0.912 & 20.300 & 0.526 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 50 & 4.947 & 1.405 & 0.050 & 0.563 & 0.911 & 25.900 & 0.498 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 6 & 50 & 4.898 & 1.350 & 0.050 & 0.554 & 0.915 & 23.400 & 0.478 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 6 & 50 & 4.812 & 1.341 & 0.067 & 0.543 & 0.922 & 25.200 & 0.488 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 6 & 50 & 4.812 & 1.337 & 0.083 & 0.531 & 0.893 & 20.300 & 0.481 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 6 & 50 & 4.882 & 1.339 & 0.057 & 0.536 & 0.938 & 22.700 & 0.491 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 6 & 50 & 4.886 & 1.333 & 0.064 & 0.528 & 0.929 & 22.600 & 0.490 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 6 & 50 & 4.846 & 1.331 & 0.036 & 0.557 & 0.916 & 21.300 & 0.450 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 6 & 50 & 4.982 & 1.373 & 0.069 & 0.541 & 0.853 & 23.000 & 0.471 \\
Talking-Babies-cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 50 & 4.525 & 1.231 & 0.094 & 0.411 & 0.921 & 22.500 & 0.414 \\
Talking-Babies-mamba-sam-seqlen-2048-original & 6 & 50 & 4.881 & 1.325 & 0.059 & 0.558 & 0.969 & 29.200 & 0.522 \\
Talking-Babies-opt-sam-orpo-mamba-2048-step448 & 6 & 50 & 4.831 & 1.369 & 0.084 & 0.553 & 0.912 & 24.200 & 0.514 \\
Talking-Babies-opt-sam-orpo-seqlen-2048-step559 & 6 & 50 & 5.072 & 1.382 & 0.055 & 0.576 & 0.868 & 25.400 & 0.491 \\
Talking-Babies-opt-sam-seqlen-2048-original & 6 & 50 & 4.858 & 1.323 & 0.052 & 0.551 & 0.932 & 24.500 & 0.481 \\
Talking-Babies-orpo\_opt\_100M\_2048\_preprocess & 6 & 50 & 5.145 & 1.411 & 0.082 & 0.546 & 0.865 & 18.400 & 0.522 \\
Talking-Babies-orpo\_opt\_cosmos & 6 & 50 & 5.375 & 1.514 & 0.055 & 0.564 & 0.858 & 17.600 & 0.541 \\
Talking-Babies-orpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 50 & 4.951 & 1.390 & 0.065 & 0.567 & 0.927 & 26.100 & 0.526 \\
Talking-Babies-orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 50 & 4.612 & 1.234 & 0.061 & 0.419 & 0.907 & 19.000 & 0.376 \\
babylm-seqlen-opt-1024-warmup-v2 & 6 & 50 & 4.864 & 1.339 & 0.038 & 0.543 & 0.901 & 25.300 & 0.446 \\
babylm-seqlen-opt-4096-warmup-v2 & 6 & 50 & 4.478 & 1.197 & 0.029 & 0.408 & 0.803 & 22.100 & 0.242 \\
Talking-Babies-cpo\_opt\_100M\_2048\_preprocess & 6 & 100 & 5.093 & 1.437 & 0.090 & 0.483 & 0.858 & 36.100 & 0.517 \\
Talking-Babies-cpo\_opt\_base & 6 & 100 & 5.035 & 1.429 & 0.080 & 0.489 & 0.892 & 38.500 & 0.521 \\
Talking-Babies-cpo\_opt\_cosmos & 6 & 100 & 5.075 & 1.395 & 0.116 & 0.465 & 0.904 & 43.300 & 0.566 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 100 & 4.904 & 1.364 & 0.094 & 0.456 & 0.932 & 55.000 & 0.535 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 6 & 100 & 4.843 & 1.325 & 0.099 & 0.453 & 0.901 & 51.400 & 0.501 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 6 & 100 & 4.805 & 1.323 & 0.092 & 0.460 & 0.892 & 49.000 & 0.482 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 6 & 100 & 4.916 & 1.107 & 0.112 & 0.465 & 0.876 & 42.900 & 0.461 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 6 & 100 & 4.943 & 1.127 & 0.078 & 0.486 & 0.888 & 40.100 & 0.439 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 6 & 100 & 4.845 & 1.366 & 0.095 & 0.469 & 0.912 & 45.600 & 0.514 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 6 & 100 & 4.953 & 1.363 & 0.068 & 0.469 & 0.915 & 44.500 & 0.495 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 6 & 100 & 4.974 & 1.394 & 0.075 & 0.483 & 0.858 & 42.800 & 0.478 \\
Talking-Babies-cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 100 & 4.430 & 1.320 & 0.129 & 0.299 & 0.764 & 55.700 & 0.346 \\
Talking-Babies-mamba-sam-seqlen-2048-original & 6 & 100 & 4.838 & 1.429 & 0.105 & 0.474 & 0.840 & 59.100 & 0.503 \\
Talking-Babies-opt-sam-orpo-mamba-2048-step448 & 6 & 100 & 4.959 & 1.411 & 0.066 & 0.478 & 0.962 & 60.700 & 0.549 \\
Talking-Babies-opt-sam-orpo-seqlen-2048-step559 & 6 & 100 & 4.912 & 1.352 & 0.080 & 0.508 & 0.944 & 44.600 & 0.535 \\
Talking-Babies-opt-sam-seqlen-2048-original & 6 & 100 & 4.861 & 1.384 & 0.071 & 0.465 & 0.838 & 52.600 & 0.446 \\
Talking-Babies-orpo\_opt\_100M\_2048\_preprocess & 6 & 100 & 4.984 & 1.399 & 0.093 & 0.479 & 0.853 & 41.800 & 0.498 \\
Talking-Babies-orpo\_opt\_cosmos & 6 & 100 & 5.155 & 1.512 & 0.111 & 0.509 & 0.917 & 38.800 & 0.616 \\
Talking-Babies-orpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 100 & 4.965 & 1.382 & 0.069 & 0.467 & 0.888 & 57.200 & 0.492 \\
Talking-Babies-orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 100 & 4.626 & 1.274 & 0.060 & 0.362 & 0.937 & 34.500 & 0.396 \\
babylm-seqlen-opt-1024-warmup-v2 & 6 & 100 & 4.895 & 1.365 & 0.080 & 0.467 & 0.955 & 55.600 & 0.536 \\
babylm-seqlen-opt-4096-warmup-v2 & 6 & 100 & 4.709 & 1.256 & 0.049 & 0.317 & 0.842 & 48.900 & 0.320 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 150 & 5.236 & 1.493 & 0.075 & 0.460 & 0.954 & 75.800 & 0.610 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 6 & 150 & 4.859 & 1.371 & 0.090 & 0.414 & 0.912 & 76.200 & 0.513 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 6 & 150 & 5.048 & 1.427 & 0.088 & 0.438 & 0.918 & 60.700 & 0.547 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 6 & 150 & 5.091 & 0.960 & 0.086 & 0.420 & 0.897 & 62.100 & 0.428 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 6 & 150 & 5.128 & 1.419 & 0.088 & 0.420 & 0.870 & 71.100 & 0.525 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 6 & 150 & 5.011 & 1.397 & 0.092 & 0.429 & 0.902 & 67.300 & 0.532 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 6 & 150 & 5.152 & 1.473 & 0.093 & 0.450 & 0.888 & 66.200 & 0.564 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 6 & 150 & 4.943 & 1.375 & 0.165 & 0.390 & 0.908 & 64.800 & 0.597 \\
Talking-Babies-cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 150 & 4.410 & 1.191 & 0.070 & 0.252 & 0.885 & 78.400 & 0.320 \\
Talking-Babies-orpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 150 & 5.056 & 1.165 & 0.086 & 0.437 & 0.827 & 75.800 & 0.439 \\
Talking-Babies-orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 150 & 4.621 & 1.283 & 0.077 & 0.306 & 0.876 & 58.000 & 0.374 \\
babylm-seqlen-opt-1024-warmup-v2 & 6 & 150 & 5.060 & 1.429 & 0.076 & 0.439 & 0.858 & 66.000 & 0.499 \\
babylm-seqlen-opt-4096-warmup-v2 & 6 & 150 & 4.537 & 1.213 & 0.063 & 0.266 & 0.890 & 89.300 & 0.347 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 6 & 200 & 5.023 & 1.419 & 0.089 & 0.412 & 0.898 & 91.200 & 0.542 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 6 & 200 & 4.785 & 1.297 & 0.122 & 0.363 & 0.776 & 117.700 & 0.449 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 6 & 200 & 4.934 & 1.398 & 0.120 & 0.369 & 0.832 & 88.800 & 0.505 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 6 & 200 & 4.947 & 1.363 & 0.142 & 0.378 & 0.888 & 79.700 & 0.560 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 6 & 200 & 4.964 & 1.372 & 0.090 & 0.411 & 0.889 & 71.100 & 0.506 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 6 & 200 & 5.100 & 1.431 & 0.088 & 0.382 & 0.915 & 77.400 & 0.544 \\
Talking-Babies-cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 200 & 4.510 & 1.267 & 0.084 & 0.244 & 0.809 & 98.300 & 0.328 \\
Talking-Babies-orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 200 & 4.456 & 1.293 & 0.120 & 0.245 & 0.909 & 118.600 & 0.451 \\
babylm-seqlen-opt-1024-warmup-v2 & 6 & 200 & 4.897 & 1.397 & 0.110 & 0.376 & 0.946 & 100.700 & 0.573 \\
babylm-seqlen-opt-4096-warmup-v2 & 6 & 200 & 4.402 & 1.181 & 0.047 & 0.227 & 0.870 & 113.300 & 0.295 \\
Talking-Babies-cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 250 & 4.375 & 1.179 & 0.104 & 0.212 & 0.857 & 132.200 & 0.360 \\
Talking-Babies-orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 250 & 4.498 & 1.226 & 0.151 & 0.214 & 0.932 & 130.800 & 0.492 \\
babylm-seqlen-opt-4096-warmup-v2 & 6 & 250 & 4.298 & 1.118 & 0.070 & 0.168 & 0.780 & 182.400 & 0.264 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_final\_checkpoint & 8 & 50 & 4.917 & 1.346 & 0.058 & 0.523 & 0.893 & 40.100 & 0.476 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 8 & 50 & 4.786 & 1.307 & 0.063 & 0.507 & 0.894 & 27.500 & 0.444 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 8 & 50 & 5.018 & 1.400 & 0.063 & 0.524 & 0.881 & 30.600 & 0.491 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 8 & 50 & 4.790 & 1.324 & 0.066 & 0.489 & 0.842 & 30.500 & 0.413 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 8 & 50 & 4.858 & 1.346 & 0.075 & 0.510 & 0.885 & 34.000 & 0.475 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 8 & 50 & 4.874 & 1.345 & 0.070 & 0.500 & 0.948 & 29.700 & 0.506 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 8 & 50 & 4.889 & 1.355 & 0.070 & 0.519 & 0.856 & 29.700 & 0.456 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 8 & 50 & 4.868 & 1.337 & 0.059 & 0.508 & 0.850 & 30.200 & 0.428 \\
Talking-Babies-cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 50 & 4.495 & 1.193 & 0.073 & 0.363 & 0.941 & 31.100 & 0.378 \\
Talking-Babies-orpo\_opt\_seqlen\_1024\_final\_checkpoint & 8 & 50 & 4.958 & 1.359 & 0.076 & 0.511 & 0.930 & 40.000 & 0.526 \\
Talking-Babies-orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 50 & 4.437 & 1.186 & 0.059 & 0.359 & 0.858 & 32.700 & 0.298 \\
babylm-seqlen-opt-1024-warmup-v2 & 8 & 50 & 4.845 & 1.344 & 0.063 & 0.504 & 0.937 & 33.400 & 0.489 \\
babylm-seqlen-opt-4096-warmup-v2 & 8 & 50 & 4.458 & 1.170 & 0.036 & 0.337 & 0.897 & 38.300 & 0.290 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_final\_checkpoint & 8 & 100 & 4.956 & 1.406 & 0.113 & 0.421 & 0.953 & 69.300 & 0.584 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 8 & 100 & 4.938 & 1.389 & 0.081 & 0.436 & 0.863 & 69.200 & 0.485 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 8 & 100 & 4.954 & 1.402 & 0.083 & 0.435 & 0.898 & 63.500 & 0.512 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 8 & 100 & 5.062 & 1.417 & 0.090 & 0.440 & 0.917 & 63.100 & 0.551 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 8 & 100 & 4.939 & 1.116 & 0.102 & 0.437 & 0.893 & 60.400 & 0.466 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 8 & 100 & 5.110 & 1.419 & 0.084 & 0.431 & 0.930 & 55.600 & 0.550 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 8 & 100 & 5.052 & 1.159 & 0.085 & 0.448 & 0.940 & 56.200 & 0.500 \\
Talking-Babies-cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 8 & 100 & 4.903 & 1.104 & 0.108 & 0.431 & 0.879 & 58.300 & 0.453 \\
Talking-Babies-cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 100 & 4.493 & 1.187 & 0.073 & 0.273 & 0.832 & 89.500 & 0.313 \\
Talking-Babies-orpo\_opt\_seqlen\_1024\_final\_checkpoint & 8 & 100 & 5.052 & 1.424 & 0.072 & 0.443 & 0.957 & 74.700 & 0.564 \\
Talking-Babies-orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 100 & 4.482 & 1.315 & 0.120 & 0.294 & 0.903 & 51.900 & 0.426 \\
babylm-seqlen-opt-1024-warmup-v2 & 8 & 100 & 5.002 & 1.432 & 0.084 & 0.447 & 0.829 & 59.200 & 0.482 \\
babylm-seqlen-opt-4096-warmup-v2 & 8 & 100 & 4.485 & 1.215 & 0.066 & 0.279 & 0.914 & 70.000 & 0.352 \\
Talking-Babies-cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 150 & 4.408 & 1.170 & 0.068 & 0.201 & 0.900 & 115.300 & 0.330 \\
Talking-Babies-orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 150 & 4.481 & 1.202 & 0.070 & 0.248 & 0.890 & 85.200 & 0.338 \\
babylm-seqlen-opt-4096-warmup-v2 & 8 & 150 & 4.505 & 1.218 & 0.036 & 0.251 & 0.856 & 100.000 & 0.293 \\
Talking-Babies-cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 200 & 4.366 & 1.223 & 0.109 & 0.196 & 0.934 & 198.200 & 0.464 \\
Talking-Babies-orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 200 & 4.663 & 1.284 & 0.107 & 0.247 & 0.830 & 113.100 & 0.403 \\
babylm-seqlen-opt-4096-warmup-v2 & 8 & 200 & 4.446 & 1.166 & 0.114 & 0.183 & 0.841 & 154.400 & 0.372 \\
Talking-Babies-cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 250 & 4.366 & 1.207 & 0.129 & 0.159 & 0.838 & 245.300 & 0.442 \\
Talking-Babies-orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 250 & 4.434 & 1.283 & 0.141 & 0.181 & 0.938 & 254.000 & 0.561 \\
babylm-seqlen-opt-4096-warmup-v2 & 8 & 250 & 4.531 & 1.193 & 0.063 & 0.171 & 0.715 & 162.200 & 0.245 \\
\bottomrule
\end{tabular}
\caption{Average metrics per BabyLM setting with min--max normalized aggregate (NormAvg) across metrics.}
\label{tab:dialogue-metrics_v3}
\end{table*}


==> tables/main-table.tex <==
\onecolumn 

\subsection{CPO and ORPO Models (Experiment 1)}

%\begin{landscape}
\small
\setlength{\tabcolsep}{4pt}

\iffalse
%%%% TABLE 1 - BASELINES
\begin{longtable}{lrrrrrrrrrrrrr}
\toprule
\textbf{BabyLM} & \textbf{Turns} & \textbf{Length} & \textbf{AoA} & \textbf{CEFR} & \textbf{Overlap} & \textbf{TTR} & \textbf{Rep.} & \textbf{NumCon} & \textbf{AdversativeCon} & \textbf{Polysemy} & \textbf{VerbRep} & \textbf{Narrativity} & \textbf{NormAvg} \\
\midrule
\endfirsthead

%\multicolumn{14}{c}%
%{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
%\toprule
%\textbf{BabyLM} & \textbf{Turns} & \textbf{Length} & \textbf{AoA} & \textbf{CEFR} & \textbf{Overlap} & \textbf{TTR} & \textbf{Rep.} & \textbf{NumCon} & \textbf{AdversativeCon} & \textbf{Polysemy} & \textbf{VerbRep} & \textbf{Narrativity} & \textbf{NormAvg} \\
\midrule
\endhead

%\midrule \multicolumn{14}{r}{{Continued on next page}} \\
%\endfoot

cpo-opt & 4 & 50 & 5.087 & 1.373 & 0.068 & 0.620 & 0.851 & 13.300 & 0.900 & 7.772 & 0.772 & 0.000 & 0.436 \\
cpo\_opt\_base & 4 & 50 & 5.214 & 1.468 & 0.074 & 0.590 & 0.881 & 13.100 & 0.900 & 7.241 & 0.684 & 0.000 & 0.425 \\
orpo\_opt\_100M\_2048\_preprocess & 4 & 50 & 5.123 & 1.415 & 0.078 & 0.582 & 0.777 & 14.300 & 1.100 & 7.963 & 0.814 & 0.000 & 0.440 \\
cpo\_opt\_100M\_2048\_preprocess & 4 & 100 & 5.028 & 1.417 & 0.121 & 0.508 & 0.931 & 23.400 & 2.300 & 7.776 & 0.857 & 0.000 & 0.529 \\
cpo\_opt\_base & 4 & 100 & 5.075 & 1.404 & 0.088 & 0.496 & 0.847 & 21.000 & 1.300 & 8.294 & 0.715 & 0.000 & 0.431 \\
orpo\_opt\_100M\_2048\_preprocess & 4 & 100 & 5.021 & 1.419 & 0.085 & 0.524 & 0.862 & 20.300 & 0.800 & 8.210 & 0.851 & 0.000 & 0.483 \\
cpo\_opt\_100M\_2048\_preprocess & 4 & 150 & 5.057 & 1.441 & 0.115 & 0.469 & 0.828 & 33.400 & 1.200 & 7.582 & 0.708 & -0.000 & 0.416 \\
cpo\_opt\_base & 4 & 150 & 5.153 & 1.433 & 0.082 & 0.458 & 0.883 & 34.500 & 1.700 & 8.358 & 0.837 & -0.000 & 0.470 \\
orpo\_opt\_100M\_2048\_preprocess & 4 & 150 & 5.169 & 1.432 & 0.109 & 0.473 & 0.766 & 33.300 & 1.600 & 8.092 & 0.722 & 0.000 & 0.441 \\
cpo\_opt\_100M\_2048\_preprocess & 4 & 200 & 5.171 & 0.932 & 0.108 & 0.432 & 0.904 & 40.300 & 3.100 & 8.410 & 0.767 & -0.000 & 0.420 \\
cpo\_opt\_base & 4 & 200 & 5.378 & 1.506 & 0.099 & 0.433 & 0.882 & 41.500 & 0.900 & 7.803 & 0.738 & -0.000 & 0.457 \\
orpo\_opt\_100M\_2048\_preprocess & 4 & 200 & 5.080 & 1.198 & 0.100 & 0.463 & 0.928 & 39.000 & 3.600 & 8.636 & 0.797 & -0.000 & 0.490 \\
cpo\_opt\_100M\_2048\_preprocess & 4 & 250 & 5.054 & 1.393 & 0.125 & 0.396 & 0.950 & 57.700 & 2.500 & 8.453 & 0.827 & 0.000 & 0.547 \\
cpo\_opt\_base & 4 & 250 & 5.655 & 1.647 & 0.108 & 0.411 & 0.835 & 47.300 & 3.000 & 7.798 & 0.780 & -0.000 & 0.524 \\
orpo\_opt\_100M\_2048\_preprocess & 4 & 250 & 5.160 & 1.247 & 0.101 & 0.424 & 0.897 & 47.700 & 4.100 & 8.531 & 0.830 & 0.000 & 0.525 \\
cpo\_opt\_100M\_2048\_preprocess & 6 & 50 & 5.071 & 1.423 & 0.065 & 0.564 & 0.830 & 19.000 & 2.500 & 8.146 & 0.740 & 0.000 & 0.434 \\
cpo\_opt\_base & 6 & 50 & 5.022 & 1.355 & 0.057 & 0.549 & 0.891 & 18.400 & 1.800 & 8.236 & 0.766 & -0.000 & 0.432 \\
orpo\_opt\_100M\_2048\_preprocess & 6 & 50 & 5.145 & 1.411 & 0.082 & 0.546 & 0.865 & 18.400 & 0.700 & 7.507 & 0.817 & 0.000 & 0.462 \\
cpo\_opt\_100M\_2048\_preprocess & 6 & 100 & 5.093 & 1.437 & 0.090 & 0.483 & 0.858 & 36.100 & 1.600 & 8.253 & 0.776 & 0.000 & 0.493 \\
cpo\_opt\_base & 6 & 100 & 5.035 & 1.429 & 0.080 & 0.489 & 0.892 & 38.500 & 2.500 & 8.295 & 0.780 & -0.000 & 0.472 \\
orpo\_opt\_100M\_2048\_preprocess & 6 & 100 & 4.984 & 1.399 & 0.093 & 0.479 & 0.853 & 41.800 & 3.200 & 8.917 & 0.748 & -0.000 & 0.463 \\
\bottomrule
%\endlastfoot
\caption{Average metrics per BabyLM setting with min--max normalized aggregate (NormAvg) across metrics for the baseline models.} \\
\end{longtable}
\fi

%%%% TABLE 1 - BASELINES_a
\begin{longtable}{lrrrrrrrr}
\toprule
\textbf{BabyLM} & \textbf{Turns} & \textbf{Length} & \textbf{AoA} & \textbf{CEFR} & \textbf{Overlap} & \textbf{TTR} & \textbf{Rep.} & \textbf{NumCon} \\
\midrule
cpo\_opt\_100M\_2048\_preprocess & 4 & 50 & 5.087 & 1.373 & 0.068 & 0.620 & 0.851 & 13.300 \\
cpo\_opt\_base & 4 & 50 & 5.214 & 1.468 & 0.074 & 0.590 & 0.881 & 13.100 \\
orpo\_opt\_100M\_2048\_preprocess & 4 & 50 & 5.123 & 1.415 & 0.078 & 0.582 & 0.777 & 14.300 \\
cpo\_opt\_100M\_2048\_preprocess & 4 & 100 & 5.028 & 1.417 & 0.121 & 0.508 & 0.931 & 23.400 \\
cpo\_opt\_base & 4 & 100 & 5.075 & 1.404 & 0.088 & 0.496 & 0.847 & 21.000 \\
orpo\_opt\_100M\_2048\_preprocess & 4 & 100 & 5.021 & 1.419 & 0.085 & 0.524 & 0.862 & 20.300 \\
cpo\_opt\_100M\_2048\_preprocess & 4 & 150 & 5.057 & 1.441 & 0.115 & 0.469 & 0.828 & 33.400 \\
cpo\_opt\_base & 4 & 150 & 5.153 & 1.433 & 0.082 & 0.458 & 0.883 & 34.500 \\
orpo\_opt\_100M\_2048\_preprocess & 4 & 150 & 5.169 & 1.432 & 0.109 & 0.473 & 0.766 & 33.300 \\
cpo\_opt\_100M\_2048\_preprocess & 4 & 200 & 5.171 & 0.932 & 0.108 & 0.432 & 0.904 & 40.300 \\
cpo\_opt\_base & 4 & 200 & 5.378 & 1.506 & 0.099 & 0.433 & 0.882 & 41.500 \\
orpo\_opt\_100M\_2048\_preprocess & 4 & 200 & 5.080 & 1.198 & 0.100 & 0.463 & 0.928 & 39.000 \\
cpo\_opt\_100M\_2048\_preprocess & 4 & 250 & 5.054 & 1.393 & 0.125 & 0.396 & 0.950 & 57.700 \\
cpo\_opt\_base & 4 & 250 & 5.655 & 1.647 & 0.108 & 0.411 & 0.835 & 47.300 \\
orpo\_opt\_100M\_2048\_preprocess & 4 & 250 & 5.160 & 1.247 & 0.101 & 0.424 & 0.897 & 47.700 \\
cpo\_opt\_100M\_2048\_preprocess & 6 & 50 & 5.071 & 1.423 & 0.065 & 0.564 & 0.830 & 19.000 \\
cpo\_opt\_base & 6 & 50 & 5.022 & 1.355 & 0.057 & 0.549 & 0.891 & 18.400 \\
orpo\_opt\_100M\_2048\_preprocess & 6 & 50 & 5.145 & 1.411 & 0.082 & 0.546 & 0.865 & 18.400 \\
cpo\_opt\_100M\_2048\_preprocess & 6 & 100 & 5.093 & 1.437 & 0.090 & 0.483 & 0.858 & 36.100 \\
cpo\_opt\_base & 6 & 100 & 5.035 & 1.429 & 0.080 & 0.489 & 0.892 & 38.500 \\
orpo\_opt\_100M\_2048\_preprocess & 6 & 100 & 4.984 & 1.399 & 0.093 & 0.479 & 0.853 & 41.800 \\
\bottomrule
\caption{Average metrics per BabyLM setting with min--max normalized aggregate (NormAvg) across metrics for the baseline models.} \\
\end{longtable}

%%%% TABLE 1 - BASELINES_b

\setcounter{table}{8}
\renewcommand{\thetable}{\arabic{table} (contd.)}

\begin{longtable}{lrrrrrrr}
\toprule
\textbf{BabyLM} & \textbf{Turns} & \textbf{Length} & \textbf{AdversativeCon} & \textbf{Polysemy} & \textbf{VerbRep} & \textbf{Narrativity} & \textbf{NormAvg} \\
\midrule
cpo\_opt\_100M\_2048\_preprocess & 4 & 50 & 0.900 & 7.772 & 0.772 & 0.000 & 0.436 \\
cpo\_opt\_base & 4 & 50 & 0.900 & 7.241 & 0.684 & 0.000 & 0.425 \\
orpo\_opt\_100M\_2048\_preprocess & 4 & 50 & 1.100 & 7.963 & 0.814 & 0.000 & 0.440 \\
cpo\_opt\_100M\_2048\_preprocess & 4 & 100 & 2.300 & 7.776 & 0.857 & 0.000 & 0.529 \\
cpo\_opt\_base & 4 & 100 & 1.300 & 8.294 & 0.715 & 0.000 & 0.431 \\
orpo\_opt\_100M\_2048\_preprocess & 4 & 100 & 0.800 & 8.210 & 0.851 & 0.000 & 0.483 \\
cpo\_opt\_100M\_2048\_preprocess & 4 & 150 & 1.200 & 7.582 & 0.708 & -0.000 & 0.416 \\
cpo\_opt\_base & 4 & 150 & 1.700 & 8.358 & 0.837 & -0.000 & 0.470 \\
orpo\_opt\_100M\_2048\_preprocess & 4 & 150 & 1.600 & 8.092 & 0.722 & 0.000 & 0.441 \\
cpo\_opt\_100M\_2048\_preprocess & 4 & 200 & 3.100 & 8.410 & 0.767 & -0.000 & 0.420 \\
cpo\_opt\_base & 4 & 200 & 0.900 & 7.803 & 0.738 & -0.000 & 0.457 \\
orpo\_opt\_100M\_2048\_preprocess & 4 & 200 & 3.600 & 8.636 & 0.797 & -0.000 & 0.490 \\
cpo\_opt\_100M\_2048\_preprocess & 4 & 250 & 2.500 & 8.453 & 0.827 & 0.000 & 0.547 \\
cpo\_opt\_base & 4 & 250 & 3.000 & 7.798 & 0.780 & -0.000 & 0.524 \\
orpo\_opt\_100M\_2048\_preprocess & 4 & 250 & 4.100 & 8.531 & 0.830 & 0.000 & 0.525 \\
cpo\_opt\_100M\_2048\_preprocess & 6 & 50 & 2.500 & 8.146 & 0.740 & 0.000 & 0.434 \\
cpo\_opt\_base & 6 & 50 & 1.800 & 8.236 & 0.766 & -0.000 & 0.432 \\
orpo\_opt\_100M\_2048\_preprocess & 6 & 50 & 0.700 & 7.507 & 0.817 & 0.000 & 0.462 \\
cpo\_opt\_100M\_2048\_preprocess & 6 & 100 & 1.600 & 8.253 & 0.776 & 0.000 & 0.493 \\
cpo\_opt\_base & 6 & 100 & 2.500 & 8.295 & 0.780 & -0.000 & 0.472 \\
orpo\_opt\_100M\_2048\_preprocess & 6 & 100 & 3.200 & 8.917 & 0.748 & -0.000 & 0.463 \\
\bottomrule
\caption{Average metrics per BabyLM setting with min--max normalized aggregate (NormAvg) across metrics for the baseline models.} \\
\end{longtable}

\renewcommand{\thetable}{\arabic{table}}
\newpage

\iffalse
%%%% TABLE 2 - CPO/ORPO
\begin{longtable}{lrrrrrrrrrrrrr}
\caption{Average metrics per BabyLM setting with NormAvg across metrics for ORPO/CPO models.} \\
\toprule
\textbf{BabyLM} & \textbf{Turns} & \textbf{Length} & \textbf{AoA} & \textbf{CEFR} & \textbf{Overlap} & \textbf{TTR} & \textbf{Rep.} & \textbf{NumCon} & \textbf{AdversativeCon} & \textbf{Polysemy} & \textbf{VerbRep} & \textbf{Narrativity} & \textbf{NormAvg} \\
\midrule
\endfirsthead

\multicolumn{14}{c}%
{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\toprule
\textbf{BabyLM} & \textbf{Turns} & \textbf{Length} & \textbf{AoA} & \textbf{CEFR} & \textbf{Overlap} & \textbf{TTR} & \textbf{Rep.} & \textbf{NumCon} & \textbf{AdversativeCon} & \textbf{Polysemy} & \textbf{VerbRep} & \textbf{Narrativity} & \textbf{NormAvg} \\
\midrule
\endhead

\midrule \multicolumn{14}{r}{{Continued on next page}} \\
\endfoot

\newpage 
\bottomrule
\endlastfoot
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 50 & 5.011 & 1.408 & 0.044 & 0.624 & 0.946 & 15.600 & 1.600 & 8.118 & 0.790 & 0.000 & 0.496 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 50 & 4.523 & 1.219 & 0.046 & 0.464 & 0.797 & 18.100 & 1.600 & 9.379 & 0.753 & 0.000 & 0.389 \\
opt-sam-orpo-mamba-2048-step448 & 4 & 50 & 4.887 & 1.376 & 0.072 & 0.617 & 0.918 & 16.800 & 1.900 & 8.294 & 0.797 & 0.000 & 0.513 \\
opt-sam-orpo-seqlen-2048-step559 & 4 & 50 & 4.948 & 1.365 & 0.052 & 0.615 & 0.866 & 15.100 & 1.400 & 8.926 & 0.590 & 0.000 & 0.390 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 50 & 4.813 & 1.343 & 0.066 & 0.604 & 0.898 & 17.900 & 1.700 & 8.916 & 0.763 & 0.000 & 0.459 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 50 & 4.487 & 1.228 & 0.075 & 0.473 & 0.879 & 11.500 & 1.400 & 8.631 & 0.720 & -0.000 & 0.346 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 100 & 4.921 & 1.353 & 0.062 & 0.537 & 0.955 & 35.900 & 3.300 & 9.218 & 0.839 & -0.000 & 0.521 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 100 & 4.532 & 1.224 & 0.058 & 0.391 & 0.891 & 33.300 & 3.000 & 9.435 & 0.821 & 0.000 & 0.419 \\
opt-sam-orpo-mamba-2048-step448 & 4 & 100 & 4.797 & 1.390 & 0.099 & 0.514 & 0.799 & 42.100 & 5.400 & 9.338 & 0.870 & -0.000 & 0.517 \\
opt-sam-orpo-seqlen-2048-step559 & 4 & 100 & 4.728 & 1.304 & 0.077 & 0.512 & 0.893 & 40.100 & 3.800 & 9.944 & 0.844 & -0.000 & 0.476 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 100 & 4.953 & 1.365 & 0.068 & 0.534 & 0.909 & 35.200 & 3.300 & 8.949 & 0.778 & -0.000 & 0.485 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 100 & 4.711 & 1.262 & 0.062 & 0.419 & 0.870 & 19.600 & 1.400 & 8.710 & 0.768 & -0.000 & 0.373 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 150 & 4.912 & 1.360 & 0.104 & 0.445 & 0.959 & 52.600 & 5.000 & 9.865 & 0.852 & 0.000 & 0.584 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 150 & 4.385 & 1.256 & 0.128 & 0.302 & 0.749 & 49.200 & 3.600 & 9.345 & 0.775 & 0.000 & 0.413 \\
opt-sam-orpo-mamba-2048-step448 & 4 & 150 & 4.880 & 1.384 & 0.073 & 0.470 & 0.870 & 64.800 & 7.600 & 9.414 & 0.783 & -0.000 & 0.519 \\
opt-sam-orpo-seqlen-2048-step559 & 4 & 150 & 4.910 & 1.371 & 0.069 & 0.473 & 0.921 & 47.300 & 3.500 & 8.704 & 0.787 & -0.000 & 0.482 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 150 & 5.077 & 1.395 & 0.076 & 0.474 & 0.825 & 69.600 & 4.500 & 8.858 & 0.815 & -0.000 & 0.470 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 150 & 4.732 & 1.301 & 0.078 & 0.391 & 0.855 & 37.700 & 2.500 & 8.890 & 0.724 & -0.000 & 0.391 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 200 & 4.960 & 1.394 & 0.105 & 0.427 & 0.891 & 67.500 & 4.300 & 9.388 & 0.823 & -0.000 & 0.521 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 200 & 4.367 & 1.188 & 0.082 & 0.245 & 0.770 & 102.700 & 3.000 & 9.584 & 0.875 & -0.000 & 0.369 \\
opt-sam-orpo-mamba-2048-step448 & 4 & 200 & 5.049 & 1.435 & 0.095 & 0.438 & 0.853 & 76.100 & 7.200 & 9.044 & 0.839 & 0.000 & 0.577 \\
opt-sam-orpo-seqlen-2048-step559 & 4 & 200 & 4.825 & 1.152 & 0.090 & 0.456 & 0.829 & 62.500 & 5.100 & 9.511 & 0.872 & 0.000 & 0.513 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 200 & 5.047 & 0.888 & 0.094 & 0.438 & 0.948 & 71.000 & 4.000 & 8.855 & 0.854 & -0.000 & 0.473 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 200 & 4.533 & 1.340 & 0.122 & 0.306 & 0.808 & 65.100 & 2.600 & 8.758 & 0.788 & 0.000 & 0.423 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 250 & 4.932 & 1.391 & 0.103 & 0.411 & 0.819 & 80.200 & 7.300 & 9.086 & 0.855 & 0.000 & 0.550 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 250 & 4.632 & 1.245 & 0.094 & 0.286 & 0.891 & 78.300 & 2.500 & 9.265 & 0.794 & 0.000 & 0.443 \\
opt-sam-orpo-mamba-2048-step448 & 4 & 250 & 4.777 & 1.140 & 0.126 & 0.388 & 0.778 & 108.300 & 12.200 & 8.808 & 0.877 & -0.000 & 0.525 \\
opt-sam-orpo-seqlen-2048-step559 & 4 & 250 & 5.091 & 1.454 & 0.092 & 0.407 & 0.861 & 67.500 & 5.600 & 8.867 & 0.791 & -0.000 & 0.518 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 250 & 5.073 & 1.197 & 0.096 & 0.412 & 0.888 & 90.700 & 8.200 & 9.247 & 0.846 & 0.000 & 0.567 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 250 & 4.741 & 1.391 & 0.117 & 0.318 & 0.810 & 49.500 & 3.900 & 7.859 & 0.794 & -0.000 & 0.395 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 50 & 4.947 & 1.405 & 0.050 & 0.563 & 0.911 & 25.900 & 1.800 & 8.552 & 0.745 & 0.000 & 0.461 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 50 & 4.525 & 1.231 & 0.094 & 0.411 & 0.921 & 22.500 & 1.600 & 8.597 & 0.787 & -0.000 & 0.387 \\
opt-sam-orpo-mamba-2048-step448 & 6 & 50 & 4.831 & 1.369 & 0.084 & 0.553 & 0.912 & 24.200 & 3.500 & 9.184 & 0.758 & 0.000 & 0.505 \\
opt-sam-orpo-seqlen-2048-step559 & 6 & 50 & 5.072 & 1.382 & 0.055 & 0.576 & 0.868 & 25.400 & 2.300 & 9.109 & 0.778 & 0.000 & 0.514 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 50 & 4.951 & 1.390 & 0.065 & 0.567 & 0.927 & 26.100 & 2.400 & 8.366 & 0.744 & -0.000 & 0.449 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 50 & 4.612 & 1.234 & 0.061 & 0.419 & 0.907 & 19.000 & 2.000 & 9.567 & 0.793 & -0.000 & 0.401 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 100 & 4.904 & 1.364 & 0.094 & 0.456 & 0.932 & 55.000 & 5.000 & 9.643 & 0.883 & 0.000 & 0.583 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 100 & 4.430 & 1.320 & 0.129 & 0.299 & 0.764 & 55.700 & 3.000 & 8.628 & 0.791 & 0.000 & 0.392 \\
opt-sam-orpo-mamba-2048-step448 & 6 & 100 & 4.959 & 1.411 & 0.066 & 0.478 & 0.962 & 60.700 & 6.500 & 8.757 & 0.757 & -0.000 & 0.516 \\
opt-sam-orpo-seqlen-2048-step559 & 6 & 100 & 4.912 & 1.352 & 0.080 & 0.508 & 0.944 & 44.600 & 3.800 & 8.853 & 0.841 & -0.000 & 0.517 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 100 & 4.965 & 1.382 & 0.069 & 0.467 & 0.888 & 57.200 & 5.100 & 9.444 & 0.759 & -0.000 & 0.483 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 100 & 4.626 & 1.274 & 0.060 & 0.362 & 0.937 & 34.500 & 2.900 & 8.691 & 0.778 & 0.000 & 0.428 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 150 & 5.236 & 1.493 & 0.075 & 0.460 & 0.954 & 75.800 & 4.900 & 8.650 & 0.882 & -0.000 & 0.574 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 150 & 4.410 & 1.191 & 0.070 & 0.252 & 0.885 & 78.400 & 5.300 & 9.609 & 0.793 & 0.000 & 0.426 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 150 & 5.056 & 1.165 & 0.086 & 0.437 & 0.827 & 75.800 & 6.200 & 8.885 & 0.886 & -0.000 & 0.499 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 150 & 4.621 & 1.283 & 0.077 & 0.306 & 0.876 & 58.000 & 4.400 & 8.878 & 0.763 & -0.000 & 0.402 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 200 & 4.510 & 1.267 & 0.084 & 0.244 & 0.809 & 98.300 & 3.700 & 9.394 & 0.811 & 0.000 & 0.447 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 200 & 4.456 & 1.293 & 0.120 & 0.245 & 0.909 & 118.600 & 5.200 & 9.021 & 0.796 & 0.000 & 0.520 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 250 & 4.375 & 1.179 & 0.104 & 0.212 & 0.857 & 132.200 & 3.300 & 9.918 & 0.816 & -0.000 & 0.429 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 250 & 4.498 & 1.226 & 0.151 & 0.214 & 0.932 & 130.800 & 5.000 & 10.981 & 0.817 & 0.000 & 0.578 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 8 & 50 & 4.917 & 1.346 & 0.058 & 0.523 & 0.893 & 40.100 & 2.800 & 8.185 & 0.818 & 0.000 & 0.491 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 50 & 4.495 & 1.193 & 0.073 & 0.363 & 0.941 & 31.100 & 2.000 & 9.187 & 0.745 & 0.000 & 0.406 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 8 & 50 & 4.958 & 1.359 & 0.076 & 0.511 & 0.930 & 40.000 & 3.800 & 9.058 & 0.807 & 0.000 & 0.567 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 50 & 4.437 & 1.186 & 0.059 & 0.359 & 0.858 & 32.700 & 4.500 & 8.461 & 0.701 & 0.000 & 0.337 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 8 & 100 & 4.956 & 1.406 & 0.113 & 0.421 & 0.953 & 69.300 & 4.300 & 8.717 & 0.882 & 0.000 & 0.591 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 100 & 4.493 & 1.187 & 0.073 & 0.273 & 0.832 & 89.500 & 4.300 & 9.361 & 0.808 & -0.000 & 0.383 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 8 & 100 & 5.052 & 1.424 & 0.072 & 0.443 & 0.957 & 74.700 & 5.800 & 8.705 & 0.847 & 0.000 & 0.590 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 100 & 4.482 & 1.315 & 0.120 & 0.294 & 0.903 & 51.900 & 4.100 & 8.326 & 0.807 & -0.000 & 0.394 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 150 & 4.408 & 1.170 & 0.068 & 0.201 & 0.900 & 115.300 & 3.100 & 9.759 & 0.798 & 0.000 & 0.429 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 150 & 4.481 & 1.202 & 0.070 & 0.248 & 0.890 & 85.200 & 3.000 & 8.217 & 0.825 & 0.000 & 0.394 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 200 & 4.366 & 1.223 & 0.109 & 0.196 & 0.934 & 198.200 & 4.000 & 9.354 & 0.851 & -0.000 & 0.471 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 200 & 4.663 & 1.284 & 0.107 & 0.247 & 0.830 & 113.100 & 5.400 & 8.748 & 0.794 & 0.000 & 0.450 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 250 & 4.366 & 1.207 & 0.129 & 0.159 & 0.838 & 245.300 & 5.200 & 9.399 & 0.865 & 0.000 & 0.508 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 250 & 4.434 & 1.283 & 0.141 & 0.181 & 0.938 & 254.000 & 5.700 & 9.094 & 0.863 & 0.000 & 0.614 \\
\end{longtable}
\fi


%%%% TABLE 2 - CPO/ORPO_a
\begin{longtable}{lrrrrrrrr}
\toprule
\textbf{BabyLM} & \textbf{Turns} & \textbf{Length} & \textbf{AoA} & \textbf{CEFR} & \textbf{Overlap} & \textbf{TTR} & \textbf{Rep.} & \textbf{NumCon} \\
\midrule

cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 50 & 5.011 & 1.408 & 0.044 & 0.624 & 0.946 & 15.600 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 50 & 4.523 & 1.219 & 0.046 & 0.464 & 0.797 & 18.100 \\
opt-sam-orpo-mamba-2048-step448 & 4 & 50 & 4.887 & 1.376 & 0.072 & 0.617 & 0.918 & 16.800 \\
opt-sam-orpo-seqlen-2048-step559 & 4 & 50 & 4.948 & 1.365 & 0.052 & 0.615 & 0.866 & 15.100 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 50 & 4.813 & 1.343 & 0.066 & 0.604 & 0.898 & 17.900 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 50 & 4.487 & 1.228 & 0.075 & 0.473 & 0.879 & 11.500 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 100 & 4.921 & 1.353 & 0.062 & 0.537 & 0.955 & 35.900 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 100 & 4.532 & 1.224 & 0.058 & 0.391 & 0.891 & 33.300 \\
opt-sam-orpo-mamba-2048-step448 & 4 & 100 & 4.797 & 1.390 & 0.099 & 0.514 & 0.799 & 42.100 \\
opt-sam-orpo-seqlen-2048-step559 & 4 & 100 & 4.728 & 1.304 & 0.077 & 0.512 & 0.893 & 40.100 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 100 & 4.953 & 1.365 & 0.068 & 0.534 & 0.909 & 35.200 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 100 & 4.711 & 1.262 & 0.062 & 0.419 & 0.870 & 19.600 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 150 & 4.912 & 1.360 & 0.104 & 0.445 & 0.959 & 52.600 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 150 & 4.385 & 1.256 & 0.128 & 0.302 & 0.749 & 49.200 \\
opt-sam-orpo-mamba-2048-step448 & 4 & 150 & 4.880 & 1.384 & 0.073 & 0.470 & 0.870 & 64.800 \\
opt-sam-orpo-seqlen-2048-step559 & 4 & 150 & 4.910 & 1.371 & 0.069 & 0.473 & 0.921 & 47.300 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 150 & 5.077 & 1.395 & 0.076 & 0.474 & 0.825 & 69.600 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 150 & 4.732 & 1.301 & 0.078 & 0.391 & 0.855 & 37.700 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 200 & 4.960 & 1.394 & 0.105 & 0.427 & 0.891 & 67.500 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 200 & 4.367 & 1.188 & 0.082 & 0.245 & 0.770 & 102.700 \\
opt-sam-orpo-mamba-2048-step448 & 4 & 200 & 5.049 & 1.435 & 0.095 & 0.438 & 0.853 & 76.100 \\
opt-sam-orpo-seqlen-2048-step559 & 4 & 200 & 4.825 & 1.152 & 0.090 & 0.456 & 0.829 & 62.500 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 200 & 5.047 & 0.888 & 0.094 & 0.438 & 0.948 & 71.000 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 200 & 4.533 & 1.340 & 0.122 & 0.306 & 0.808 & 65.100 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 250 & 4.932 & 1.391 & 0.103 & 0.411 & 0.819 & 80.200 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 250 & 4.632 & 1.245 & 0.094 & 0.286 & 0.891 & 78.300 \\
opt-sam-orpo-mamba-2048-step448 & 4 & 250 & 4.777 & 1.140 & 0.126 & 0.388 & 0.778 & 108.300 \\
opt-sam-orpo-seqlen-2048-step559 & 4 & 250 & 5.091 & 1.454 & 0.092 & 0.407 & 0.861 & 67.500 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 250 & 5.073 & 1.197 & 0.096 & 0.412 & 0.888 & 90.700 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 250 & 4.741 & 1.391 & 0.117 & 0.318 & 0.810 & 49.500 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 50 & 4.947 & 1.405 & 0.050 & 0.563 & 0.911 & 25.900 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 50 & 4.525 & 1.231 & 0.094 & 0.411 & 0.921 & 22.500 \\
opt-sam-orpo-mamba-2048-step448 & 6 & 50 & 4.831 & 1.369 & 0.084 & 0.553 & 0.912 & 24.200 \\
opt-sam-orpo-seqlen-2048-step559 & 6 & 50 & 5.072 & 1.382 & 0.055 & 0.576 & 0.868 & 25.400 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 50 & 4.951 & 1.390 & 0.065 & 0.567 & 0.927 & 26.100 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 50 & 4.612 & 1.234 & 0.061 & 0.419 & 0.907 & 19.000 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 100 & 4.904 & 1.364 & 0.094 & 0.456 & 0.932 & 55.000 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 100 & 4.430 & 1.320 & 0.129 & 0.299 & 0.764 & 55.700 \\
opt-sam-orpo-mamba-2048-step448 & 6 & 100 & 4.959 & 1.411 & 0.066 & 0.478 & 0.962 & 60.700 \\
opt-sam-orpo-seqlen-2048-step559 & 6 & 100 & 4.912 & 1.352 & 0.080 & 0.508 & 0.944 & 44.600 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 100 & 4.965 & 1.382 & 0.069 & 0.467 & 0.888 & 57.200 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 100 & 4.626 & 1.274 & 0.060 & 0.362 & 0.937 & 34.500 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 150 & 5.236 & 1.493 & 0.075 & 0.460 & 0.954 & 75.800 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 150 & 4.410 & 1.191 & 0.070 & 0.252 & 0.885 & 78.400 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 150 & 5.056 & 1.165 & 0.086 & 0.437 & 0.827 & 75.800 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 150 & 4.621 & 1.283 & 0.077 & 0.306 & 0.876 & 58.000 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 200 & 4.510 & 1.267 & 0.084 & 0.244 & 0.809 & 98.300 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 200 & 4.456 & 1.293 & 0.120 & 0.245 & 0.909 & 118.600 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 250 & 4.375 & 1.179 & 0.104 & 0.212 & 0.857 & 132.200 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 250 & 4.498 & 1.226 & 0.151 & 0.214 & 0.932 & 130.800 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 8 & 50 & 4.917 & 1.346 & 0.058 & 0.523 & 0.893 & 40.100 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 50 & 4.495 & 1.193 & 0.073 & 0.363 & 0.941 & 31.100 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 8 & 50 & 4.958 & 1.359 & 0.076 & 0.511 & 0.930 & 40.000 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 50 & 4.437 & 1.186 & 0.059 & 0.359 & 0.858 & 32.700 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 8 & 100 & 4.956 & 1.406 & 0.113 & 0.421 & 0.953 & 69.300 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 100 & 4.493 & 1.187 & 0.073 & 0.273 & 0.832 & 89.500 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 8 & 100 & 5.052 & 1.424 & 0.072 & 0.443 & 0.957 & 74.700 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 100 & 4.482 & 1.315 & 0.120 & 0.294 & 0.903 & 51.900 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 150 & 4.408 & 1.170 & 0.068 & 0.201 & 0.900 & 115.300 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 150 & 4.481 & 1.202 & 0.070 & 0.248 & 0.890 & 85.200 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 200 & 4.366 & 1.223 & 0.109 & 0.196 & 0.934 & 198.200 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 200 & 4.663 & 1.284 & 0.107 & 0.247 & 0.830 & 113.100 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 250 & 4.366 & 1.207 & 0.129 & 0.159 & 0.838 & 245.300 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 250 & 4.434 & 1.283 & 0.141 & 0.181 & 0.938 & 254.000\\
\bottomrule
\caption{Average metrics per BabyLM setting with NormAvg across metrics for ORPO/CPO models.} \\

\end{longtable}

\newpage 
%%%% TABLE 2 - CPO/ORPO_b

\setcounter{table}{9}
\renewcommand{\thetable}{\arabic{table} (contd.)}

\begin{longtable}{lrrrrrrr}
\toprule
\textbf{BabyLM} & \textbf{Turns} & \textbf{Length} & \textbf{AdversativeCon} & \textbf{Polysemy} & \textbf{VerbRep} & \textbf{Narrativity} & \textbf{NormAvg} \\
\midrule

cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 50 & 1.600 & 8.118 & 0.790 & 0.000 & 0.496 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 50 & 1.600 & 9.379 & 0.753 & 0.000 & 0.389 \\
opt-sam-orpo-mamba-2048-step448 & 4 & 50 & 1.900 & 8.294 & 0.797 & 0.000 & 0.513 \\
opt-sam-orpo-seqlen-2048-step559 & 4 & 50 & 1.400 & 8.926 & 0.590 & 0.000 & 0.390 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 50 & 1.700 & 8.916 & 0.763 & 0.000 & 0.459 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 50 & 1.400 & 8.631 & 0.720 & -0.000 & 0.346 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 100 & 3.300 & 9.218 & 0.839 & -0.000 & 0.521 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 100 & 3.000 & 9.435 & 0.821 & 0.000 & 0.419 \\
opt-sam-orpo-mamba-2048-step448 & 4 & 100 & 5.400 & 9.338 & 0.870 & -0.000 & 0.517 \\
opt-sam-orpo-seqlen-2048-step559 & 4 & 100 & 3.800 & 9.944 & 0.844 & -0.000 & 0.476 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 100 & 3.300 & 8.949 & 0.778 & -0.000 & 0.485 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 100 & 1.400 & 8.710 & 0.768 & -0.000 & 0.373 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 150 & 5.000 & 9.865 & 0.852 & 0.000 & 0.584 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 150 & 3.600 & 9.345 & 0.775 & 0.000 & 0.413 \\
opt-sam-orpo-mamba-2048-step448 & 4 & 150 & 7.600 & 9.414 & 0.783 & -0.000 & 0.519 \\
opt-sam-orpo-seqlen-2048-step559 & 4 & 150 & 3.500 & 8.704 & 0.787 & -0.000 & 0.482 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 150 & 4.500 & 8.858 & 0.815 & -0.000 & 0.470 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 150 & 2.500 & 8.890 & 0.724 & -0.000 & 0.391 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 200 & 4.300 & 9.388 & 0.823 & -0.000 & 0.521 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 200 & 3.000 & 9.584 & 0.875 & -0.000 & 0.369 \\
opt-sam-orpo-mamba-2048-step448 & 4 & 200 & 7.200 & 9.044 & 0.839 & 0.000 & 0.577 \\
opt-sam-orpo-seqlen-2048-step559 & 4 & 200 & 5.100 & 9.511 & 0.872 & 0.000 & 0.513 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 200 & 4.000 & 8.855 & 0.854 & -0.000 & 0.473 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 200 & 2.600 & 8.758 & 0.788 & 0.000 & 0.423 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 250 & 7.300 & 9.086 & 0.855 & 0.000 & 0.550 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 250 & 2.500 & 9.265 & 0.794 & 0.000 & 0.443 \\
opt-sam-orpo-mamba-2048-step448 & 4 & 250 & 12.200 & 8.808 & 0.877 & -0.000 & 0.525 \\
opt-sam-orpo-seqlen-2048-step559 & 4 & 250 & 5.600 & 8.867 & 0.791 & -0.000 & 0.518 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 250 & 8.200 & 9.247 & 0.846 & 0.000 & 0.567 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 250 & 3.900 & 7.859 & 0.794 & -0.000 & 0.395 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 50 & 1.800 & 8.552 & 0.745 & 0.000 & 0.461 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 50 & 1.600 & 8.597 & 0.787 & -0.000 & 0.387 \\
opt-sam-orpo-mamba-2048-step448 & 6 & 50 & 3.500 & 9.184 & 0.758 & 0.000 & 0.505 \\
opt-sam-orpo-seqlen-2048-step559 & 6 & 50 & 2.300 & 9.109 & 0.778 & 0.000 & 0.514 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 50 & 2.400 & 8.366 & 0.744 & -0.000 & 0.449 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 50 & 2.000 & 9.567 & 0.793 & -0.000 & 0.401 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 100 & 5.000 & 9.643 & 0.883 & 0.000 & 0.583 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 100 & 3.000 & 8.628 & 0.791 & 0.000 & 0.392 \\
opt-sam-orpo-mamba-2048-step448 & 6 & 100 & 6.500 & 8.757 & 0.757 & -0.000 & 0.516 \\
opt-sam-orpo-seqlen-2048-step559 & 6 & 100 & 3.800 & 8.853 & 0.841 & -0.000 & 0.517 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 5.100 & 9.444 & 0.759 & -0.000 & 0.483 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 100 & 2.900 & 8.691 & 0.778 & 0.000 & 0.428 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 150 & 4.900 & 8.650 & 0.882 & -0.000 & 0.574 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 150 & 5.300 & 9.609 & 0.793 & 0.000 & 0.426 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 150 & 6.200 & 8.885 & 0.886 & -0.000 & 0.499 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 150 & 4.400 & 8.878 & 0.763 & -0.000 & 0.402 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 200 & 3.700 & 9.394 & 0.811 & 0.000 & 0.447 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 200 & 5.200 & 9.021 & 0.796 & 0.000 & 0.520 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 250 & 3.300 & 9.918 & 0.816 & -0.000 & 0.429 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 250 & 5.000 & 10.981 & 0.817 & 0.000 & 0.578 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 8 & 50 & 2.800 & 8.185 & 0.818 & 0.000 & 0.491 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 50 & 2.000 & 9.187 & 0.745 & 0.000 & 0.406 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 8 & 50 & 3.800 & 9.058 & 0.807 & 0.000 & 0.567 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 50 & 4.500 & 8.461 & 0.701 & 0.000 & 0.337 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 8 & 100 & 4.300 & 8.717 & 0.882 & 0.000 & 0.591 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 100 & 4.300 & 9.361 & 0.808 & -0.000 & 0.383 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 8 & 100 & 5.800 & 8.705 & 0.847 & 0.000 & 0.590 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 100 & 4.100 & 8.326 & 0.807 & -0.000 & 0.394 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 150 & 3.100 & 9.759 & 0.798 & 0.000 & 0.429 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 150 & 3.000 & 8.217 & 0.825 & 0.000 & 0.394 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 200 & 4.000 & 9.354 & 0.851 & -0.000 & 0.471 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 200 & 5.400 & 8.748 & 0.794 & 0.000 & 0.450 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 250 & 5.200 & 9.399 & 0.865 & 0.000 & 0.508 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 250 & 5.700 & 9.094 & 0.863 & 0.000 & 0.614 \\
\bottomrule
\caption{Average metrics per BabyLM setting with NormAvg across metrics for ORPO/CPO models.} \\
\end{longtable}

\renewcommand{\thetable}{\arabic{table}}
\newpage


\subsection{CEFR Progressive and Regressive (Experiment 2)}
%%%% TABLE 3 - CEFR progressive/regressive
\begin{longtable}{lrrrrrrrrrrrrr}
\caption{Average metrics per BabyLM setting with min--max normalized aggregate (NormAvg) across metrics for CEFR progressive/regressive models.} \\
\toprule
\textbf{BabyLM} & \textbf{Turns} & \textbf{Length} & \textbf{AoA} & \textbf{CEFR} & \textbf{Overlap} & \textbf{TTR} & \textbf{Rep.} & \textbf{NumCon} & \textbf{AdversativeCon} & \textbf{Polysemy} & \textbf{VerbRep} & \textbf{Narrativity} & \textbf{NormAvg} \\
\midrule
\endfirsthead

\multicolumn{14}{c}%
{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\toprule
\textbf{BabyLM} & \textbf{Turns} & \textbf{Length} & \textbf{AoA} & \textbf{CEFR} & \textbf{Overlap} & \textbf{TTR} & \textbf{Rep.} & \textbf{NumCon} & \textbf{AdversativeCon} & \textbf{Polysemy} & \textbf{VerbRep} & \textbf{Narrativity} & \textbf{NormAvg} \\
\midrule
\endhead

\midrule \multicolumn{14}{r}{{Continued on next page}} \\
\endfoot

\bottomrule
\endlastfoot
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 4 & 50 & 4.813 & 1.325 & 0.044 & 0.627 & 0.803 & 16.100 & 1.300 & 9.121 & 0.622 & 0.000 & 0.386 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 4 & 50 & 4.802 & 1.371 & 0.053 & 0.610 & 0.870 & 16.500 & 1.600 & 8.488 & 0.773 & 0.000 & 0.454 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 4 & 50 & 4.782 & 1.305 & 0.082 & 0.606 & 0.904 & 13.600 & 1.500 & 8.769 & 0.822 & -0.000 & 0.469 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 4 & 50 & 4.951 & 1.328 & 0.062 & 0.599 & 0.887 & 13.400 & 1.300 & 7.826 & 0.759 & 0.000 & 0.465 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 4 & 50 & 4.819 & 1.328 & 0.056 & 0.572 & 0.909 & 13.800 & 1.300 & 8.635 & 0.863 & -0.000 & 0.465 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 4 & 50 & 4.948 & 1.331 & 0.062 & 0.620 & 0.942 & 14.400 & 1.000 & 8.725 & 0.750 & -0.000 & 0.458 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 4 & 50 & 4.929 & 1.322 & 0.063 & 0.596 & 0.867 & 15.000 & 1.700 & 7.667 & 0.666 & 0.000 & 0.399 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 4 & 100 & 4.974 & 1.391 & 0.069 & 0.548 & 0.879 & 29.800 & 2.800 & 8.771 & 0.791 & 0.000 & 0.481 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 4 & 100 & 4.888 & 1.374 & 0.082 & 0.523 & 0.817 & 31.700 & 2.100 & 8.968 & 0.717 & 0.000 & 0.427 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 4 & 100 & 4.900 & 1.365 & 0.083 & 0.522 & 0.903 & 33.600 & 4.200 & 9.265 & 0.825 & 0.000 & 0.543 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 4 & 100 & 4.934 & 1.350 & 0.045 & 0.526 & 0.906 & 26.400 & 2.000 & 8.090 & 0.876 & 0.000 & 0.479 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 4 & 100 & 4.984 & 1.395 & 0.063 & 0.524 & 0.905 & 25.700 & 2.600 & 8.415 & 0.826 & -0.000 & 0.475 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 4 & 100 & 4.954 & 1.367 & 0.076 & 0.513 & 0.844 & 21.900 & 2.000 & 8.098 & 0.671 & 0.000 & 0.413 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 4 & 100 & 4.847 & 1.353 & 0.092 & 0.513 & 0.884 & 27.400 & 2.100 & 8.416 & 0.752 & 0.000 & 0.459 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 4 & 150 & 4.893 & 1.360 & 0.092 & 0.469 & 0.896 & 43.200 & 3.200 & 9.341 & 0.819 & 0.000 & 0.522 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 4 & 150 & 4.923 & 1.418 & 0.105 & 0.467 & 0.936 & 45.100 & 3.000 & 9.136 & 0.847 & 0.000 & 0.600 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 4 & 150 & 4.949 & 1.353 & 0.109 & 0.439 & 0.901 & 40.200 & 3.700 & 8.797 & 0.768 & 0.000 & 0.494 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 4 & 150 & 5.055 & 1.350 & 0.083 & 0.448 & 0.889 & 33.300 & 2.600 & 8.742 & 0.717 & -0.000 & 0.400 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 4 & 150 & 4.989 & 1.379 & 0.114 & 0.443 & 0.870 & 34.600 & 2.100 & 8.785 & 0.765 & 0.000 & 0.476 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 4 & 150 & 4.983 & 1.375 & 0.081 & 0.499 & 0.894 & 35.000 & 1.900 & 8.627 & 0.716 & 0.000 & 0.449 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 4 & 150 & 4.901 & 1.380 & 0.070 & 0.470 & 0.862 & 40.900 & 3.600 & 8.410 & 0.760 & -0.000 & 0.427 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 4 & 200 & 4.827 & 1.345 & 0.113 & 0.430 & 0.946 & 59.900 & 5.300 & 9.482 & 0.862 & -0.000 & 0.558 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 4 & 200 & 4.952 & 1.391 & 0.061 & 0.419 & 0.874 & 58.100 & 3.200 & 9.061 & 0.795 & 0.000 & 0.492 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 4 & 200 & 5.184 & 1.474 & 0.115 & 0.434 & 0.873 & 60.400 & 3.500 & 8.268 & 0.800 & -0.000 & 0.508 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 4 & 200 & 4.899 & 1.337 & 0.071 & 0.469 & 0.872 & 44.300 & 3.200 & 8.790 & 0.730 & -0.000 & 0.420 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 4 & 200 & 5.025 & 1.387 & 0.093 & 0.441 & 0.904 & 50.500 & 3.700 & 8.466 & 0.833 & -0.000 & 0.510 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 4 & 200 & 5.006 & 1.444 & 0.068 & 0.454 & 0.887 & 43.300 & 3.200 & 7.894 & 0.706 & -0.000 & 0.400 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 4 & 200 & 5.163 & 1.257 & 0.083 & 0.453 & 0.875 & 50.100 & 4.400 & 7.789 & 0.786 & 0.000 & 0.463 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 4 & 250 & 5.149 & 1.467 & 0.104 & 0.399 & 0.910 & 60.400 & 2.900 & 8.551 & 0.805 & -0.000 & 0.509 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 4 & 250 & 4.927 & 1.378 & 0.099 & 0.396 & 0.840 & 55.800 & 5.800 & 9.602 & 0.653 & 0.000 & 0.475 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 4 & 250 & 4.898 & 1.375 & 0.140 & 0.409 & 0.805 & 60.800 & 4.900 & 9.658 & 0.855 & 0.000 & 0.541 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 4 & 250 & 5.029 & 1.427 & 0.092 & 0.387 & 0.887 & 66.900 & 5.800 & 8.251 & 0.719 & -0.000 & 0.472 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 4 & 250 & 5.183 & 1.434 & 0.095 & 0.419 & 0.838 & 59.000 & 3.100 & 8.245 & 0.761 & 0.000 & 0.499 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 4 & 250 & 5.007 & 1.391 & 0.101 & 0.409 & 0.839 & 48.600 & 3.600 & 8.467 & 0.727 & 0.000 & 0.467 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 4 & 250 & 5.016 & 0.910 & 0.155 & 0.370 & 0.911 & 68.100 & 4.700 & 8.382 & 0.860 & 0.000 & 0.514 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 6 & 50 & 4.898 & 1.350 & 0.050 & 0.554 & 0.915 & 23.400 & 2.600 & 8.527 & 0.796 & 0.000 & 0.491 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 6 & 50 & 4.812 & 1.341 & 0.067 & 0.543 & 0.922 & 25.200 & 1.200 & 9.002 & 0.845 & 0.000 & 0.514 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 6 & 50 & 4.812 & 1.337 & 0.083 & 0.531 & 0.893 & 20.300 & 1.100 & 8.223 & 0.722 & 0.000 & 0.429 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 6 & 50 & 4.882 & 1.339 & 0.057 & 0.536 & 0.938 & 22.700 & 2.400 & 9.117 & 0.678 & 0.000 & 0.444 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 6 & 50 & 4.886 & 1.333 & 0.064 & 0.528 & 0.929 & 22.600 & 2.100 & 8.392 & 0.800 & 0.000 & 0.463 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 6 & 50 & 4.846 & 1.331 & 0.036 & 0.557 & 0.916 & 21.300 & 1.700 & 8.521 & 0.740 & 0.000 & 0.428 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 6 & 50 & 4.982 & 1.373 & 0.069 & 0.541 & 0.853 & 23.000 & 2.000 & 7.914 & 0.754 & -0.000 & 0.402 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 6 & 100 & 4.843 & 1.325 & 0.099 & 0.453 & 0.901 & 51.400 & 3.500 & 9.253 & 0.783 & 0.000 & 0.497 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 6 & 100 & 4.805 & 1.323 & 0.092 & 0.460 & 0.892 & 49.000 & 4.000 & 9.001 & 0.787 & 0.000 & 0.500 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 6 & 100 & 4.916 & 1.107 & 0.112 & 0.465 & 0.876 & 42.900 & 2.400 & 8.827 & 0.810 & -0.000 & 0.457 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 6 & 100 & 4.943 & 1.127 & 0.078 & 0.486 & 0.888 & 40.100 & 3.700 & 8.228 & 0.743 & 0.000 & 0.433 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 6 & 100 & 4.845 & 1.366 & 0.095 & 0.469 & 0.912 & 45.600 & 3.200 & 8.514 & 0.796 & -0.000 & 0.472 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 6 & 100 & 4.953 & 1.363 & 0.068 & 0.469 & 0.915 & 44.500 & 3.600 & 8.648 & 0.744 & -0.000 & 0.457 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 6 & 100 & 4.974 & 1.394 & 0.075 & 0.483 & 0.858 & 42.800 & 3.900 & 8.832 & 0.723 & 0.000 & 0.462 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 6 & 150 & 4.859 & 1.371 & 0.090 & 0.414 & 0.912 & 76.200 & 5.500 & 9.054 & 0.800 & -0.000 & 0.493 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 6 & 150 & 5.048 & 1.427 & 0.088 & 0.438 & 0.918 & 60.700 & 5.000 & 8.728 & 0.723 & 0.000 & 0.505 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 6 & 150 & 5.091 & 0.960 & 0.086 & 0.420 & 0.897 & 62.100 & 4.800 & 8.118 & 0.759 & 0.000 & 0.453 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 6 & 150 & 5.128 & 1.419 & 0.088 & 0.420 & 0.870 & 71.100 & 4.800 & 8.799 & 0.756 & 0.000 & 0.508 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 6 & 150 & 5.011 & 1.397 & 0.092 & 0.429 & 0.902 & 67.300 & 5.300 & 8.373 & 0.835 & 0.000 & 0.542 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 6 & 150 & 5.152 & 1.473 & 0.093 & 0.450 & 0.888 & 66.200 & 5.000 & 8.070 & 0.731 & 0.000 & 0.516 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 6 & 150 & 4.943 & 1.375 & 0.165 & 0.390 & 0.908 & 64.800 & 4.600 & 8.833 & 0.822 & 0.000 & 0.614 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 6 & 200 & 5.023 & 1.419 & 0.089 & 0.412 & 0.898 & 91.200 & 5.600 & 8.917 & 0.861 & 0.000 & 0.568 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 6 & 200 & 4.785 & 1.297 & 0.122 & 0.363 & 0.776 & 117.700 & 6.500 & 8.964 & 0.821 & 0.000 & 0.497 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 6 & 200 & 4.934 & 1.398 & 0.120 & 0.369 & 0.832 & 88.800 & 6.200 & 9.136 & 0.832 & -0.000 & 0.527 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 6 & 200 & 4.947 & 1.363 & 0.142 & 0.378 & 0.888 & 79.700 & 6.100 & 8.782 & 0.816 & 0.000 & 0.554 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 6 & 200 & 4.964 & 1.372 & 0.090 & 0.411 & 0.889 & 71.100 & 6.700 & 8.708 & 0.782 & 0.000 & 0.553 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 6 & 200 & 5.100 & 1.431 & 0.088 & 0.382 & 0.915 & 77.400 & 5.000 & 8.313 & 0.808 & -0.000 & 0.511 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 8 & 50 & 4.786 & 1.307 & 0.063 & 0.507 & 0.894 & 27.500 & 3.000 & 9.427 & 0.715 & -0.000 & 0.435 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 8 & 50 & 5.018 & 1.400 & 0.063 & 0.524 & 0.881 & 30.600 & 2.700 & 8.512 & 0.766 & 0.000 & 0.466 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 8 & 50 & 4.790 & 1.324 & 0.066 & 0.489 & 0.842 & 30.500 & 2.400 & 9.141 & 0.725 & -0.000 & 0.393 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 8 & 50 & 4.858 & 1.346 & 0.075 & 0.510 & 0.885 & 34.000 & 2.900 & 8.717 & 0.788 & 0.000 & 0.475 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 8 & 50 & 4.874 & 1.345 & 0.070 & 0.500 & 0.948 & 29.700 & 2.200 & 8.792 & 0.789 & 0.000 & 0.480 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 8 & 50 & 4.889 & 1.355 & 0.070 & 0.519 & 0.856 & 29.700 & 2.800 & 8.579 & 0.767 & 0.000 & 0.447 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 8 & 50 & 4.868 & 1.337 & 0.059 & 0.508 & 0.850 & 30.200 & 2.900 & 8.428 & 0.723 & 0.000 & 0.437 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 8 & 100 & 4.938 & 1.389 & 0.081 & 0.436 & 0.863 & 69.200 & 4.700 & 8.739 & 0.780 & 0.000 & 0.509 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 8 & 100 & 4.954 & 1.402 & 0.083 & 0.435 & 0.898 & 63.500 & 5.600 & 8.987 & 0.758 & -0.000 & 0.468 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 8 & 100 & 5.062 & 1.417 & 0.090 & 0.440 & 0.917 & 63.100 & 4.400 & 8.401 & 0.739 & -0.000 & 0.490 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 8 & 100 & 4.939 & 1.116 & 0.102 & 0.437 & 0.893 & 60.400 & 5.300 & 8.821 & 0.862 & 0.000 & 0.518 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 8 & 100 & 5.110 & 1.419 & 0.084 & 0.431 & 0.930 & 55.600 & 4.000 & 7.904 & 0.844 & 0.000 & 0.529 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 8 & 100 & 5.052 & 1.159 & 0.085 & 0.448 & 0.940 & 56.200 & 5.600 & 8.342 & 0.755 & 0.000 & 0.531 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 8 & 100 & 4.903 & 1.104 & 0.108 & 0.431 & 0.879 & 58.300 & 4.400 & 9.010 & 0.794 & 0.000 & 0.479 \\
\end{longtable}


\newpage

%%%% TABLE 4 - All other models
\begin{longtable}{lrrrrrrrrrrrrr}
\caption{Average metrics per BabyLM setting with min--max normalized aggregate (NormAvg) across metrics for remaining models.} \\
\toprule
\textbf{BabyLM} & \textbf{Turns} & \textbf{Length} & \textbf{AoA} & \textbf{CEFR} & \textbf{Overlap} & \textbf{TTR} & \textbf{Rep.} & \textbf{NumCon} & \textbf{AdversativeCon} & \textbf{Polysemy} & \textbf{VerbRep} & \textbf{Narrativity} & \textbf{NormAvg} \\
\midrule
\endfirsthead

\multicolumn{14}{c}%
{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\toprule
\textbf{BabyLM} & \textbf{Turns} & \textbf{Length} & \textbf{AoA} & \textbf{CEFR} & \textbf{Overlap} & \textbf{TTR} & \textbf{Rep.} & \textbf{NumCon} & \textbf{AdversativeCon} & \textbf{Polysemy} & \textbf{VerbRep} & \textbf{Narrativity} & \textbf{NormAvg} \\
\midrule
\endhead

\midrule \multicolumn{14}{r}{{Continued on next page}} \\
\endfoot

\bottomrule
\endlastfoot
cpo\_opt\_cosmos & 4 & 50 & 5.067 & 1.383 & 0.052 & 0.638 & 0.912 & 14.200 & 1.700 & 8.115 & 0.792 & -0.000 & 0.435 \\
mamba-sam-seqlen-2048-original & 4 & 50 & 4.770 & 1.353 & 0.048 & 0.609 & 0.945 & 15.700 & 1.700 & 9.280 & 0.828 & 0.000 & 0.494 \\
opt-sam-seqlen-2048-original & 4 & 50 & 4.843 & 1.318 & 0.052 & 0.618 & 0.942 & 17.000 & 1.900 & 8.893 & 0.866 & 0.000 & 0.506 \\
orpo\_opt\_cosmos & 4 & 50 & 5.200 & 1.459 & 0.067 & 0.624 & 0.822 & 10.300 & 1.500 & 7.632 & 0.645 & 0.000 & 0.407 \\
babylm-seqlen-opt-1024-warmup-v2 & 4 & 50 & 4.864 & 1.343 & 0.057 & 0.594 & 0.925 & 16.500 & 1.600 & 8.589 & 0.827 & 0.000 & 0.491 \\
babylm-seqlen-opt-4096-warmup-v2 & 4 & 50 & 4.487 & 1.172 & 0.030 & 0.449 & 0.867 & 17.100 & 1.000 & 8.662 & 0.677 & -0.000 & 0.290 \\
cpo\_opt\_cosmos & 4 & 100 & 5.196 & 1.458 & 0.075 & 0.540 & 0.876 & 25.100 & 1.500 & 8.216 & 0.796 & -0.000 & 0.461 \\
mamba-sam-seqlen-2048-original & 4 & 100 & 4.770 & 1.406 & 0.118 & 0.501 & 0.956 & 40.900 & 4.700 & 8.543 & 0.788 & -0.000 & 0.521 \\
opt-sam-seqlen-2048-original & 4 & 100 & 4.917 & 1.439 & 0.089 & 0.523 & 0.904 & 35.500 & 3.000 & 9.314 & 0.796 & -0.000 & 0.497 \\
orpo\_opt\_cosmos & 4 & 100 & 5.211 & 1.443 & 0.091 & 0.532 & 0.866 & 26.100 & 2.000 & 7.734 & 0.851 & -0.000 & 0.484 \\
babylm-seqlen-opt-1024-warmup-v2 & 4 & 100 & 4.878 & 1.342 & 0.110 & 0.493 & 0.847 & 38.800 & 3.300 & 9.587 & 0.867 & -0.000 & 0.503 \\
babylm-seqlen-opt-4096-warmup-v2 & 4 & 100 & 4.378 & 1.189 & 0.067 & 0.341 & 0.770 & 35.000 & 2.900 & 8.478 & 0.793 & -0.000 & 0.299 \\
cpo\_opt\_cosmos & 4 & 150 & 5.174 & 1.460 & 0.076 & 0.488 & 0.894 & 33.800 & 3.400 & 7.571 & 0.748 & 0.000 & 0.481 \\
mamba-sam-seqlen-2048-original & 4 & 150 & 4.918 & 1.435 & 0.075 & 0.470 & 0.906 & 55.800 & 5.500 & 9.043 & 0.816 & -0.000 & 0.520 \\
opt-sam-seqlen-2048-original & 4 & 150 & 4.998 & 1.416 & 0.117 & 0.466 & 0.913 & 45.500 & 1.800 & 9.115 & 0.789 & 0.000 & 0.541 \\
orpo\_opt\_cosmos & 4 & 150 & 5.284 & 1.489 & 0.102 & 0.507 & 0.847 & 27.000 & 1.500 & 8.097 & 0.797 & -0.000 & 0.488 \\
babylm-seqlen-opt-1024-warmup-v2 & 4 & 150 & 4.778 & 1.351 & 0.098 & 0.441 & 0.903 & 55.800 & 4.300 & 9.446 & 0.820 & -0.000 & 0.490 \\
babylm-seqlen-opt-4096-warmup-v2 & 4 & 150 & 4.473 & 1.222 & 0.032 & 0.355 & 0.900 & 50.300 & 3.200 & 9.304 & 0.779 & 0.000 & 0.383 \\
cpo\_opt\_cosmos & 4 & 200 & 5.191 & 1.270 & 0.130 & 0.435 & 0.933 & 50.800 & 3.500 & 8.165 & 0.868 & -0.000 & 0.510 \\
mamba-sam-seqlen-2048-original & 4 & 200 & 4.967 & 1.547 & 0.108 & 0.430 & 0.819 & 73.800 & 8.200 & 8.868 & 0.779 & 0.000 & 0.544 \\
opt-sam-seqlen-2048-original & 4 & 200 & 4.947 & 1.384 & 0.073 & 0.456 & 0.841 & 59.800 & 3.300 & 9.724 & 0.825 & 0.000 & 0.498 \\
orpo\_opt\_cosmos & 4 & 200 & 5.417 & 1.546 & 0.074 & 0.478 & 0.854 & 43.100 & 3.200 & 7.906 & 0.842 & -0.000 & 0.513 \\
babylm-seqlen-opt-1024-warmup-v2 & 4 & 200 & 5.010 & 1.410 & 0.072 & 0.436 & 0.952 & 75.800 & 4.400 & 9.447 & 0.804 & -0.000 & 0.537 \\
babylm-seqlen-opt-4096-warmup-v2 & 4 & 200 & 4.418 & 1.164 & 0.042 & 0.268 & 0.750 & 70.400 & 1.900 & 8.675 & 0.764 & 0.000 & 0.291 \\
cpo\_opt\_cosmos & 4 & 250 & 5.124 & 1.435 & 0.104 & 0.419 & 0.855 & 61.500 & 5.500 & 8.321 & 0.752 & -0.000 & 0.482 \\
mamba-sam-seqlen-2048-original & 4 & 250 & 4.836 & 1.413 & 0.100 & 0.411 & 0.869 & 100.300 & 10.300 & 9.417 & 0.858 & -0.000 & 0.576 \\
opt-sam-seqlen-2048-original & 4 & 250 & 4.997 & 1.439 & 0.116 & 0.401 & 0.907 & 71.200 & 5.900 & 8.697 & 0.834 & 0.000 & 0.567 \\
orpo\_opt\_cosmos & 4 & 250 & 5.386 & 1.497 & 0.120 & 0.436 & 0.844 & 47.600 & 3.000 & 7.614 & 0.824 & -0.000 & 0.503 \\
babylm-seqlen-opt-1024-warmup-v2 & 4 & 250 & 4.977 & 1.426 & 0.077 & 0.429 & 0.905 & 71.000 & 4.000 & 8.592 & 0.823 & 0.000 & 0.545 \\
babylm-seqlen-opt-4096-warmup-v2 & 4 & 250 & 4.549 & 1.223 & 0.070 & 0.266 & 0.922 & 79.400 & 3.300 & 9.127 & 0.816 & 0.000 & 0.447 \\
cpo\_opt\_cosmos & 6 & 50 & 5.123 & 1.457 & 0.049 & 0.560 & 0.912 & 20.300 & 2.100 & 7.358 & 0.745 & -0.000 & 0.432 \\
mamba-sam-seqlen-2048-original & 6 & 50 & 4.881 & 1.325 & 0.059 & 0.558 & 0.969 & 29.200 & 3.100 & 9.034 & 0.832 & -0.000 & 0.516 \\
opt-sam-seqlen-2048-original & 6 & 50 & 4.858 & 1.323 & 0.052 & 0.551 & 0.932 & 24.500 & 2.100 & 8.350 & 0.762 & -0.000 & 0.422 \\
orpo\_opt\_cosmos & 6 & 50 & 5.375 & 1.514 & 0.055 & 0.564 & 0.858 & 17.600 & 0.500 & 6.911 & 0.740 & -0.000 & 0.390 \\
babylm-seqlen-opt-1024-warmup-v2 & 6 & 50 & 4.864 & 1.339 & 0.038 & 0.543 & 0.901 & 25.300 & 2.500 & 8.834 & 0.774 & -0.000 & 0.423 \\
babylm-seqlen-opt-4096-warmup-v2 & 6 & 50 & 4.478 & 1.197 & 0.029 & 0.408 & 0.803 & 22.100 & 1.300 & 8.928 & 0.643 & -0.000 & 0.239 \\
cpo\_opt\_cosmos & 6 & 100 & 5.075 & 1.395 & 0.116 & 0.465 & 0.904 & 43.300 & 4.000 & 8.329 & 0.887 & -0.000 & 0.548 \\
mamba-sam-seqlen-2048-original & 6 & 100 & 4.838 & 1.429 & 0.105 & 0.474 & 0.840 & 59.100 & 5.600 & 9.590 & 0.811 & -0.000 & 0.506 \\
opt-sam-seqlen-2048-original & 6 & 100 & 4.861 & 1.384 & 0.071 & 0.465 & 0.838 & 52.600 & 4.700 & 9.464 & 0.822 & 0.000 & 0.503 \\
orpo\_opt\_cosmos & 6 & 100 & 5.155 & 1.512 & 0.111 & 0.509 & 0.917 & 38.800 & 2.700 & 7.380 & 0.818 & 0.000 & 0.545 \\
babylm-seqlen-opt-1024-warmup-v2 & 6 & 100 & 4.895 & 1.365 & 0.080 & 0.467 & 0.955 & 55.600 & 2.300 & 10.311 & 0.825 & 0.000 & 0.568 \\
babylm-seqlen-opt-4096-warmup-v2 & 6 & 100 & 4.709 & 1.256 & 0.049 & 0.317 & 0.842 & 48.900 & 2.800 & 8.554 & 0.710 & -0.000 & 0.332 \\
babylm-seqlen-opt-1024-warmup-v2 & 6 & 150 & 5.060 & 1.429 & 0.076 & 0.439 & 0.858 & 66.000 & 4.600 & 8.523 & 0.724 & 0.000 & 0.482 \\
babylm-seqlen-opt-4096-warmup-v2 & 6 & 150 & 4.537 & 1.213 & 0.063 & 0.266 & 0.890 & 89.300 & 3.700 & 8.916 & 0.802 & -0.000 & 0.397 \\
babylm-seqlen-opt-1024-warmup-v2 & 6 & 200 & 4.897 & 1.397 & 0.110 & 0.376 & 0.946 & 100.700 & 6.800 & 9.551 & 0.816 & 0.000 & 0.597 \\
babylm-seqlen-opt-4096-warmup-v2 & 6 & 200 & 4.402 & 1.181 & 0.047 & 0.227 & 0.870 & 113.300 & 3.100 & 9.030 & 0.773 & 0.000 & 0.376 \\
babylm-seqlen-opt-4096-warmup-v2 & 6 & 250 & 4.298 & 1.118 & 0.070 & 0.168 & 0.780 & 182.400 & 2.700 & 9.331 & 0.820 & 0.000 & 0.373 \\
babylm-seqlen-opt-1024-warmup-v2 & 8 & 50 & 4.845 & 1.344 & 0.063 & 0.504 & 0.937 & 33.400 & 3.000 & 9.526 & 0.782 & 0.000 & 0.502 \\
babylm-seqlen-opt-4096-warmup-v2 & 8 & 50 & 4.458 & 1.170 & 0.036 & 0.337 & 0.897 & 38.300 & 1.300 & 8.458 & 0.663 & 0.000 & 0.292 \\
babylm-seqlen-opt-1024-warmup-v2 & 8 & 100 & 5.002 & 1.432 & 0.084 & 0.447 & 0.829 & 59.200 & 4.600 & 8.566 & 0.799 & 0.000 & 0.486 \\
babylm-seqlen-opt-4096-warmup-v2 & 8 & 100 & 4.485 & 1.215 & 0.066 & 0.279 & 0.914 & 70.000 & 2.900 & 8.584 & 0.766 & -0.000 & 0.371 \\
babylm-seqlen-opt-4096-warmup-v2 & 8 & 150 & 4.505 & 1.218 & 0.036 & 0.251 & 0.856 & 100.000 & 2.500 & 8.419 & 0.828 & -0.000 & 0.334 \\
babylm-seqlen-opt-4096-warmup-v2 & 8 & 200 & 4.446 & 1.166 & 0.114 & 0.183 & 0.841 & 154.400 & 3.300 & 8.978 & 0.781 & 0.000 & 0.416 \\
babylm-seqlen-opt-4096-warmup-v2 & 8 & 250 & 4.531 & 1.193 & 0.063 & 0.171 & 0.715 & 162.200 & 4.800 & 8.916 & 0.751 & -0.000 & 0.307 \\

\end{longtable}

% \begin{longtable}{lrrrrrrrrrrrrr}
% \caption{Average metrics per BabyLM setting with min--max normalized aggregate (NormAvg) across metrics.} \\
% \toprule
% \textbf{BabyLM} & \textbf{Turns} & \textbf{Length} & \textbf{AoA} & \textbf{CEFR} & \textbf{Overlap} & \textbf{TTR} & \textbf{Rep.} & \textbf{NumCon} & \textbf{AdversativeCon} & \textbf{Polysemy} & \textbf{VerbRep} & \textbf{Narrativity} & \textbf{NormAvg} \\
% \midrule
% \endfirsthead

% \multicolumn{14}{c}%
% {{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
% \toprule
% \textbf{BabyLM} & \textbf{Turns} & \textbf{Length} & \textbf{AoA} & \textbf{CEFR} & \textbf{Overlap} & \textbf{TTR} & \textbf{Rep.} & \textbf{NumCon} & \textbf{AdversativeCon} & \textbf{Polysemy} & \textbf{VerbRep} & \textbf{Narrativity} & \textbf{NormAvg} \\
% \midrule
% \endhead

% \midrule \multicolumn{14}{r}{{Continued on next page}} \\
% \endfoot

% \bottomrule
% \endlastfoot

% cpo\_opt\_100M\_2048\_preprocess & 4 & 50 & 5.087 & 1.373 & 0.068 & 0.620 & 0.851 & 13.300 & 0.900 & 7.772 & 0.772 & 0.000 & 0.436 \\
% cpo\_opt\_base & 4 & 50 & 5.214 & 1.468 & 0.074 & 0.590 & 0.881 & 13.100 & 0.900 & 7.241 & 0.684 & 0.000 & 0.425 \\
% cpo\_opt\_cosmos & 4 & 50 & 5.067 & 1.383 & 0.052 & 0.638 & 0.912 & 14.200 & 1.700 & 8.115 & 0.792 & -0.000 & 0.435 \\
% cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 50 & 5.011 & 1.408 & 0.044 & 0.624 & 0.946 & 15.600 & 1.600 & 8.118 & 0.790 & 0.000 & 0.496 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 4 & 50 & 4.813 & 1.325 & 0.044 & 0.627 & 0.803 & 16.100 & 1.300 & 9.121 & 0.622 & 0.000 & 0.386 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 4 & 50 & 4.802 & 1.371 & 0.053 & 0.610 & 0.870 & 16.500 & 1.600 & 8.488 & 0.773 & 0.000 & 0.454 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 4 & 50 & 4.782 & 1.305 & 0.082 & 0.606 & 0.904 & 13.600 & 1.500 & 8.769 & 0.822 & -0.000 & 0.469 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 4 & 50 & 4.951 & 1.328 & 0.062 & 0.599 & 0.887 & 13.400 & 1.300 & 7.826 & 0.759 & 0.000 & 0.465 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 4 & 50 & 4.819 & 1.328 & 0.056 & 0.572 & 0.909 & 13.800 & 1.300 & 8.635 & 0.863 & -0.000 & 0.465 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 4 & 50 & 4.948 & 1.331 & 0.062 & 0.620 & 0.942 & 14.400 & 1.000 & 8.725 & 0.750 & -0.000 & 0.458 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 4 & 50 & 4.929 & 1.322 & 0.063 & 0.596 & 0.867 & 15.000 & 1.700 & 7.667 & 0.666 & 0.000 & 0.399 \\
% cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 50 & 4.523 & 1.219 & 0.046 & 0.464 & 0.797 & 18.100 & 1.600 & 9.379 & 0.753 & 0.000 & 0.389 \\
% mamba-sam-seqlen-2048-original & 4 & 50 & 4.770 & 1.353 & 0.048 & 0.609 & 0.945 & 15.700 & 1.700 & 9.280 & 0.828 & 0.000 & 0.494 \\
% opt-sam-orpo-mamba-2048-step448 & 4 & 50 & 4.887 & 1.376 & 0.072 & 0.617 & 0.918 & 16.800 & 1.900 & 8.294 & 0.797 & 0.000 & 0.513 \\
% opt-sam-orpo-seqlen-2048-step559 & 4 & 50 & 4.948 & 1.365 & 0.052 & 0.615 & 0.866 & 15.100 & 1.400 & 8.926 & 0.590 & 0.000 & 0.390 \\
% opt-sam-seqlen-2048-original & 4 & 50 & 4.843 & 1.318 & 0.052 & 0.618 & 0.942 & 17.000 & 1.900 & 8.893 & 0.866 & 0.000 & 0.506 \\
% orpo\_opt\_100M\_2048\_preprocess & 4 & 50 & 5.123 & 1.415 & 0.078 & 0.582 & 0.777 & 14.300 & 1.100 & 7.963 & 0.814 & 0.000 & 0.440 \\
% orpo\_opt\_cosmos & 4 & 50 & 5.200 & 1.459 & 0.067 & 0.624 & 0.822 & 10.300 & 1.500 & 7.632 & 0.645 & 0.000 & 0.407 \\
% orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 50 & 4.813 & 1.343 & 0.066 & 0.604 & 0.898 & 17.900 & 1.700 & 8.916 & 0.763 & 0.000 & 0.459 \\
% orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 50 & 4.487 & 1.228 & 0.075 & 0.473 & 0.879 & 11.500 & 1.400 & 8.631 & 0.720 & -0.000 & 0.346 \\
% babylm-seqlen-opt-1024-warmup-v2 & 4 & 50 & 4.864 & 1.343 & 0.057 & 0.594 & 0.925 & 16.500 & 1.600 & 8.589 & 0.827 & 0.000 & 0.491 \\
% babylm-seqlen-opt-4096-warmup-v2 & 4 & 50 & 4.487 & 1.172 & 0.030 & 0.449 & 0.867 & 17.100 & 1.000 & 8.662 & 0.677 & -0.000 & 0.290 \\
% cpo\_opt\_100M\_2048\_preprocess & 4 & 100 & 5.028 & 1.417 & 0.121 & 0.508 & 0.931 & 23.400 & 2.300 & 7.776 & 0.857 & 0.000 & 0.529 \\
% cpo\_opt\_base & 4 & 100 & 5.075 & 1.404 & 0.088 & 0.496 & 0.847 & 21.000 & 1.300 & 8.294 & 0.715 & 0.000 & 0.431 \\
% cpo\_opt\_cosmos & 4 & 100 & 5.196 & 1.458 & 0.075 & 0.540 & 0.876 & 25.100 & 1.500 & 8.216 & 0.796 & -0.000 & 0.461 \\
% cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 100 & 4.921 & 1.353 & 0.062 & 0.537 & 0.955 & 35.900 & 3.300 & 9.218 & 0.839 & -0.000 & 0.521 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 4 & 100 & 4.974 & 1.391 & 0.069 & 0.548 & 0.879 & 29.800 & 2.800 & 8.771 & 0.791 & 0.000 & 0.481 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 4 & 100 & 4.888 & 1.374 & 0.082 & 0.523 & 0.817 & 31.700 & 2.100 & 8.968 & 0.717 & 0.000 & 0.427 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 4 & 100 & 4.900 & 1.365 & 0.083 & 0.522 & 0.903 & 33.600 & 4.200 & 9.265 & 0.825 & 0.000 & 0.543 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 4 & 100 & 4.934 & 1.350 & 0.045 & 0.526 & 0.906 & 26.400 & 2.000 & 8.090 & 0.876 & 0.000 & 0.479 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 4 & 100 & 4.984 & 1.395 & 0.063 & 0.524 & 0.905 & 25.700 & 2.600 & 8.415 & 0.826 & -0.000 & 0.475 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 4 & 100 & 4.954 & 1.367 & 0.076 & 0.513 & 0.844 & 21.900 & 2.000 & 8.098 & 0.671 & 0.000 & 0.413 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 4 & 100 & 4.847 & 1.353 & 0.092 & 0.513 & 0.884 & 27.400 & 2.100 & 8.416 & 0.752 & 0.000 & 0.459 \\
% cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 100 & 4.532 & 1.224 & 0.058 & 0.391 & 0.891 & 33.300 & 3.000 & 9.435 & 0.821 & 0.000 & 0.419 \\
% mamba-sam-seqlen-2048-original & 4 & 100 & 4.770 & 1.406 & 0.118 & 0.501 & 0.956 & 40.900 & 4.700 & 8.543 & 0.788 & -0.000 & 0.521 \\
% opt-sam-orpo-mamba-2048-step448 & 4 & 100 & 4.797 & 1.390 & 0.099 & 0.514 & 0.799 & 42.100 & 5.400 & 9.338 & 0.870 & -0.000 & 0.517 \\
% opt-sam-orpo-seqlen-2048-step559 & 4 & 100 & 4.728 & 1.304 & 0.077 & 0.512 & 0.893 & 40.100 & 3.800 & 9.944 & 0.844 & -0.000 & 0.476 \\
% opt-sam-seqlen-2048-original & 4 & 100 & 4.917 & 1.439 & 0.089 & 0.523 & 0.904 & 35.500 & 3.000 & 9.314 & 0.796 & -0.000 & 0.497 \\
% orpo\_opt\_100M\_2048\_preprocess & 4 & 100 & 5.021 & 1.419 & 0.085 & 0.524 & 0.862 & 20.300 & 0.800 & 8.210 & 0.851 & 0.000 & 0.483 \\
% orpo\_opt\_cosmos & 4 & 100 & 5.211 & 1.443 & 0.091 & 0.532 & 0.866 & 26.100 & 2.000 & 7.734 & 0.851 & -0.000 & 0.484 \\
% orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 100 & 4.953 & 1.365 & 0.068 & 0.534 & 0.909 & 35.200 & 3.300 & 8.949 & 0.778 & -0.000 & 0.485 \\
% orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 100 & 4.711 & 1.262 & 0.062 & 0.419 & 0.870 & 19.600 & 1.400 & 8.710 & 0.768 & -0.000 & 0.373 \\
% babylm-seqlen-opt-1024-warmup-v2 & 4 & 100 & 4.878 & 1.342 & 0.110 & 0.493 & 0.847 & 38.800 & 3.300 & 9.587 & 0.867 & -0.000 & 0.503 \\
% babylm-seqlen-opt-4096-warmup-v2 & 4 & 100 & 4.378 & 1.189 & 0.067 & 0.341 & 0.770 & 35.000 & 2.900 & 8.478 & 0.793 & -0.000 & 0.299 \\
% cpo\_opt\_100M\_2048\_preprocess & 4 & 150 & 5.057 & 1.441 & 0.115 & 0.469 & 0.828 & 33.400 & 1.200 & 7.582 & 0.708 & -0.000 & 0.416 \\
% cpo\_opt\_base & 4 & 150 & 5.153 & 1.433 & 0.082 & 0.458 & 0.883 & 34.500 & 1.700 & 8.358 & 0.837 & -0.000 & 0.470 \\
% cpo\_opt\_cosmos & 4 & 150 & 5.174 & 1.460 & 0.076 & 0.488 & 0.894 & 33.800 & 3.400 & 7.571 & 0.748 & 0.000 & 0.481 \\
% cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 150 & 4.912 & 1.360 & 0.104 & 0.445 & 0.959 & 52.600 & 5.000 & 9.865 & 0.852 & 0.000 & 0.584 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 4 & 150 & 4.893 & 1.360 & 0.092 & 0.469 & 0.896 & 43.200 & 3.200 & 9.341 & 0.819 & 0.000 & 0.522 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 4 & 150 & 4.923 & 1.418 & 0.105 & 0.467 & 0.936 & 45.100 & 3.000 & 9.136 & 0.847 & 0.000 & 0.600 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 4 & 150 & 4.949 & 1.353 & 0.109 & 0.439 & 0.901 & 40.200 & 3.700 & 8.797 & 0.768 & 0.000 & 0.494 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 4 & 150 & 5.055 & 1.350 & 0.083 & 0.448 & 0.889 & 33.300 & 2.600 & 8.742 & 0.717 & -0.000 & 0.400 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 4 & 150 & 4.989 & 1.379 & 0.114 & 0.443 & 0.870 & 34.600 & 2.100 & 8.785 & 0.765 & 0.000 & 0.476 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 4 & 150 & 4.983 & 1.375 & 0.081 & 0.499 & 0.894 & 35.000 & 1.900 & 8.627 & 0.716 & 0.000 & 0.449 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 4 & 150 & 4.901 & 1.380 & 0.070 & 0.470 & 0.862 & 40.900 & 3.600 & 8.410 & 0.760 & -0.000 & 0.427 \\
% cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 150 & 4.385 & 1.256 & 0.128 & 0.302 & 0.749 & 49.200 & 3.600 & 9.345 & 0.775 & 0.000 & 0.413 \\
% mamba-sam-seqlen-2048-original & 4 & 150 & 4.918 & 1.435 & 0.075 & 0.470 & 0.906 & 55.800 & 5.500 & 9.043 & 0.816 & -0.000 & 0.520 \\
% opt-sam-orpo-mamba-2048-step448 & 4 & 150 & 4.880 & 1.384 & 0.073 & 0.470 & 0.870 & 64.800 & 7.600 & 9.414 & 0.783 & -0.000 & 0.519 \\
% opt-sam-orpo-seqlen-2048-step559 & 4 & 150 & 4.910 & 1.371 & 0.069 & 0.473 & 0.921 & 47.300 & 3.500 & 8.704 & 0.787 & -0.000 & 0.482 \\
% opt-sam-seqlen-2048-original & 4 & 150 & 4.998 & 1.416 & 0.117 & 0.466 & 0.913 & 45.500 & 1.800 & 9.115 & 0.789 & 0.000 & 0.541 \\
% orpo\_opt\_100M\_2048\_preprocess & 4 & 150 & 5.169 & 1.432 & 0.109 & 0.473 & 0.766 & 33.300 & 1.600 & 8.092 & 0.722 & 0.000 & 0.441 \\
% orpo\_opt\_cosmos & 4 & 150 & 5.284 & 1.489 & 0.102 & 0.507 & 0.847 & 27.000 & 1.500 & 8.097 & 0.797 & -0.000 & 0.488 \\
% orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 150 & 5.077 & 1.395 & 0.076 & 0.474 & 0.825 & 69.600 & 4.500 & 8.858 & 0.815 & -0.000 & 0.470 \\
% orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 150 & 4.732 & 1.301 & 0.078 & 0.391 & 0.855 & 37.700 & 2.500 & 8.890 & 0.724 & -0.000 & 0.391 \\
% babylm-seqlen-opt-1024-warmup-v2 & 4 & 150 & 4.778 & 1.351 & 0.098 & 0.441 & 0.903 & 55.800 & 4.300 & 9.446 & 0.820 & -0.000 & 0.490 \\
% babylm-seqlen-opt-4096-warmup-v2 & 4 & 150 & 4.473 & 1.222 & 0.032 & 0.355 & 0.900 & 50.300 & 3.200 & 9.304 & 0.779 & 0.000 & 0.383 \\
% cpo\_opt\_100M\_2048\_preprocess & 4 & 200 & 5.171 & 0.932 & 0.108 & 0.432 & 0.904 & 40.300 & 3.100 & 8.410 & 0.767 & -0.000 & 0.420 \\
% cpo\_opt\_base & 4 & 200 & 5.378 & 1.506 & 0.099 & 0.433 & 0.882 & 41.500 & 0.900 & 7.803 & 0.738 & -0.000 & 0.457 \\
% cpo\_opt\_cosmos & 4 & 200 & 5.191 & 1.270 & 0.130 & 0.435 & 0.933 & 50.800 & 3.500 & 8.165 & 0.868 & -0.000 & 0.510 \\
% cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 200 & 4.960 & 1.394 & 0.105 & 0.427 & 0.891 & 67.500 & 4.300 & 9.388 & 0.823 & -0.000 & 0.521 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 4 & 200 & 4.827 & 1.345 & 0.113 & 0.430 & 0.946 & 59.900 & 5.300 & 9.482 & 0.862 & -0.000 & 0.558 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 4 & 200 & 4.952 & 1.391 & 0.061 & 0.419 & 0.874 & 58.100 & 3.200 & 9.061 & 0.795 & 0.000 & 0.492 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 4 & 200 & 5.184 & 1.474 & 0.115 & 0.434 & 0.873 & 60.400 & 3.500 & 8.268 & 0.800 & -0.000 & 0.508 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 4 & 200 & 4.899 & 1.337 & 0.071 & 0.469 & 0.872 & 44.300 & 3.200 & 8.790 & 0.730 & -0.000 & 0.420 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 4 & 200 & 5.025 & 1.387 & 0.093 & 0.441 & 0.904 & 50.500 & 3.700 & 8.466 & 0.833 & -0.000 & 0.510 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 4 & 200 & 5.006 & 1.444 & 0.068 & 0.454 & 0.887 & 43.300 & 3.200 & 7.894 & 0.706 & -0.000 & 0.400 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 4 & 200 & 5.163 & 1.257 & 0.083 & 0.453 & 0.875 & 50.100 & 4.400 & 7.789 & 0.786 & 0.000 & 0.463 \\
% cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 200 & 4.367 & 1.188 & 0.082 & 0.245 & 0.770 & 102.700 & 3.000 & 9.584 & 0.875 & -0.000 & 0.369 \\
% mamba-sam-seqlen-2048-original & 4 & 200 & 4.967 & 1.547 & 0.108 & 0.430 & 0.819 & 73.800 & 8.200 & 8.868 & 0.779 & 0.000 & 0.544 \\
% opt-sam-orpo-mamba-2048-step448 & 4 & 200 & 5.049 & 1.435 & 0.095 & 0.438 & 0.853 & 76.100 & 7.200 & 9.044 & 0.839 & 0.000 & 0.577 \\
% opt-sam-orpo-seqlen-2048-step559 & 4 & 200 & 4.825 & 1.152 & 0.090 & 0.456 & 0.829 & 62.500 & 5.100 & 9.511 & 0.872 & 0.000 & 0.513 \\
% opt-sam-seqlen-2048-original & 4 & 200 & 4.947 & 1.384 & 0.073 & 0.456 & 0.841 & 59.800 & 3.300 & 9.724 & 0.825 & 0.000 & 0.498 \\
% orpo\_opt\_100M\_2048\_preprocess & 4 & 200 & 5.080 & 1.198 & 0.100 & 0.463 & 0.928 & 39.000 & 3.600 & 8.636 & 0.797 & -0.000 & 0.490 \\
% orpo\_opt\_cosmos & 4 & 200 & 5.417 & 1.546 & 0.074 & 0.478 & 0.854 & 43.100 & 3.200 & 7.906 & 0.842 & -0.000 & 0.513 \\
% orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 200 & 5.047 & 0.888 & 0.094 & 0.438 & 0.948 & 71.000 & 4.000 & 8.855 & 0.854 & -0.000 & 0.473 \\
% orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 200 & 4.533 & 1.340 & 0.122 & 0.306 & 0.808 & 65.100 & 2.600 & 8.758 & 0.788 & 0.000 & 0.423 \\
% babylm-seqlen-opt-1024-warmup-v2 & 4 & 200 & 5.010 & 1.410 & 0.072 & 0.436 & 0.952 & 75.800 & 4.400 & 9.447 & 0.804 & -0.000 & 0.537 \\
% babylm-seqlen-opt-4096-warmup-v2 & 4 & 200 & 4.418 & 1.164 & 0.042 & 0.268 & 0.750 & 70.400 & 1.900 & 8.675 & 0.764 & 0.000 & 0.291 \\
% cpo\_opt\_100M\_2048\_preprocess & 4 & 250 & 5.054 & 1.393 & 0.125 & 0.396 & 0.950 & 57.700 & 2.500 & 8.453 & 0.827 & 0.000 & 0.547 \\
% cpo\_opt\_base & 4 & 250 & 5.655 & 1.647 & 0.108 & 0.411 & 0.835 & 47.300 & 3.000 & 7.798 & 0.780 & -0.000 & 0.524 \\
% cpo\_opt\_cosmos & 4 & 250 & 5.124 & 1.435 & 0.104 & 0.419 & 0.855 & 61.500 & 5.500 & 8.321 & 0.752 & -0.000 & 0.482 \\
% cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 250 & 4.932 & 1.391 & 0.103 & 0.411 & 0.819 & 80.200 & 7.300 & 9.086 & 0.855 & 0.000 & 0.550 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 4 & 250 & 5.149 & 1.467 & 0.104 & 0.399 & 0.910 & 60.400 & 2.900 & 8.551 & 0.805 & -0.000 & 0.509 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 4 & 250 & 4.927 & 1.378 & 0.099 & 0.396 & 0.840 & 55.800 & 5.800 & 9.602 & 0.653 & 0.000 & 0.475 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 4 & 250 & 4.898 & 1.375 & 0.140 & 0.409 & 0.805 & 60.800 & 4.900 & 9.658 & 0.855 & 0.000 & 0.541 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 4 & 250 & 5.029 & 1.427 & 0.092 & 0.387 & 0.887 & 66.900 & 5.800 & 8.251 & 0.719 & -0.000 & 0.472 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 4 & 250 & 5.183 & 1.434 & 0.095 & 0.419 & 0.838 & 59.000 & 3.100 & 8.245 & 0.761 & 0.000 & 0.499 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 4 & 250 & 5.007 & 1.391 & 0.101 & 0.409 & 0.839 & 48.600 & 3.600 & 8.467 & 0.727 & 0.000 & 0.467 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 4 & 250 & 5.016 & 0.910 & 0.155 & 0.370 & 0.911 & 68.100 & 4.700 & 8.382 & 0.860 & 0.000 & 0.514 \\
% cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 250 & 4.632 & 1.245 & 0.094 & 0.286 & 0.891 & 78.300 & 2.500 & 9.265 & 0.794 & 0.000 & 0.443 \\
% mamba-sam-seqlen-2048-original & 4 & 250 & 4.836 & 1.413 & 0.100 & 0.411 & 0.869 & 100.300 & 10.300 & 9.417 & 0.858 & -0.000 & 0.576 \\
% opt-sam-orpo-mamba-2048-step448 & 4 & 250 & 4.777 & 1.140 & 0.126 & 0.388 & 0.778 & 108.300 & 12.200 & 8.808 & 0.877 & -0.000 & 0.525 \\
% opt-sam-orpo-seqlen-2048-step559 & 4 & 250 & 5.091 & 1.454 & 0.092 & 0.407 & 0.861 & 67.500 & 5.600 & 8.867 & 0.791 & -0.000 & 0.518 \\
% opt-sam-seqlen-2048-original & 4 & 250 & 4.997 & 1.439 & 0.116 & 0.401 & 0.907 & 71.200 & 5.900 & 8.697 & 0.834 & 0.000 & 0.567 \\
% orpo\_opt\_100M\_2048\_preprocess & 4 & 250 & 5.160 & 1.247 & 0.101 & 0.424 & 0.897 & 47.700 & 4.100 & 8.531 & 0.830 & 0.000 & 0.525 \\
% orpo\_opt\_cosmos & 4 & 250 & 5.386 & 1.497 & 0.120 & 0.436 & 0.844 & 47.600 & 3.000 & 7.614 & 0.824 & -0.000 & 0.503 \\
% orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 250 & 5.073 & 1.197 & 0.096 & 0.412 & 0.888 & 90.700 & 8.200 & 9.247 & 0.846 & 0.000 & 0.567 \\
% orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 250 & 4.741 & 1.391 & 0.117 & 0.318 & 0.810 & 49.500 & 3.900 & 7.859 & 0.794 & -0.000 & 0.395 \\
% babylm-seqlen-opt-1024-warmup-v2 & 4 & 250 & 4.977 & 1.426 & 0.077 & 0.429 & 0.905 & 71.000 & 4.000 & 8.592 & 0.823 & 0.000 & 0.545 \\
% babylm-seqlen-opt-4096-warmup-v2 & 4 & 250 & 4.549 & 1.223 & 0.070 & 0.266 & 0.922 & 79.400 & 3.300 & 9.127 & 0.816 & 0.000 & 0.447 \\
% cpo\_opt\_100M\_2048\_preprocess & 6 & 50 & 5.071 & 1.423 & 0.065 & 0.564 & 0.830 & 19.000 & 2.500 & 8.146 & 0.740 & 0.000 & 0.434 \\
% cpo\_opt\_base & 6 & 50 & 5.022 & 1.355 & 0.057 & 0.549 & 0.891 & 18.400 & 1.800 & 8.236 & 0.766 & -0.000 & 0.432 \\
% cpo\_opt\_cosmos & 6 & 50 & 5.123 & 1.457 & 0.049 & 0.560 & 0.912 & 20.300 & 2.100 & 7.358 & 0.745 & -0.000 & 0.432 \\
% cpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 50 & 4.947 & 1.405 & 0.050 & 0.563 & 0.911 & 25.900 & 1.800 & 8.552 & 0.745 & 0.000 & 0.461 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 6 & 50 & 4.898 & 1.350 & 0.050 & 0.554 & 0.915 & 23.400 & 2.600 & 8.527 & 0.796 & 0.000 & 0.491 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 6 & 50 & 4.812 & 1.341 & 0.067 & 0.543 & 0.922 & 25.200 & 1.200 & 9.002 & 0.845 & 0.000 & 0.514 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 6 & 50 & 4.812 & 1.337 & 0.083 & 0.531 & 0.893 & 20.300 & 1.100 & 8.223 & 0.722 & 0.000 & 0.429 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 6 & 50 & 4.882 & 1.339 & 0.057 & 0.536 & 0.938 & 22.700 & 2.400 & 9.117 & 0.678 & 0.000 & 0.444 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 6 & 50 & 4.886 & 1.333 & 0.064 & 0.528 & 0.929 & 22.600 & 2.100 & 8.392 & 0.800 & 0.000 & 0.463 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 6 & 50 & 4.846 & 1.331 & 0.036 & 0.557 & 0.916 & 21.300 & 1.700 & 8.521 & 0.740 & 0.000 & 0.428 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 6 & 50 & 4.982 & 1.373 & 0.069 & 0.541 & 0.853 & 23.000 & 2.000 & 7.914 & 0.754 & -0.000 & 0.402 \\
% cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 50 & 4.525 & 1.231 & 0.094 & 0.411 & 0.921 & 22.500 & 1.600 & 8.597 & 0.787 & -0.000 & 0.387 \\
% mamba-sam-seqlen-2048-original & 6 & 50 & 4.881 & 1.325 & 0.059 & 0.558 & 0.969 & 29.200 & 3.100 & 9.034 & 0.832 & -0.000 & 0.516 \\
% opt-sam-orpo-mamba-2048-step448 & 6 & 50 & 4.831 & 1.369 & 0.084 & 0.553 & 0.912 & 24.200 & 3.500 & 9.184 & 0.758 & 0.000 & 0.505 \\
% opt-sam-orpo-seqlen-2048-step559 & 6 & 50 & 5.072 & 1.382 & 0.055 & 0.576 & 0.868 & 25.400 & 2.300 & 9.109 & 0.778 & 0.000 & 0.514 \\
% opt-sam-seqlen-2048-original & 6 & 50 & 4.858 & 1.323 & 0.052 & 0.551 & 0.932 & 24.500 & 2.100 & 8.350 & 0.762 & -0.000 & 0.422 \\
% orpo\_opt\_100M\_2048\_preprocess & 6 & 50 & 5.145 & 1.411 & 0.082 & 0.546 & 0.865 & 18.400 & 0.700 & 7.507 & 0.817 & 0.000 & 0.462 \\
% orpo\_opt\_cosmos & 6 & 50 & 5.375 & 1.514 & 0.055 & 0.564 & 0.858 & 17.600 & 0.500 & 6.911 & 0.740 & -0.000 & 0.390 \\
% orpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 50 & 4.951 & 1.390 & 0.065 & 0.567 & 0.927 & 26.100 & 2.400 & 8.366 & 0.744 & -0.000 & 0.449 \\
% orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 50 & 4.612 & 1.234 & 0.061 & 0.419 & 0.907 & 19.000 & 2.000 & 9.567 & 0.793 & -0.000 & 0.401 \\
% babylm-seqlen-opt-1024-warmup-v2 & 6 & 50 & 4.864 & 1.339 & 0.038 & 0.543 & 0.901 & 25.300 & 2.500 & 8.834 & 0.774 & -0.000 & 0.423 \\
% babylm-seqlen-opt-4096-warmup-v2 & 6 & 50 & 4.478 & 1.197 & 0.029 & 0.408 & 0.803 & 22.100 & 1.300 & 8.928 & 0.643 & -0.000 & 0.239 \\
% cpo\_opt\_100M\_2048\_preprocess & 6 & 100 & 5.093 & 1.437 & 0.090 & 0.483 & 0.858 & 36.100 & 1.600 & 8.253 & 0.776 & 0.000 & 0.493 \\
% cpo\_opt\_base & 6 & 100 & 5.035 & 1.429 & 0.080 & 0.489 & 0.892 & 38.500 & 2.500 & 8.295 & 0.780 & -0.000 & 0.472 \\
% cpo\_opt\_cosmos & 6 & 100 & 5.075 & 1.395 & 0.116 & 0.465 & 0.904 & 43.300 & 4.000 & 8.329 & 0.887 & -0.000 & 0.548 \\
% cpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 100 & 4.904 & 1.364 & 0.094 & 0.456 & 0.932 & 55.000 & 5.000 & 9.643 & 0.883 & 0.000 & 0.583 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 6 & 100 & 4.843 & 1.325 & 0.099 & 0.453 & 0.901 & 51.400 & 3.500 & 9.253 & 0.783 & 0.000 & 0.497 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 6 & 100 & 4.805 & 1.323 & 0.092 & 0.460 & 0.892 & 49.000 & 4.000 & 9.001 & 0.787 & 0.000 & 0.500 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 6 & 100 & 4.916 & 1.107 & 0.112 & 0.465 & 0.876 & 42.900 & 2.400 & 8.827 & 0.810 & -0.000 & 0.457 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 6 & 100 & 4.943 & 1.127 & 0.078 & 0.486 & 0.888 & 40.100 & 3.700 & 8.228 & 0.743 & 0.000 & 0.433 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 6 & 100 & 4.845 & 1.366 & 0.095 & 0.469 & 0.912 & 45.600 & 3.200 & 8.514 & 0.796 & -0.000 & 0.472 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 6 & 100 & 4.953 & 1.363 & 0.068 & 0.469 & 0.915 & 44.500 & 3.600 & 8.648 & 0.744 & -0.000 & 0.457 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 6 & 100 & 4.974 & 1.394 & 0.075 & 0.483 & 0.858 & 42.800 & 3.900 & 8.832 & 0.723 & 0.000 & 0.462 \\
% cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 100 & 4.430 & 1.320 & 0.129 & 0.299 & 0.764 & 55.700 & 3.000 & 8.628 & 0.791 & 0.000 & 0.392 \\
% mamba-sam-seqlen-2048-original & 6 & 100 & 4.838 & 1.429 & 0.105 & 0.474 & 0.840 & 59.100 & 5.600 & 9.590 & 0.811 & -0.000 & 0.506 \\
% opt-sam-orpo-mamba-2048-step448 & 6 & 100 & 4.959 & 1.411 & 0.066 & 0.478 & 0.962 & 60.700 & 6.500 & 8.757 & 0.757 & -0.000 & 0.516 \\
% opt-sam-orpo-seqlen-2048-step559 & 6 & 100 & 4.912 & 1.352 & 0.080 & 0.508 & 0.944 & 44.600 & 3.800 & 8.853 & 0.841 & -0.000 & 0.517 \\
% opt-sam-seqlen-2048-original & 6 & 100 & 4.861 & 1.384 & 0.071 & 0.465 & 0.838 & 52.600 & 4.700 & 9.464 & 0.822 & 0.000 & 0.503 \\
% orpo\_opt\_100M\_2048\_preprocess & 6 & 100 & 4.984 & 1.399 & 0.093 & 0.479 & 0.853 & 41.800 & 3.200 & 8.917 & 0.748 & -0.000 & 0.463 \\
% orpo\_opt\_cosmos & 6 & 100 & 5.155 & 1.512 & 0.111 & 0.509 & 0.917 & 38.800 & 2.700 & 7.380 & 0.818 & 0.000 & 0.545 \\
% orpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 100 & 4.965 & 1.382 & 0.069 & 0.467 & 0.888 & 57.200 & 5.100 & 9.444 & 0.759 & -0.000 & 0.483 \\
% orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 100 & 4.626 & 1.274 & 0.060 & 0.362 & 0.937 & 34.500 & 2.900 & 8.691 & 0.778 & 0.000 & 0.428 \\
% babylm-seqlen-opt-1024-warmup-v2 & 6 & 100 & 4.895 & 1.365 & 0.080 & 0.467 & 0.955 & 55.600 & 2.300 & 10.311 & 0.825 & 0.000 & 0.568 \\
% babylm-seqlen-opt-4096-warmup-v2 & 6 & 100 & 4.709 & 1.256 & 0.049 & 0.317 & 0.842 & 48.900 & 2.800 & 8.554 & 0.710 & -0.000 & 0.332 \\
% cpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 150 & 5.236 & 1.493 & 0.075 & 0.460 & 0.954 & 75.800 & 4.900 & 8.650 & 0.882 & -0.000 & 0.574 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 6 & 150 & 4.859 & 1.371 & 0.090 & 0.414 & 0.912 & 76.200 & 5.500 & 9.054 & 0.800 & -0.000 & 0.493 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 6 & 150 & 5.048 & 1.427 & 0.088 & 0.438 & 0.918 & 60.700 & 5.000 & 8.728 & 0.723 & 0.000 & 0.505 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 6 & 150 & 5.091 & 0.960 & 0.086 & 0.420 & 0.897 & 62.100 & 4.800 & 8.118 & 0.759 & 0.000 & 0.453 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 6 & 150 & 5.128 & 1.419 & 0.088 & 0.420 & 0.870 & 71.100 & 4.800 & 8.799 & 0.756 & 0.000 & 0.508 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 6 & 150 & 5.011 & 1.397 & 0.092 & 0.429 & 0.902 & 67.300 & 5.300 & 8.373 & 0.835 & 0.000 & 0.542 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 6 & 150 & 5.152 & 1.473 & 0.093 & 0.450 & 0.888 & 66.200 & 5.000 & 8.070 & 0.731 & 0.000 & 0.516 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 6 & 150 & 4.943 & 1.375 & 0.165 & 0.390 & 0.908 & 64.800 & 4.600 & 8.833 & 0.822 & 0.000 & 0.614 \\
% cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 150 & 4.410 & 1.191 & 0.070 & 0.252 & 0.885 & 78.400 & 5.300 & 9.609 & 0.793 & 0.000 & 0.426 \\
% orpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 150 & 5.056 & 1.165 & 0.086 & 0.437 & 0.827 & 75.800 & 6.200 & 8.885 & 0.886 & -0.000 & 0.499 \\
% orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 150 & 4.621 & 1.283 & 0.077 & 0.306 & 0.876 & 58.000 & 4.400 & 8.878 & 0.763 & -0.000 & 0.402 \\
% babylm-seqlen-opt-1024-warmup-v2 & 6 & 150 & 5.060 & 1.429 & 0.076 & 0.439 & 0.858 & 66.000 & 4.600 & 8.523 & 0.724 & 0.000 & 0.482 \\
% babylm-seqlen-opt-4096-warmup-v2 & 6 & 150 & 4.537 & 1.213 & 0.063 & 0.266 & 0.890 & 89.300 & 3.700 & 8.916 & 0.802 & -0.000 & 0.397 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 6 & 200 & 5.023 & 1.419 & 0.089 & 0.412 & 0.898 & 91.200 & 5.600 & 8.917 & 0.861 & 0.000 & 0.568 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 6 & 200 & 4.785 & 1.297 & 0.122 & 0.363 & 0.776 & 117.700 & 6.500 & 8.964 & 0.821 & 0.000 & 0.497 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 6 & 200 & 4.934 & 1.398 & 0.120 & 0.369 & 0.832 & 88.800 & 6.200 & 9.136 & 0.832 & -0.000 & 0.527 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 6 & 200 & 4.947 & 1.363 & 0.142 & 0.378 & 0.888 & 79.700 & 6.100 & 8.782 & 0.816 & 0.000 & 0.554 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 6 & 200 & 4.964 & 1.372 & 0.090 & 0.411 & 0.889 & 71.100 & 6.700 & 8.708 & 0.782 & 0.000 & 0.553 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 6 & 200 & 5.100 & 1.431 & 0.088 & 0.382 & 0.915 & 77.400 & 5.000 & 8.313 & 0.808 & -0.000 & 0.511 \\
% cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 200 & 4.510 & 1.267 & 0.084 & 0.244 & 0.809 & 98.300 & 3.700 & 9.394 & 0.811 & 0.000 & 0.447 \\
% orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 200 & 4.456 & 1.293 & 0.120 & 0.245 & 0.909 & 118.600 & 5.200 & 9.021 & 0.796 & 0.000 & 0.520 \\
% babylm-seqlen-opt-1024-warmup-v2 & 6 & 200 & 4.897 & 1.397 & 0.110 & 0.376 & 0.946 & 100.700 & 6.800 & 9.551 & 0.816 & 0.000 & 0.597 \\
% babylm-seqlen-opt-4096-warmup-v2 & 6 & 200 & 4.402 & 1.181 & 0.047 & 0.227 & 0.870 & 113.300 & 3.100 & 9.030 & 0.773 & 0.000 & 0.376 \\
% cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 250 & 4.375 & 1.179 & 0.104 & 0.212 & 0.857 & 132.200 & 3.300 & 9.918 & 0.816 & -0.000 & 0.429 \\
% orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 250 & 4.498 & 1.226 & 0.151 & 0.214 & 0.932 & 130.800 & 5.000 & 10.981 & 0.817 & 0.000 & 0.578 \\
% babylm-seqlen-opt-4096-warmup-v2 & 6 & 250 & 4.298 & 1.118 & 0.070 & 0.168 & 0.780 & 182.400 & 2.700 & 9.331 & 0.820 & 0.000 & 0.373 \\
% cpo\_opt\_seqlen\_1024\_final\_checkpoint & 8 & 50 & 4.917 & 1.346 & 0.058 & 0.523 & 0.893 & 40.100 & 2.800 & 8.185 & 0.818 & 0.000 & 0.491 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 8 & 50 & 4.786 & 1.307 & 0.063 & 0.507 & 0.894 & 27.500 & 3.000 & 9.427 & 0.715 & -0.000 & 0.435 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 8 & 50 & 5.018 & 1.400 & 0.063 & 0.524 & 0.881 & 30.600 & 2.700 & 8.512 & 0.766 & 0.000 & 0.466 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 8 & 50 & 4.790 & 1.324 & 0.066 & 0.489 & 0.842 & 30.500 & 2.400 & 9.141 & 0.725 & -0.000 & 0.393 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 8 & 50 & 4.858 & 1.346 & 0.075 & 0.510 & 0.885 & 34.000 & 2.900 & 8.717 & 0.788 & 0.000 & 0.475 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 8 & 50 & 4.874 & 1.345 & 0.070 & 0.500 & 0.948 & 29.700 & 2.200 & 8.792 & 0.789 & 0.000 & 0.480 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 8 & 50 & 4.889 & 1.355 & 0.070 & 0.519 & 0.856 & 29.700 & 2.800 & 8.579 & 0.767 & 0.000 & 0.447 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 8 & 50 & 4.868 & 1.337 & 0.059 & 0.508 & 0.850 & 30.200 & 2.900 & 8.428 & 0.723 & 0.000 & 0.437 \\
% cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 50 & 4.495 & 1.193 & 0.073 & 0.363 & 0.941 & 31.100 & 2.000 & 9.187 & 0.745 & 0.000 & 0.406 \\
% orpo\_opt\_seqlen\_1024\_final\_checkpoint & 8 & 50 & 4.958 & 1.359 & 0.076 & 0.511 & 0.930 & 40.000 & 3.800 & 9.058 & 0.807 & 0.000 & 0.567 \\
% orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 50 & 4.437 & 1.186 & 0.059 & 0.359 & 0.858 & 32.700 & 4.500 & 8.461 & 0.701 & 0.000 & 0.337 \\
% babylm-seqlen-opt-1024-warmup-v2 & 8 & 50 & 4.845 & 1.344 & 0.063 & 0.504 & 0.937 & 33.400 & 3.000 & 9.526 & 0.782 & 0.000 & 0.502 \\
% babylm-seqlen-opt-4096-warmup-v2 & 8 & 50 & 4.458 & 1.170 & 0.036 & 0.337 & 0.897 & 38.300 & 1.300 & 8.458 & 0.663 & 0.000 & 0.292 \\
% cpo\_opt\_seqlen\_1024\_final\_checkpoint & 8 & 100 & 4.956 & 1.406 & 0.113 & 0.421 & 0.953 & 69.300 & 4.300 & 8.717 & 0.882 & 0.000 & 0.591 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 8 & 100 & 4.938 & 1.389 & 0.081 & 0.436 & 0.863 & 69.200 & 4.700 & 8.739 & 0.780 & 0.000 & 0.509 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 8 & 100 & 4.954 & 1.402 & 0.083 & 0.435 & 0.898 & 63.500 & 5.600 & 8.987 & 0.758 & -0.000 & 0.468 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 8 & 100 & 5.062 & 1.417 & 0.090 & 0.440 & 0.917 & 63.100 & 4.400 & 8.401 & 0.739 & -0.000 & 0.490 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 8 & 100 & 4.939 & 1.116 & 0.102 & 0.437 & 0.893 & 60.400 & 5.300 & 8.821 & 0.862 & 0.000 & 0.518 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 8 & 100 & 5.110 & 1.419 & 0.084 & 0.431 & 0.930 & 55.600 & 4.000 & 7.904 & 0.844 & 0.000 & 0.529 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 8 & 100 & 5.052 & 1.159 & 0.085 & 0.448 & 0.940 & 56.200 & 5.600 & 8.342 & 0.755 & 0.000 & 0.531 \\
% cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 8 & 100 & 4.903 & 1.104 & 0.108 & 0.431 & 0.879 & 58.300 & 4.400 & 9.010 & 0.794 & 0.000 & 0.479 \\
% cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 100 & 4.493 & 1.187 & 0.073 & 0.273 & 0.832 & 89.500 & 4.300 & 9.361 & 0.808 & -0.000 & 0.383 \\
% orpo\_opt\_seqlen\_1024\_final\_checkpoint & 8 & 100 & 5.052 & 1.424 & 0.072 & 0.443 & 0.957 & 74.700 & 5.800 & 8.705 & 0.847 & 0.000 & 0.590 \\
% orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 100 & 4.482 & 1.315 & 0.120 & 0.294 & 0.903 & 51.900 & 4.100 & 8.326 & 0.807 & -0.000 & 0.394 \\
% babylm-seqlen-opt-1024-warmup-v2 & 8 & 100 & 5.002 & 1.432 & 0.084 & 0.447 & 0.829 & 59.200 & 4.600 & 8.566 & 0.799 & 0.000 & 0.486 \\
% babylm-seqlen-opt-4096-warmup-v2 & 8 & 100 & 4.485 & 1.215 & 0.066 & 0.279 & 0.914 & 70.000 & 2.900 & 8.584 & 0.766 & -0.000 & 0.371 \\
% cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 150 & 4.408 & 1.170 & 0.068 & 0.201 & 0.900 & 115.300 & 3.100 & 9.759 & 0.798 & 0.000 & 0.429 \\
% orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 150 & 4.481 & 1.202 & 0.070 & 0.248 & 0.890 & 85.200 & 3.000 & 8.217 & 0.825 & 0.000 & 0.394 \\
% babylm-seqlen-opt-4096-warmup-v2 & 8 & 150 & 4.505 & 1.218 & 0.036 & 0.251 & 0.856 & 100.000 & 2.500 & 8.419 & 0.828 & -0.000 & 0.334 \\
% cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 200 & 4.366 & 1.223 & 0.109 & 0.196 & 0.934 & 198.200 & 4.000 & 9.354 & 0.851 & -0.000 & 0.471 \\
% orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 200 & 4.663 & 1.284 & 0.107 & 0.247 & 0.830 & 113.100 & 5.400 & 8.748 & 0.794 & 0.000 & 0.450 \\
% babylm-seqlen-opt-4096-warmup-v2 & 8 & 200 & 4.446 & 1.166 & 0.114 & 0.183 & 0.841 & 154.400 & 3.300 & 8.978 & 0.781 & 0.000 & 0.416 \\
% cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 250 & 4.366 & 1.207 & 0.129 & 0.159 & 0.838 & 245.300 & 5.200 & 9.399 & 0.865 & 0.000 & 0.508 \\
% orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 250 & 4.434 & 1.283 & 0.141 & 0.181 & 0.938 & 254.000 & 5.700 & 9.094 & 0.863 & 0.000 & 0.614 \\
% babylm-seqlen-opt-4096-warmup-v2 & 8 & 250 & 4.531 & 1.193 & 0.063 & 0.171 & 0.715 & 162.200 & 4.800 & 8.916 & 0.751 & -0.000 & 0.307 \\

% \end{longtable}
%\end{landscape}

==> tables/multi-turn_dialog_reduced_paper.tex <==
\begin{table*}[!ht]
\centering
\small
\scriptsize
\setlength{\tabcolsep}{3pt} % tighten column padding
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
\textbf{Model} & \textbf{Turn} & \textbf{AoA} & \textbf{CEFR} & \textbf{TTR} & \textbf{Rep.} & \textbf{Overlap} & \textbf{Norm. Avg} \\
\midrule
opt-cefr-iteration1 & 4 & 4.813 & 1.325 & 0.627 & 0.803 & 0.044 & 0.386 \\
opt-cefr-iteration2 & 4 & 4.802 & 1.371 & 0.610 & 0.870 & 0.053 & 0.454 \\
opt-cefr-iteration3 & 4 & 4.782 & 1.305 & 0.606 & 0.904 & 0.082 & 0.469 \\
opt-cefr-iteration4 & 4 & 4.951 & 1.328 & 0.599 & 0.887 & 0.062 & 0.465 \\
opt-cefr-iteration5 & 4 & 4.819 & 1.328 & 0.572 & 0.909 & 0.056 & 0.465 \\
% opt-cefr-reverse-iteration1 & --- & --- & --- & --- & --- & --- & --- \\
% opt-cefr-reverse-iteration2 & --- & --- & --- & --- & --- & --- & --- \\
% opt-cefr-reverse-iteration3 & --- & --- & --- & --- & --- & --- & --- \\
opt-cefr-reverse-iteration4 & 4 & 4.948 & 1.331 & 0.620 & 0.942 & 0.062 & 0.458 \\
opt-cefr-reverse-iteration5 & 4 & 4.929 & 1.322 & 0.596 & 0.867 & 0.063 & 0.399 \\
\midrule
cpo-opt-4096 & 4 & 4.523 & 1.219 & 0.464 & 0.797 & 0.046 & 0.389 \\
cpo-opt-1024 & 4 & 5.011 & 1.408 & 0.624 & 0.946 & 0.044 & 0.496 \\
orpo-opt-1024 & 4 & 4.813 & 1.343 & 0.604 & 0.898 & 0.066 & 0.459 \\
orpo-opt-4096 & 4 & 4.487 & 1.228 & 0.473 & 0.879 & 0.075 & 0.346 \\
\midrule
orpo-opt-100M-2048-preprocess & 4 & 5.123 & 1.415 & 0.582 & 0.777 & 0.078 & 0.440 \\
cpo-opt-100M-2048-preprocess & 4 & 5.087 & 1.373 & 0.620 & 0.851 & 0.068 & 0.436 \\
opt-base & 4 & 5.214 & 1.468 & 0.590 & 0.881 & 0.074 & 0.425 \\
\bottomrule
\end{tabular}%
}
\caption{Evaluation results across progressive CEFR iterations, reverse CEFR iterations, and baseline checkpoints.}
\label{tab:evaluation-results_v3}
\end{table*}


==> tables/multi_turn_dialog_reduced.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lrrrrrrrrrrrrr}
\toprule
\textbf{BabyLM} & \textbf{Turns} & \textbf{Length} & \textbf{AoA} & \textbf{CEFR} & \textbf{Overlap} & \textbf{TTR} & \textbf{Rep.} & \textbf{NumCon} & \textbf{AdversativeCon} & \textbf{Polysemy} & \textbf{VerbRep} & \textbf{Narrativity} & \textbf{NormAvg} \\
\midrule
cpo\_opt\_100M\_2048\_preprocess & 4 & 50 & 5.087 & 1.373 & 0.068 & 0.620 & 0.851 & 13.300 & 0.900 & 7.772 & 0.772 & 0.000 & 0.436 \\
cpo\_opt\_base & 4 & 50 & 5.214 & 1.468 & 0.074 & 0.590 & 0.881 & 13.100 & 0.900 & 7.241 & 0.684 & 0.000 & 0.425 \\
cpo\_opt\_cosmos & 4 & 50 & 5.067 & 1.383 & 0.052 & 0.638 & 0.912 & 14.200 & 1.700 & 8.115 & 0.792 & -0.000 & 0.435 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 50 & 5.011 & 1.408 & 0.044 & 0.624 & 0.946 & 15.600 & 1.600 & 8.118 & 0.790 & 0.000 & 0.496 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 4 & 50 & 4.813 & 1.325 & 0.044 & 0.627 & 0.803 & 16.100 & 1.300 & 9.121 & 0.622 & 0.000 & 0.386 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 4 & 50 & 4.802 & 1.371 & 0.053 & 0.610 & 0.870 & 16.500 & 1.600 & 8.488 & 0.773 & 0.000 & 0.454 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 4 & 50 & 4.782 & 1.305 & 0.082 & 0.606 & 0.904 & 13.600 & 1.500 & 8.769 & 0.822 & -0.000 & 0.469 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 4 & 50 & 4.951 & 1.328 & 0.062 & 0.599 & 0.887 & 13.400 & 1.300 & 7.826 & 0.759 & 0.000 & 0.465 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 4 & 50 & 4.819 & 1.328 & 0.056 & 0.572 & 0.909 & 13.800 & 1.300 & 8.635 & 0.863 & -0.000 & 0.465 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 4 & 50 & 4.948 & 1.331 & 0.062 & 0.620 & 0.942 & 14.400 & 1.000 & 8.725 & 0.750 & -0.000 & 0.458 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 4 & 50 & 4.929 & 1.322 & 0.063 & 0.596 & 0.867 & 15.000 & 1.700 & 7.667 & 0.666 & 0.000 & 0.399 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 50 & 4.523 & 1.219 & 0.046 & 0.464 & 0.797 & 18.100 & 1.600 & 9.379 & 0.753 & 0.000 & 0.389 \\
mamba-sam-seqlen-2048-original & 4 & 50 & 4.770 & 1.353 & 0.048 & 0.609 & 0.945 & 15.700 & 1.700 & 9.280 & 0.828 & 0.000 & 0.494 \\
opt-sam-orpo-mamba-2048-step448 & 4 & 50 & 4.887 & 1.376 & 0.072 & 0.617 & 0.918 & 16.800 & 1.900 & 8.294 & 0.797 & 0.000 & 0.513 \\
opt-sam-orpo-seqlen-2048-step559 & 4 & 50 & 4.948 & 1.365 & 0.052 & 0.615 & 0.866 & 15.100 & 1.400 & 8.926 & 0.590 & 0.000 & 0.390 \\
opt-sam-seqlen-2048-original & 4 & 50 & 4.843 & 1.318 & 0.052 & 0.618 & 0.942 & 17.000 & 1.900 & 8.893 & 0.866 & 0.000 & 0.506 \\
orpo\_opt\_100M\_2048\_preprocess & 4 & 50 & 5.123 & 1.415 & 0.078 & 0.582 & 0.777 & 14.300 & 1.100 & 7.963 & 0.814 & 0.000 & 0.440 \\
orpo\_opt\_cosmos & 4 & 50 & 5.200 & 1.459 & 0.067 & 0.624 & 0.822 & 10.300 & 1.500 & 7.632 & 0.645 & 0.000 & 0.407 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 50 & 4.813 & 1.343 & 0.066 & 0.604 & 0.898 & 17.900 & 1.700 & 8.916 & 0.763 & 0.000 & 0.459 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 50 & 4.487 & 1.228 & 0.075 & 0.473 & 0.879 & 11.500 & 1.400 & 8.631 & 0.720 & -0.000 & 0.346 \\
babylm-seqlen-opt-1024-warmup-v2 & 4 & 50 & 4.864 & 1.343 & 0.057 & 0.594 & 0.925 & 16.500 & 1.600 & 8.589 & 0.827 & 0.000 & 0.491 \\
babylm-seqlen-opt-4096-warmup-v2 & 4 & 50 & 4.487 & 1.172 & 0.030 & 0.449 & 0.867 & 17.100 & 1.000 & 8.662 & 0.677 & -0.000 & 0.290 \\
cpo\_opt\_100M\_2048\_preprocess & 4 & 100 & 5.028 & 1.417 & 0.121 & 0.508 & 0.931 & 23.400 & 2.300 & 7.776 & 0.857 & 0.000 & 0.529 \\
cpo\_opt\_base & 4 & 100 & 5.075 & 1.404 & 0.088 & 0.496 & 0.847 & 21.000 & 1.300 & 8.294 & 0.715 & 0.000 & 0.431 \\
cpo\_opt\_cosmos & 4 & 100 & 5.196 & 1.458 & 0.075 & 0.540 & 0.876 & 25.100 & 1.500 & 8.216 & 0.796 & -0.000 & 0.461 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 100 & 4.921 & 1.353 & 0.062 & 0.537 & 0.955 & 35.900 & 3.300 & 9.218 & 0.839 & -0.000 & 0.521 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 4 & 100 & 4.974 & 1.391 & 0.069 & 0.548 & 0.879 & 29.800 & 2.800 & 8.771 & 0.791 & 0.000 & 0.481 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 4 & 100 & 4.888 & 1.374 & 0.082 & 0.523 & 0.817 & 31.700 & 2.100 & 8.968 & 0.717 & 0.000 & 0.427 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 4 & 100 & 4.900 & 1.365 & 0.083 & 0.522 & 0.903 & 33.600 & 4.200 & 9.265 & 0.825 & 0.000 & 0.543 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 4 & 100 & 4.934 & 1.350 & 0.045 & 0.526 & 0.906 & 26.400 & 2.000 & 8.090 & 0.876 & 0.000 & 0.479 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 4 & 100 & 4.984 & 1.395 & 0.063 & 0.524 & 0.905 & 25.700 & 2.600 & 8.415 & 0.826 & -0.000 & 0.475 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 4 & 100 & 4.954 & 1.367 & 0.076 & 0.513 & 0.844 & 21.900 & 2.000 & 8.098 & 0.671 & 0.000 & 0.413 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 4 & 100 & 4.847 & 1.353 & 0.092 & 0.513 & 0.884 & 27.400 & 2.100 & 8.416 & 0.752 & 0.000 & 0.459 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 100 & 4.532 & 1.224 & 0.058 & 0.391 & 0.891 & 33.300 & 3.000 & 9.435 & 0.821 & 0.000 & 0.419 \\
mamba-sam-seqlen-2048-original & 4 & 100 & 4.770 & 1.406 & 0.118 & 0.501 & 0.956 & 40.900 & 4.700 & 8.543 & 0.788 & -0.000 & 0.521 \\
opt-sam-orpo-mamba-2048-step448 & 4 & 100 & 4.797 & 1.390 & 0.099 & 0.514 & 0.799 & 42.100 & 5.400 & 9.338 & 0.870 & -0.000 & 0.517 \\
opt-sam-orpo-seqlen-2048-step559 & 4 & 100 & 4.728 & 1.304 & 0.077 & 0.512 & 0.893 & 40.100 & 3.800 & 9.944 & 0.844 & -0.000 & 0.476 \\
opt-sam-seqlen-2048-original & 4 & 100 & 4.917 & 1.439 & 0.089 & 0.523 & 0.904 & 35.500 & 3.000 & 9.314 & 0.796 & -0.000 & 0.497 \\
orpo\_opt\_100M\_2048\_preprocess & 4 & 100 & 5.021 & 1.419 & 0.085 & 0.524 & 0.862 & 20.300 & 0.800 & 8.210 & 0.851 & 0.000 & 0.483 \\
orpo\_opt\_cosmos & 4 & 100 & 5.211 & 1.443 & 0.091 & 0.532 & 0.866 & 26.100 & 2.000 & 7.734 & 0.851 & -0.000 & 0.484 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 100 & 4.953 & 1.365 & 0.068 & 0.534 & 0.909 & 35.200 & 3.300 & 8.949 & 0.778 & -0.000 & 0.485 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 100 & 4.711 & 1.262 & 0.062 & 0.419 & 0.870 & 19.600 & 1.400 & 8.710 & 0.768 & -0.000 & 0.373 \\
babylm-seqlen-opt-1024-warmup-v2 & 4 & 100 & 4.878 & 1.342 & 0.110 & 0.493 & 0.847 & 38.800 & 3.300 & 9.587 & 0.867 & -0.000 & 0.503 \\
babylm-seqlen-opt-4096-warmup-v2 & 4 & 100 & 4.378 & 1.189 & 0.067 & 0.341 & 0.770 & 35.000 & 2.900 & 8.478 & 0.793 & -0.000 & 0.299 \\
cpo\_opt\_100M\_2048\_preprocess & 4 & 150 & 5.057 & 1.441 & 0.115 & 0.469 & 0.828 & 33.400 & 1.200 & 7.582 & 0.708 & -0.000 & 0.416 \\
cpo\_opt\_base & 4 & 150 & 5.153 & 1.433 & 0.082 & 0.458 & 0.883 & 34.500 & 1.700 & 8.358 & 0.837 & -0.000 & 0.470 \\
cpo\_opt\_cosmos & 4 & 150 & 5.174 & 1.460 & 0.076 & 0.488 & 0.894 & 33.800 & 3.400 & 7.571 & 0.748 & 0.000 & 0.481 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 150 & 4.912 & 1.360 & 0.104 & 0.445 & 0.959 & 52.600 & 5.000 & 9.865 & 0.852 & 0.000 & 0.584 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 4 & 150 & 4.893 & 1.360 & 0.092 & 0.469 & 0.896 & 43.200 & 3.200 & 9.341 & 0.819 & 0.000 & 0.522 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 4 & 150 & 4.923 & 1.418 & 0.105 & 0.467 & 0.936 & 45.100 & 3.000 & 9.136 & 0.847 & 0.000 & 0.600 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 4 & 150 & 4.949 & 1.353 & 0.109 & 0.439 & 0.901 & 40.200 & 3.700 & 8.797 & 0.768 & 0.000 & 0.494 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 4 & 150 & 5.055 & 1.350 & 0.083 & 0.448 & 0.889 & 33.300 & 2.600 & 8.742 & 0.717 & -0.000 & 0.400 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 4 & 150 & 4.989 & 1.379 & 0.114 & 0.443 & 0.870 & 34.600 & 2.100 & 8.785 & 0.765 & 0.000 & 0.476 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 4 & 150 & 4.983 & 1.375 & 0.081 & 0.499 & 0.894 & 35.000 & 1.900 & 8.627 & 0.716 & 0.000 & 0.449 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 4 & 150 & 4.901 & 1.380 & 0.070 & 0.470 & 0.862 & 40.900 & 3.600 & 8.410 & 0.760 & -0.000 & 0.427 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 150 & 4.385 & 1.256 & 0.128 & 0.302 & 0.749 & 49.200 & 3.600 & 9.345 & 0.775 & 0.000 & 0.413 \\
mamba-sam-seqlen-2048-original & 4 & 150 & 4.918 & 1.435 & 0.075 & 0.470 & 0.906 & 55.800 & 5.500 & 9.043 & 0.816 & -0.000 & 0.520 \\
opt-sam-orpo-mamba-2048-step448 & 4 & 150 & 4.880 & 1.384 & 0.073 & 0.470 & 0.870 & 64.800 & 7.600 & 9.414 & 0.783 & -0.000 & 0.519 \\
opt-sam-orpo-seqlen-2048-step559 & 4 & 150 & 4.910 & 1.371 & 0.069 & 0.473 & 0.921 & 47.300 & 3.500 & 8.704 & 0.787 & -0.000 & 0.482 \\
opt-sam-seqlen-2048-original & 4 & 150 & 4.998 & 1.416 & 0.117 & 0.466 & 0.913 & 45.500 & 1.800 & 9.115 & 0.789 & 0.000 & 0.541 \\
orpo\_opt\_100M\_2048\_preprocess & 4 & 150 & 5.169 & 1.432 & 0.109 & 0.473 & 0.766 & 33.300 & 1.600 & 8.092 & 0.722 & 0.000 & 0.441 \\
orpo\_opt\_cosmos & 4 & 150 & 5.284 & 1.489 & 0.102 & 0.507 & 0.847 & 27.000 & 1.500 & 8.097 & 0.797 & -0.000 & 0.488 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 150 & 5.077 & 1.395 & 0.076 & 0.474 & 0.825 & 69.600 & 4.500 & 8.858 & 0.815 & -0.000 & 0.470 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 150 & 4.732 & 1.301 & 0.078 & 0.391 & 0.855 & 37.700 & 2.500 & 8.890 & 0.724 & -0.000 & 0.391 \\
babylm-seqlen-opt-1024-warmup-v2 & 4 & 150 & 4.778 & 1.351 & 0.098 & 0.441 & 0.903 & 55.800 & 4.300 & 9.446 & 0.820 & -0.000 & 0.490 \\
babylm-seqlen-opt-4096-warmup-v2 & 4 & 150 & 4.473 & 1.222 & 0.032 & 0.355 & 0.900 & 50.300 & 3.200 & 9.304 & 0.779 & 0.000 & 0.383 \\
cpo\_opt\_100M\_2048\_preprocess & 4 & 200 & 5.171 & 0.932 & 0.108 & 0.432 & 0.904 & 40.300 & 3.100 & 8.410 & 0.767 & -0.000 & 0.420 \\
cpo\_opt\_base & 4 & 200 & 5.378 & 1.506 & 0.099 & 0.433 & 0.882 & 41.500 & 0.900 & 7.803 & 0.738 & -0.000 & 0.457 \\
cpo\_opt\_cosmos & 4 & 200 & 5.191 & 1.270 & 0.130 & 0.435 & 0.933 & 50.800 & 3.500 & 8.165 & 0.868 & -0.000 & 0.510 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 200 & 4.960 & 1.394 & 0.105 & 0.427 & 0.891 & 67.500 & 4.300 & 9.388 & 0.823 & -0.000 & 0.521 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 4 & 200 & 4.827 & 1.345 & 0.113 & 0.430 & 0.946 & 59.900 & 5.300 & 9.482 & 0.862 & -0.000 & 0.558 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 4 & 200 & 4.952 & 1.391 & 0.061 & 0.419 & 0.874 & 58.100 & 3.200 & 9.061 & 0.795 & 0.000 & 0.492 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 4 & 200 & 5.184 & 1.474 & 0.115 & 0.434 & 0.873 & 60.400 & 3.500 & 8.268 & 0.800 & -0.000 & 0.508 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 4 & 200 & 4.899 & 1.337 & 0.071 & 0.469 & 0.872 & 44.300 & 3.200 & 8.790 & 0.730 & -0.000 & 0.420 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 4 & 200 & 5.025 & 1.387 & 0.093 & 0.441 & 0.904 & 50.500 & 3.700 & 8.466 & 0.833 & -0.000 & 0.510 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 4 & 200 & 5.006 & 1.444 & 0.068 & 0.454 & 0.887 & 43.300 & 3.200 & 7.894 & 0.706 & -0.000 & 0.400 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 4 & 200 & 5.163 & 1.257 & 0.083 & 0.453 & 0.875 & 50.100 & 4.400 & 7.789 & 0.786 & 0.000 & 0.463 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 200 & 4.367 & 1.188 & 0.082 & 0.245 & 0.770 & 102.700 & 3.000 & 9.584 & 0.875 & -0.000 & 0.369 \\
mamba-sam-seqlen-2048-original & 4 & 200 & 4.967 & 1.547 & 0.108 & 0.430 & 0.819 & 73.800 & 8.200 & 8.868 & 0.779 & 0.000 & 0.544 \\
opt-sam-orpo-mamba-2048-step448 & 4 & 200 & 5.049 & 1.435 & 0.095 & 0.438 & 0.853 & 76.100 & 7.200 & 9.044 & 0.839 & 0.000 & 0.577 \\
opt-sam-orpo-seqlen-2048-step559 & 4 & 200 & 4.825 & 1.152 & 0.090 & 0.456 & 0.829 & 62.500 & 5.100 & 9.511 & 0.872 & 0.000 & 0.513 \\
opt-sam-seqlen-2048-original & 4 & 200 & 4.947 & 1.384 & 0.073 & 0.456 & 0.841 & 59.800 & 3.300 & 9.724 & 0.825 & 0.000 & 0.498 \\
orpo\_opt\_100M\_2048\_preprocess & 4 & 200 & 5.080 & 1.198 & 0.100 & 0.463 & 0.928 & 39.000 & 3.600 & 8.636 & 0.797 & -0.000 & 0.490 \\
orpo\_opt\_cosmos & 4 & 200 & 5.417 & 1.546 & 0.074 & 0.478 & 0.854 & 43.100 & 3.200 & 7.906 & 0.842 & -0.000 & 0.513 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 200 & 5.047 & 0.888 & 0.094 & 0.438 & 0.948 & 71.000 & 4.000 & 8.855 & 0.854 & -0.000 & 0.473 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 200 & 4.533 & 1.340 & 0.122 & 0.306 & 0.808 & 65.100 & 2.600 & 8.758 & 0.788 & 0.000 & 0.423 \\
babylm-seqlen-opt-1024-warmup-v2 & 4 & 200 & 5.010 & 1.410 & 0.072 & 0.436 & 0.952 & 75.800 & 4.400 & 9.447 & 0.804 & -0.000 & 0.537 \\
babylm-seqlen-opt-4096-warmup-v2 & 4 & 200 & 4.418 & 1.164 & 0.042 & 0.268 & 0.750 & 70.400 & 1.900 & 8.675 & 0.764 & 0.000 & 0.291 \\
cpo\_opt\_100M\_2048\_preprocess & 4 & 250 & 5.054 & 1.393 & 0.125 & 0.396 & 0.950 & 57.700 & 2.500 & 8.453 & 0.827 & 0.000 & 0.547 \\
cpo\_opt\_base & 4 & 250 & 5.655 & 1.647 & 0.108 & 0.411 & 0.835 & 47.300 & 3.000 & 7.798 & 0.780 & -0.000 & 0.524 \\
cpo\_opt\_cosmos & 4 & 250 & 5.124 & 1.435 & 0.104 & 0.419 & 0.855 & 61.500 & 5.500 & 8.321 & 0.752 & -0.000 & 0.482 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 250 & 4.932 & 1.391 & 0.103 & 0.411 & 0.819 & 80.200 & 7.300 & 9.086 & 0.855 & 0.000 & 0.550 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 4 & 250 & 5.149 & 1.467 & 0.104 & 0.399 & 0.910 & 60.400 & 2.900 & 8.551 & 0.805 & -0.000 & 0.509 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 4 & 250 & 4.927 & 1.378 & 0.099 & 0.396 & 0.840 & 55.800 & 5.800 & 9.602 & 0.653 & 0.000 & 0.475 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 4 & 250 & 4.898 & 1.375 & 0.140 & 0.409 & 0.805 & 60.800 & 4.900 & 9.658 & 0.855 & 0.000 & 0.541 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 4 & 250 & 5.029 & 1.427 & 0.092 & 0.387 & 0.887 & 66.900 & 5.800 & 8.251 & 0.719 & -0.000 & 0.472 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 4 & 250 & 5.183 & 1.434 & 0.095 & 0.419 & 0.838 & 59.000 & 3.100 & 8.245 & 0.761 & 0.000 & 0.499 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 4 & 250 & 5.007 & 1.391 & 0.101 & 0.409 & 0.839 & 48.600 & 3.600 & 8.467 & 0.727 & 0.000 & 0.467 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 4 & 250 & 5.016 & 0.910 & 0.155 & 0.370 & 0.911 & 68.100 & 4.700 & 8.382 & 0.860 & 0.000 & 0.514 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 250 & 4.632 & 1.245 & 0.094 & 0.286 & 0.891 & 78.300 & 2.500 & 9.265 & 0.794 & 0.000 & 0.443 \\
mamba-sam-seqlen-2048-original & 4 & 250 & 4.836 & 1.413 & 0.100 & 0.411 & 0.869 & 100.300 & 10.300 & 9.417 & 0.858 & -0.000 & 0.576 \\
opt-sam-orpo-mamba-2048-step448 & 4 & 250 & 4.777 & 1.140 & 0.126 & 0.388 & 0.778 & 108.300 & 12.200 & 8.808 & 0.877 & -0.000 & 0.525 \\
opt-sam-orpo-seqlen-2048-step559 & 4 & 250 & 5.091 & 1.454 & 0.092 & 0.407 & 0.861 & 67.500 & 5.600 & 8.867 & 0.791 & -0.000 & 0.518 \\
opt-sam-seqlen-2048-original & 4 & 250 & 4.997 & 1.439 & 0.116 & 0.401 & 0.907 & 71.200 & 5.900 & 8.697 & 0.834 & 0.000 & 0.567 \\
orpo\_opt\_100M\_2048\_preprocess & 4 & 250 & 5.160 & 1.247 & 0.101 & 0.424 & 0.897 & 47.700 & 4.100 & 8.531 & 0.830 & 0.000 & 0.525 \\
orpo\_opt\_cosmos & 4 & 250 & 5.386 & 1.497 & 0.120 & 0.436 & 0.844 & 47.600 & 3.000 & 7.614 & 0.824 & -0.000 & 0.503 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 250 & 5.073 & 1.197 & 0.096 & 0.412 & 0.888 & 90.700 & 8.200 & 9.247 & 0.846 & 0.000 & 0.567 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 250 & 4.741 & 1.391 & 0.117 & 0.318 & 0.810 & 49.500 & 3.900 & 7.859 & 0.794 & -0.000 & 0.395 \\
babylm-seqlen-opt-1024-warmup-v2 & 4 & 250 & 4.977 & 1.426 & 0.077 & 0.429 & 0.905 & 71.000 & 4.000 & 8.592 & 0.823 & 0.000 & 0.545 \\
babylm-seqlen-opt-4096-warmup-v2 & 4 & 250 & 4.549 & 1.223 & 0.070 & 0.266 & 0.922 & 79.400 & 3.300 & 9.127 & 0.816 & 0.000 & 0.447 \\
cpo\_opt\_100M\_2048\_preprocess & 6 & 50 & 5.071 & 1.423 & 0.065 & 0.564 & 0.830 & 19.000 & 2.500 & 8.146 & 0.740 & 0.000 & 0.434 \\
cpo\_opt\_base & 6 & 50 & 5.022 & 1.355 & 0.057 & 0.549 & 0.891 & 18.400 & 1.800 & 8.236 & 0.766 & -0.000 & 0.432 \\
cpo\_opt\_cosmos & 6 & 50 & 5.123 & 1.457 & 0.049 & 0.560 & 0.912 & 20.300 & 2.100 & 7.358 & 0.745 & -0.000 & 0.432 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 50 & 4.947 & 1.405 & 0.050 & 0.563 & 0.911 & 25.900 & 1.800 & 8.552 & 0.745 & 0.000 & 0.461 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 6 & 50 & 4.898 & 1.350 & 0.050 & 0.554 & 0.915 & 23.400 & 2.600 & 8.527 & 0.796 & 0.000 & 0.491 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 6 & 50 & 4.812 & 1.341 & 0.067 & 0.543 & 0.922 & 25.200 & 1.200 & 9.002 & 0.845 & 0.000 & 0.514 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 6 & 50 & 4.812 & 1.337 & 0.083 & 0.531 & 0.893 & 20.300 & 1.100 & 8.223 & 0.722 & 0.000 & 0.429 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 6 & 50 & 4.882 & 1.339 & 0.057 & 0.536 & 0.938 & 22.700 & 2.400 & 9.117 & 0.678 & 0.000 & 0.444 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 6 & 50 & 4.886 & 1.333 & 0.064 & 0.528 & 0.929 & 22.600 & 2.100 & 8.392 & 0.800 & 0.000 & 0.463 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 6 & 50 & 4.846 & 1.331 & 0.036 & 0.557 & 0.916 & 21.300 & 1.700 & 8.521 & 0.740 & 0.000 & 0.428 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 6 & 50 & 4.982 & 1.373 & 0.069 & 0.541 & 0.853 & 23.000 & 2.000 & 7.914 & 0.754 & -0.000 & 0.402 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 50 & 4.525 & 1.231 & 0.094 & 0.411 & 0.921 & 22.500 & 1.600 & 8.597 & 0.787 & -0.000 & 0.387 \\
mamba-sam-seqlen-2048-original & 6 & 50 & 4.881 & 1.325 & 0.059 & 0.558 & 0.969 & 29.200 & 3.100 & 9.034 & 0.832 & -0.000 & 0.516 \\
opt-sam-orpo-mamba-2048-step448 & 6 & 50 & 4.831 & 1.369 & 0.084 & 0.553 & 0.912 & 24.200 & 3.500 & 9.184 & 0.758 & 0.000 & 0.505 \\
opt-sam-orpo-seqlen-2048-step559 & 6 & 50 & 5.072 & 1.382 & 0.055 & 0.576 & 0.868 & 25.400 & 2.300 & 9.109 & 0.778 & 0.000 & 0.514 \\
opt-sam-seqlen-2048-original & 6 & 50 & 4.858 & 1.323 & 0.052 & 0.551 & 0.932 & 24.500 & 2.100 & 8.350 & 0.762 & -0.000 & 0.422 \\
orpo\_opt\_100M\_2048\_preprocess & 6 & 50 & 5.145 & 1.411 & 0.082 & 0.546 & 0.865 & 18.400 & 0.700 & 7.507 & 0.817 & 0.000 & 0.462 \\
orpo\_opt\_cosmos & 6 & 50 & 5.375 & 1.514 & 0.055 & 0.564 & 0.858 & 17.600 & 0.500 & 6.911 & 0.740 & -0.000 & 0.390 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 50 & 4.951 & 1.390 & 0.065 & 0.567 & 0.927 & 26.100 & 2.400 & 8.366 & 0.744 & -0.000 & 0.449 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 50 & 4.612 & 1.234 & 0.061 & 0.419 & 0.907 & 19.000 & 2.000 & 9.567 & 0.793 & -0.000 & 0.401 \\
babylm-seqlen-opt-1024-warmup-v2 & 6 & 50 & 4.864 & 1.339 & 0.038 & 0.543 & 0.901 & 25.300 & 2.500 & 8.834 & 0.774 & -0.000 & 0.423 \\
babylm-seqlen-opt-4096-warmup-v2 & 6 & 50 & 4.478 & 1.197 & 0.029 & 0.408 & 0.803 & 22.100 & 1.300 & 8.928 & 0.643 & -0.000 & 0.239 \\
cpo\_opt\_100M\_2048\_preprocess & 6 & 100 & 5.093 & 1.437 & 0.090 & 0.483 & 0.858 & 36.100 & 1.600 & 8.253 & 0.776 & 0.000 & 0.493 \\
cpo\_opt\_base & 6 & 100 & 5.035 & 1.429 & 0.080 & 0.489 & 0.892 & 38.500 & 2.500 & 8.295 & 0.780 & -0.000 & 0.472 \\
cpo\_opt\_cosmos & 6 & 100 & 5.075 & 1.395 & 0.116 & 0.465 & 0.904 & 43.300 & 4.000 & 8.329 & 0.887 & -0.000 & 0.548 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 100 & 4.904 & 1.364 & 0.094 & 0.456 & 0.932 & 55.000 & 5.000 & 9.643 & 0.883 & 0.000 & 0.583 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 6 & 100 & 4.843 & 1.325 & 0.099 & 0.453 & 0.901 & 51.400 & 3.500 & 9.253 & 0.783 & 0.000 & 0.497 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 6 & 100 & 4.805 & 1.323 & 0.092 & 0.460 & 0.892 & 49.000 & 4.000 & 9.001 & 0.787 & 0.000 & 0.500 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 6 & 100 & 4.916 & 1.107 & 0.112 & 0.465 & 0.876 & 42.900 & 2.400 & 8.827 & 0.810 & -0.000 & 0.457 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 6 & 100 & 4.943 & 1.127 & 0.078 & 0.486 & 0.888 & 40.100 & 3.700 & 8.228 & 0.743 & 0.000 & 0.433 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 6 & 100 & 4.845 & 1.366 & 0.095 & 0.469 & 0.912 & 45.600 & 3.200 & 8.514 & 0.796 & -0.000 & 0.472 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 6 & 100 & 4.953 & 1.363 & 0.068 & 0.469 & 0.915 & 44.500 & 3.600 & 8.648 & 0.744 & -0.000 & 0.457 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 6 & 100 & 4.974 & 1.394 & 0.075 & 0.483 & 0.858 & 42.800 & 3.900 & 8.832 & 0.723 & 0.000 & 0.462 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 100 & 4.430 & 1.320 & 0.129 & 0.299 & 0.764 & 55.700 & 3.000 & 8.628 & 0.791 & 0.000 & 0.392 \\
mamba-sam-seqlen-2048-original & 6 & 100 & 4.838 & 1.429 & 0.105 & 0.474 & 0.840 & 59.100 & 5.600 & 9.590 & 0.811 & -0.000 & 0.506 \\
opt-sam-orpo-mamba-2048-step448 & 6 & 100 & 4.959 & 1.411 & 0.066 & 0.478 & 0.962 & 60.700 & 6.500 & 8.757 & 0.757 & -0.000 & 0.516 \\
opt-sam-orpo-seqlen-2048-step559 & 6 & 100 & 4.912 & 1.352 & 0.080 & 0.508 & 0.944 & 44.600 & 3.800 & 8.853 & 0.841 & -0.000 & 0.517 \\
opt-sam-seqlen-2048-original & 6 & 100 & 4.861 & 1.384 & 0.071 & 0.465 & 0.838 & 52.600 & 4.700 & 9.464 & 0.822 & 0.000 & 0.503 \\
orpo\_opt\_100M\_2048\_preprocess & 6 & 100 & 4.984 & 1.399 & 0.093 & 0.479 & 0.853 & 41.800 & 3.200 & 8.917 & 0.748 & -0.000 & 0.463 \\
orpo\_opt\_cosmos & 6 & 100 & 5.155 & 1.512 & 0.111 & 0.509 & 0.917 & 38.800 & 2.700 & 7.380 & 0.818 & 0.000 & 0.545 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 100 & 4.965 & 1.382 & 0.069 & 0.467 & 0.888 & 57.200 & 5.100 & 9.444 & 0.759 & -0.000 & 0.483 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 100 & 4.626 & 1.274 & 0.060 & 0.362 & 0.937 & 34.500 & 2.900 & 8.691 & 0.778 & 0.000 & 0.428 \\
babylm-seqlen-opt-1024-warmup-v2 & 6 & 100 & 4.895 & 1.365 & 0.080 & 0.467 & 0.955 & 55.600 & 2.300 & 10.311 & 0.825 & 0.000 & 0.568 \\
babylm-seqlen-opt-4096-warmup-v2 & 6 & 100 & 4.709 & 1.256 & 0.049 & 0.317 & 0.842 & 48.900 & 2.800 & 8.554 & 0.710 & -0.000 & 0.332 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 150 & 5.236 & 1.493 & 0.075 & 0.460 & 0.954 & 75.800 & 4.900 & 8.650 & 0.882 & -0.000 & 0.574 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 6 & 150 & 4.859 & 1.371 & 0.090 & 0.414 & 0.912 & 76.200 & 5.500 & 9.054 & 0.800 & -0.000 & 0.493 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 6 & 150 & 5.048 & 1.427 & 0.088 & 0.438 & 0.918 & 60.700 & 5.000 & 8.728 & 0.723 & 0.000 & 0.505 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 6 & 150 & 5.091 & 0.960 & 0.086 & 0.420 & 0.897 & 62.100 & 4.800 & 8.118 & 0.759 & 0.000 & 0.453 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 6 & 150 & 5.128 & 1.419 & 0.088 & 0.420 & 0.870 & 71.100 & 4.800 & 8.799 & 0.756 & 0.000 & 0.508 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 6 & 150 & 5.011 & 1.397 & 0.092 & 0.429 & 0.902 & 67.300 & 5.300 & 8.373 & 0.835 & 0.000 & 0.542 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 6 & 150 & 5.152 & 1.473 & 0.093 & 0.450 & 0.888 & 66.200 & 5.000 & 8.070 & 0.731 & 0.000 & 0.516 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 6 & 150 & 4.943 & 1.375 & 0.165 & 0.390 & 0.908 & 64.800 & 4.600 & 8.833 & 0.822 & 0.000 & 0.614 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 150 & 4.410 & 1.191 & 0.070 & 0.252 & 0.885 & 78.400 & 5.300 & 9.609 & 0.793 & 0.000 & 0.426 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 150 & 5.056 & 1.165 & 0.086 & 0.437 & 0.827 & 75.800 & 6.200 & 8.885 & 0.886 & -0.000 & 0.499 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 150 & 4.621 & 1.283 & 0.077 & 0.306 & 0.876 & 58.000 & 4.400 & 8.878 & 0.763 & -0.000 & 0.402 \\
babylm-seqlen-opt-1024-warmup-v2 & 6 & 150 & 5.060 & 1.429 & 0.076 & 0.439 & 0.858 & 66.000 & 4.600 & 8.523 & 0.724 & 0.000 & 0.482 \\
babylm-seqlen-opt-4096-warmup-v2 & 6 & 150 & 4.537 & 1.213 & 0.063 & 0.266 & 0.890 & 89.300 & 3.700 & 8.916 & 0.802 & -0.000 & 0.397 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 6 & 200 & 5.023 & 1.419 & 0.089 & 0.412 & 0.898 & 91.200 & 5.600 & 8.917 & 0.861 & 0.000 & 0.568 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 6 & 200 & 4.785 & 1.297 & 0.122 & 0.363 & 0.776 & 117.700 & 6.500 & 8.964 & 0.821 & 0.000 & 0.497 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 6 & 200 & 4.934 & 1.398 & 0.120 & 0.369 & 0.832 & 88.800 & 6.200 & 9.136 & 0.832 & -0.000 & 0.527 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 6 & 200 & 4.947 & 1.363 & 0.142 & 0.378 & 0.888 & 79.700 & 6.100 & 8.782 & 0.816 & 0.000 & 0.554 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 6 & 200 & 4.964 & 1.372 & 0.090 & 0.411 & 0.889 & 71.100 & 6.700 & 8.708 & 0.782 & 0.000 & 0.553 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 6 & 200 & 5.100 & 1.431 & 0.088 & 0.382 & 0.915 & 77.400 & 5.000 & 8.313 & 0.808 & -0.000 & 0.511 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 200 & 4.510 & 1.267 & 0.084 & 0.244 & 0.809 & 98.300 & 3.700 & 9.394 & 0.811 & 0.000 & 0.447 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 200 & 4.456 & 1.293 & 0.120 & 0.245 & 0.909 & 118.600 & 5.200 & 9.021 & 0.796 & 0.000 & 0.520 \\
babylm-seqlen-opt-1024-warmup-v2 & 6 & 200 & 4.897 & 1.397 & 0.110 & 0.376 & 0.946 & 100.700 & 6.800 & 9.551 & 0.816 & 0.000 & 0.597 \\
babylm-seqlen-opt-4096-warmup-v2 & 6 & 200 & 4.402 & 1.181 & 0.047 & 0.227 & 0.870 & 113.300 & 3.100 & 9.030 & 0.773 & 0.000 & 0.376 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 250 & 4.375 & 1.179 & 0.104 & 0.212 & 0.857 & 132.200 & 3.300 & 9.918 & 0.816 & -0.000 & 0.429 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 250 & 4.498 & 1.226 & 0.151 & 0.214 & 0.932 & 130.800 & 5.000 & 10.981 & 0.817 & 0.000 & 0.578 \\
babylm-seqlen-opt-4096-warmup-v2 & 6 & 250 & 4.298 & 1.118 & 0.070 & 0.168 & 0.780 & 182.400 & 2.700 & 9.331 & 0.820 & 0.000 & 0.373 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 8 & 50 & 4.917 & 1.346 & 0.058 & 0.523 & 0.893 & 40.100 & 2.800 & 8.185 & 0.818 & 0.000 & 0.491 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 8 & 50 & 4.786 & 1.307 & 0.063 & 0.507 & 0.894 & 27.500 & 3.000 & 9.427 & 0.715 & -0.000 & 0.435 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 8 & 50 & 5.018 & 1.400 & 0.063 & 0.524 & 0.881 & 30.600 & 2.700 & 8.512 & 0.766 & 0.000 & 0.466 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 8 & 50 & 4.790 & 1.324 & 0.066 & 0.489 & 0.842 & 30.500 & 2.400 & 9.141 & 0.725 & -0.000 & 0.393 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 8 & 50 & 4.858 & 1.346 & 0.075 & 0.510 & 0.885 & 34.000 & 2.900 & 8.717 & 0.788 & 0.000 & 0.475 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 8 & 50 & 4.874 & 1.345 & 0.070 & 0.500 & 0.948 & 29.700 & 2.200 & 8.792 & 0.789 & 0.000 & 0.480 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 8 & 50 & 4.889 & 1.355 & 0.070 & 0.519 & 0.856 & 29.700 & 2.800 & 8.579 & 0.767 & 0.000 & 0.447 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 8 & 50 & 4.868 & 1.337 & 0.059 & 0.508 & 0.850 & 30.200 & 2.900 & 8.428 & 0.723 & 0.000 & 0.437 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 50 & 4.495 & 1.193 & 0.073 & 0.363 & 0.941 & 31.100 & 2.000 & 9.187 & 0.745 & 0.000 & 0.406 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 8 & 50 & 4.958 & 1.359 & 0.076 & 0.511 & 0.930 & 40.000 & 3.800 & 9.058 & 0.807 & 0.000 & 0.567 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 50 & 4.437 & 1.186 & 0.059 & 0.359 & 0.858 & 32.700 & 4.500 & 8.461 & 0.701 & 0.000 & 0.337 \\
babylm-seqlen-opt-1024-warmup-v2 & 8 & 50 & 4.845 & 1.344 & 0.063 & 0.504 & 0.937 & 33.400 & 3.000 & 9.526 & 0.782 & 0.000 & 0.502 \\
babylm-seqlen-opt-4096-warmup-v2 & 8 & 50 & 4.458 & 1.170 & 0.036 & 0.337 & 0.897 & 38.300 & 1.300 & 8.458 & 0.663 & 0.000 & 0.292 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 8 & 100 & 4.956 & 1.406 & 0.113 & 0.421 & 0.953 & 69.300 & 4.300 & 8.717 & 0.882 & 0.000 & 0.591 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 8 & 100 & 4.938 & 1.389 & 0.081 & 0.436 & 0.863 & 69.200 & 4.700 & 8.739 & 0.780 & 0.000 & 0.509 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 8 & 100 & 4.954 & 1.402 & 0.083 & 0.435 & 0.898 & 63.500 & 5.600 & 8.987 & 0.758 & -0.000 & 0.468 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 8 & 100 & 5.062 & 1.417 & 0.090 & 0.440 & 0.917 & 63.100 & 4.400 & 8.401 & 0.739 & -0.000 & 0.490 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 8 & 100 & 4.939 & 1.116 & 0.102 & 0.437 & 0.893 & 60.400 & 5.300 & 8.821 & 0.862 & 0.000 & 0.518 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 8 & 100 & 5.110 & 1.419 & 0.084 & 0.431 & 0.930 & 55.600 & 4.000 & 7.904 & 0.844 & 0.000 & 0.529 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 8 & 100 & 5.052 & 1.159 & 0.085 & 0.448 & 0.940 & 56.200 & 5.600 & 8.342 & 0.755 & 0.000 & 0.531 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 8 & 100 & 4.903 & 1.104 & 0.108 & 0.431 & 0.879 & 58.300 & 4.400 & 9.010 & 0.794 & 0.000 & 0.479 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 100 & 4.493 & 1.187 & 0.073 & 0.273 & 0.832 & 89.500 & 4.300 & 9.361 & 0.808 & -0.000 & 0.383 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 8 & 100 & 5.052 & 1.424 & 0.072 & 0.443 & 0.957 & 74.700 & 5.800 & 8.705 & 0.847 & 0.000 & 0.590 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 100 & 4.482 & 1.315 & 0.120 & 0.294 & 0.903 & 51.900 & 4.100 & 8.326 & 0.807 & -0.000 & 0.394 \\
babylm-seqlen-opt-1024-warmup-v2 & 8 & 100 & 5.002 & 1.432 & 0.084 & 0.447 & 0.829 & 59.200 & 4.600 & 8.566 & 0.799 & 0.000 & 0.486 \\
babylm-seqlen-opt-4096-warmup-v2 & 8 & 100 & 4.485 & 1.215 & 0.066 & 0.279 & 0.914 & 70.000 & 2.900 & 8.584 & 0.766 & -0.000 & 0.371 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 150 & 4.408 & 1.170 & 0.068 & 0.201 & 0.900 & 115.300 & 3.100 & 9.759 & 0.798 & 0.000 & 0.429 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 150 & 4.481 & 1.202 & 0.070 & 0.248 & 0.890 & 85.200 & 3.000 & 8.217 & 0.825 & 0.000 & 0.394 \\
babylm-seqlen-opt-4096-warmup-v2 & 8 & 150 & 4.505 & 1.218 & 0.036 & 0.251 & 0.856 & 100.000 & 2.500 & 8.419 & 0.828 & -0.000 & 0.334 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 200 & 4.366 & 1.223 & 0.109 & 0.196 & 0.934 & 198.200 & 4.000 & 9.354 & 0.851 & -0.000 & 0.471 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 200 & 4.663 & 1.284 & 0.107 & 0.247 & 0.830 & 113.100 & 5.400 & 8.748 & 0.794 & 0.000 & 0.450 \\
babylm-seqlen-opt-4096-warmup-v2 & 8 & 200 & 4.446 & 1.166 & 0.114 & 0.183 & 0.841 & 154.400 & 3.300 & 8.978 & 0.781 & 0.000 & 0.416 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 250 & 4.366 & 1.207 & 0.129 & 0.159 & 0.838 & 245.300 & 5.200 & 9.399 & 0.865 & 0.000 & 0.508 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 250 & 4.434 & 1.283 & 0.141 & 0.181 & 0.938 & 254.000 & 5.700 & 9.094 & 0.863 & 0.000 & 0.614 \\
babylm-seqlen-opt-4096-warmup-v2 & 8 & 250 & 4.531 & 1.193 & 0.063 & 0.171 & 0.715 & 162.200 & 4.800 & 8.916 & 0.751 & -0.000 & 0.307 \\
\bottomrule
\end{tabular}
\caption{Average metrics per BabyLM setting with min--max normalized aggregate (NormAvg) across metrics.}
\label{tab:dialogue-metrics}
\end{table*}


==> tables/multi_turn_dialogs.tex <==
\begin{table*}[t]
\centering
\tiny
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lccccccccccccccccccccc}
\toprule
\textbf{BabyLM} & \textbf{Turns} & \textbf{Length} & \textbf{AvgSentLen} & \textbf{AoA} & \textbf{AddCon} & \textbf{CEFR} & \textbf{Overlap} & \textbf{CausalCon} & \textbf{TTR} & \textbf{ConceptDensity} & \textbf{VerbOverlap} & \textbf{AvgClauses} & \textbf{MATTR} & \textbf{AvgFam} & \textbf{Rep.} & \textbf{NumCon} & \textbf{AdversativeCon} & \textbf{Polysemy} & \textbf{VerbRep} & \textbf{Narrativity} & \textbf{NormAvg} \\
\midrule
cpo\_opt\_100M\_2048\_preprocess & 4 & 50 & 26.649 & 5.087 & 9.000 & 1.373 & 0.068 & 1.800 & 0.620 & 8.764 & 0.076 & 2.528 & 0.845 & 13.492 & 0.851 & 13.300 & 0.900 & 7.772 & 0.772 & 0.000 & 0.327 \\
cpo\_opt\_base & 4 & 50 & 25.612 & 5.214 & 9.100 & 1.468 & 0.074 & 1.000 & 0.590 & 9.039 & 0.089 & 2.387 & 0.826 & 13.221 & 0.881 & 13.100 & 0.900 & 7.241 & 0.684 & 0.000 & 0.310 \\
cpo\_opt\_cosmos & 4 & 50 & 31.545 & 5.067 & 10.600 & 1.383 & 0.052 & 2.000 & 0.638 & 10.082 & 0.073 & 2.767 & 0.858 & 13.565 & 0.912 & 14.200 & 1.700 & 8.115 & 0.792 & -0.000 & 0.336 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 50 & 35.133 & 5.011 & 10.000 & 1.408 & 0.044 & 2.400 & 0.624 & 10.357 & 0.073 & 3.213 & 0.871 & 13.875 & 0.946 & 15.600 & 1.600 & 8.118 & 0.790 & 0.000 & 0.388 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 4 & 50 & 33.436 & 4.813 & 8.600 & 1.325 & 0.044 & 2.600 & 0.627 & 9.616 & 0.057 & 3.205 & 0.874 & 13.958 & 0.803 & 16.100 & 1.300 & 9.121 & 0.622 & 0.000 & 0.324 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 4 & 50 & 31.883 & 4.802 & 10.100 & 1.371 & 0.053 & 1.800 & 0.610 & 9.272 & 0.077 & 2.839 & 0.847 & 13.846 & 0.870 & 16.500 & 1.600 & 8.488 & 0.773 & 0.000 & 0.354 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 4 & 50 & 32.883 & 4.782 & 7.600 & 1.305 & 0.082 & 1.800 & 0.606 & 9.761 & 0.067 & 3.733 & 0.849 & 13.972 & 0.904 & 13.600 & 1.500 & 8.769 & 0.822 & -0.000 & 0.372 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 4 & 50 & 27.302 & 4.951 & 8.500 & 1.328 & 0.062 & 1.500 & 0.599 & 8.157 & 0.079 & 2.747 & 0.821 & 13.825 & 0.887 & 13.400 & 1.300 & 7.826 & 0.759 & 0.000 & 0.352 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 4 & 50 & 35.471 & 4.819 & 9.100 & 1.328 & 0.056 & 2.000 & 0.572 & 9.558 & 0.057 & 2.845 & 0.831 & 13.946 & 0.909 & 13.800 & 1.300 & 8.635 & 0.863 & -0.000 & 0.358 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 4 & 50 & 31.042 & 4.948 & 9.100 & 1.331 & 0.062 & 1.700 & 0.620 & 9.478 & 0.068 & 3.011 & 0.847 & 13.817 & 0.942 & 14.400 & 1.000 & 8.725 & 0.750 & -0.000 & 0.354 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 4 & 50 & 24.330 & 4.929 & 10.000 & 1.322 & 0.063 & 1.000 & 0.596 & 7.521 & 0.061 & 2.371 & 0.836 & 13.859 & 0.867 & 15.000 & 1.700 & 7.667 & 0.666 & 0.000 & 0.307 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 50 & 50.143 & 4.523 & 13.700 & 1.219 & 0.046 & 2.200 & 0.464 & 7.037 & 0.107 & 3.798 & 0.740 & 14.401 & 0.797 & 18.100 & 1.600 & 9.379 & 0.753 & 0.000 & 0.342 \\
mamba-sam-seqlen-2048-original & 4 & 50 & 35.357 & 4.770 & 8.900 & 1.353 & 0.048 & 2.900 & 0.609 & 10.020 & 0.080 & 3.277 & 0.869 & 13.989 & 0.945 & 15.700 & 1.700 & 9.280 & 0.828 & 0.000 & 0.394 \\
opt-sam-orpo-mamba-2048-step448 & 4 & 50 & 37.152 & 4.887 & 9.400 & 1.376 & 0.072 & 2.800 & 0.617 & 10.105 & 0.084 & 3.153 & 0.867 & 13.926 & 0.918 & 16.800 & 1.900 & 8.294 & 0.797 & 0.000 & 0.403 \\
opt-sam-orpo-seqlen-2048-step559 & 4 & 50 & 33.302 & 4.948 & 11.000 & 1.365 & 0.052 & 1.000 & 0.615 & 9.601 & 0.059 & 2.682 & 0.855 & 13.739 & 0.866 & 15.100 & 1.400 & 8.926 & 0.590 & 0.000 & 0.308 \\
opt-sam-seqlen-2048-original & 4 & 50 & 29.592 & 4.843 & 9.900 & 1.318 & 0.052 & 2.500 & 0.618 & 8.939 & 0.069 & 3.107 & 0.849 & 13.855 & 0.942 & 17.000 & 1.900 & 8.893 & 0.866 & 0.000 & 0.385 \\
orpo\_opt\_100M\_2048\_preprocess & 4 & 50 & 33.325 & 5.123 & 10.400 & 1.415 & 0.078 & 1.600 & 0.582 & 9.806 & 0.086 & 2.865 & 0.806 & 13.431 & 0.777 & 14.300 & 1.100 & 7.963 & 0.814 & 0.000 & 0.331 \\
orpo\_opt\_cosmos & 4 & 50 & 24.685 & 5.200 & 6.900 & 1.459 & 0.067 & 1.400 & 0.624 & 8.824 & 0.066 & 2.603 & 0.853 & 13.503 & 0.822 & 10.300 & 1.500 & 7.632 & 0.645 & 0.000 & 0.308 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 50 & 37.582 & 4.813 & 11.500 & 1.343 & 0.066 & 2.400 & 0.604 & 10.495 & 0.101 & 3.789 & 0.855 & 14.103 & 0.898 & 17.900 & 1.700 & 8.916 & 0.763 & 0.000 & 0.388 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 50 & 42.143 & 4.487 & 8.800 & 1.228 & 0.075 & 1.600 & 0.473 & 6.737 & 0.136 & 2.726 & 0.763 & 14.346 & 0.879 & 11.500 & 1.400 & 8.631 & 0.720 & -0.000 & 0.313 \\
babylm-seqlen-opt-1024-warmup-v2 & 4 & 50 & 41.648 & 4.864 & 11.200 & 1.343 & 0.057 & 1.700 & 0.594 & 10.951 & 0.056 & 2.981 & 0.844 & 13.768 & 0.925 & 16.500 & 1.600 & 8.589 & 0.827 & 0.000 & 0.372 \\
babylm-seqlen-opt-4096-warmup-v2 & 4 & 50 & 51.757 & 4.487 & 12.500 & 1.172 & 0.030 & 1.600 & 0.449 & 6.699 & 0.076 & 2.669 & 0.732 & 14.489 & 0.867 & 17.100 & 1.000 & 8.662 & 0.677 & -0.000 & 0.268 \\
cpo\_opt\_100M\_2048\_preprocess & 4 & 100 & 48.849 & 5.028 & 16.100 & 1.417 & 0.121 & 3.000 & 0.508 & 13.440 & 0.117 & 3.630 & 0.795 & 13.620 & 0.931 & 23.400 & 2.300 & 7.776 & 0.857 & 0.000 & 0.417 \\
cpo\_opt\_base & 4 & 100 & 22.647 & 5.075 & 16.000 & 1.404 & 0.088 & 1.800 & 0.496 & 7.749 & 0.070 & 2.658 & 0.798 & 13.511 & 0.847 & 21.000 & 1.300 & 8.294 & 0.715 & 0.000 & 0.318 \\
cpo\_opt\_cosmos & 4 & 100 & 47.333 & 5.196 & 16.900 & 1.458 & 0.075 & 2.700 & 0.540 & 14.637 & 0.072 & 3.888 & 0.811 & 13.509 & 0.876 & 25.100 & 1.500 & 8.216 & 0.796 & -0.000 & 0.367 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 100 & 51.051 & 4.921 & 22.200 & 1.353 & 0.062 & 4.500 & 0.537 & 15.123 & 0.056 & 4.570 & 0.831 & 14.021 & 0.955 & 35.900 & 3.300 & 9.218 & 0.839 & -0.000 & 0.430 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 4 & 100 & 59.530 & 4.974 & 16.600 & 1.391 & 0.069 & 3.500 & 0.548 & 14.860 & 0.083 & 4.200 & 0.825 & 13.774 & 0.879 & 29.800 & 2.800 & 8.771 & 0.791 & 0.000 & 0.400 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 4 & 100 & 55.903 & 4.888 & 19.900 & 1.374 & 0.082 & 2.600 & 0.523 & 14.268 & 0.097 & 4.628 & 0.812 & 13.966 & 0.817 & 31.700 & 2.100 & 8.968 & 0.717 & 0.000 & 0.379 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 4 & 100 & 60.866 & 4.900 & 20.900 & 1.365 & 0.083 & 4.400 & 0.522 & 14.470 & 0.085 & 4.327 & 0.819 & 14.008 & 0.903 & 33.600 & 4.200 & 9.265 & 0.825 & 0.000 & 0.447 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 4 & 100 & 42.838 & 4.934 & 17.000 & 1.350 & 0.045 & 2.700 & 0.526 & 12.472 & 0.070 & 3.683 & 0.804 & 13.916 & 0.906 & 26.400 & 2.000 & 8.090 & 0.876 & 0.000 & 0.383 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 4 & 100 & 35.580 & 4.984 & 17.100 & 1.395 & 0.063 & 2.600 & 0.524 & 10.134 & 0.067 & 3.734 & 0.811 & 13.837 & 0.905 & 25.700 & 2.600 & 8.415 & 0.826 & -0.000 & 0.373 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 4 & 100 & 25.115 & 4.954 & 14.900 & 1.367 & 0.076 & 2.500 & 0.513 & 8.005 & 0.058 & 2.664 & 0.803 & 13.792 & 0.844 & 21.900 & 2.000 & 8.098 & 0.671 & 0.000 & 0.317 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 4 & 100 & 36.532 & 4.847 & 17.500 & 1.353 & 0.092 & 3.600 & 0.513 & 9.663 & 0.122 & 3.335 & 0.808 & 13.862 & 0.884 & 27.400 & 2.100 & 8.416 & 0.752 & 0.000 & 0.380 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 100 & 67.795 & 4.532 & 24.300 & 1.224 & 0.058 & 3.100 & 0.391 & 9.693 & 0.120 & 3.674 & 0.721 & 14.390 & 0.891 & 33.300 & 3.000 & 9.435 & 0.821 & 0.000 & 0.373 \\
mamba-sam-seqlen-2048-original & 4 & 100 & 84.157 & 4.770 & 24.900 & 1.406 & 0.118 & 6.200 & 0.501 & 18.036 & 0.141 & 5.356 & 0.796 & 14.105 & 0.956 & 40.900 & 4.700 & 8.543 & 0.788 & -0.000 & 0.478 \\
opt-sam-orpo-mamba-2048-step448 & 4 & 100 & 99.104 & 4.797 & 25.000 & 1.390 & 0.099 & 7.400 & 0.514 & 20.593 & 0.134 & 5.443 & 0.811 & 14.065 & 0.799 & 42.100 & 5.400 & 9.338 & 0.870 & -0.000 & 0.486 \\
opt-sam-orpo-seqlen-2048-step559 & 4 & 100 & 53.356 & 4.728 & 26.100 & 1.304 & 0.077 & 5.500 & 0.512 & 12.973 & 0.119 & 4.463 & 0.810 & 14.172 & 0.893 & 40.100 & 3.800 & 9.944 & 0.844 & -0.000 & 0.426 \\
opt-sam-seqlen-2048-original & 4 & 100 & 82.179 & 4.917 & 20.300 & 1.439 & 0.089 & 4.300 & 0.523 & 21.515 & 0.074 & 4.929 & 0.827 & 13.847 & 0.904 & 35.500 & 3.000 & 9.314 & 0.796 & -0.000 & 0.434 \\
orpo\_opt\_100M\_2048\_preprocess & 4 & 100 & 36.023 & 5.021 & 14.900 & 1.419 & 0.085 & 2.400 & 0.524 & 11.905 & 0.092 & 3.366 & 0.802 & 13.182 & 0.862 & 20.300 & 0.800 & 8.210 & 0.851 & 0.000 & 0.361 \\
orpo\_opt\_cosmos & 4 & 100 & 54.220 & 5.211 & 17.500 & 1.443 & 0.091 & 3.000 & 0.532 & 14.989 & 0.074 & 4.299 & 0.819 & 13.629 & 0.866 & 26.100 & 2.000 & 7.734 & 0.851 & -0.000 & 0.392 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 100 & 41.250 & 4.953 & 21.300 & 1.365 & 0.068 & 4.600 & 0.534 & 11.484 & 0.071 & 3.941 & 0.828 & 13.991 & 0.909 & 35.200 & 3.300 & 8.949 & 0.778 & -0.000 & 0.400 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 100 & 42.025 & 4.711 & 14.700 & 1.262 & 0.062 & 2.200 & 0.419 & 7.984 & 0.081 & 3.018 & 0.737 & 14.108 & 0.870 & 19.600 & 1.400 & 8.710 & 0.768 & -0.000 & 0.309 \\
babylm-seqlen-opt-1024-warmup-v2 & 4 & 100 & 73.212 & 4.878 & 25.800 & 1.342 & 0.110 & 5.000 & 0.493 & 17.239 & 0.122 & 4.636 & 0.795 & 14.010 & 0.847 & 38.800 & 3.300 & 9.587 & 0.867 & -0.000 & 0.446 \\
babylm-seqlen-opt-4096-warmup-v2 & 4 & 100 & 84.967 & 4.378 & 27.200 & 1.189 & 0.067 & 2.200 & 0.341 & 8.322 & 0.149 & 2.531 & 0.613 & 14.515 & 0.770 & 35.000 & 2.900 & 8.478 & 0.793 & -0.000 & 0.294 \\
cpo\_opt\_100M\_2048\_preprocess & 4 & 150 & 36.181 & 5.057 & 22.900 & 1.441 & 0.115 & 4.400 & 0.469 & 11.928 & 0.119 & 3.914 & 0.802 & 13.377 & 0.828 & 33.400 & 1.200 & 7.582 & 0.708 & -0.000 & 0.352 \\
cpo\_opt\_base & 4 & 150 & 28.543 & 5.153 & 24.400 & 1.433 & 0.082 & 4.000 & 0.458 & 9.831 & 0.072 & 2.832 & 0.806 & 13.475 & 0.883 & 34.500 & 1.700 & 8.358 & 0.837 & -0.000 & 0.356 \\
cpo\_opt\_cosmos & 4 & 150 & 64.949 & 5.174 & 21.200 & 1.460 & 0.076 & 6.100 & 0.488 & 15.448 & 0.111 & 4.766 & 0.800 & 13.609 & 0.894 & 33.800 & 3.400 & 7.571 & 0.748 & 0.000 & 0.416 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 150 & 108.381 & 4.912 & 31.800 & 1.360 & 0.104 & 7.900 & 0.445 & 24.370 & 0.137 & 5.796 & 0.792 & 14.135 & 0.959 & 52.600 & 5.000 & 9.865 & 0.852 & 0.000 & 0.539 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 4 & 150 & 70.803 & 4.893 & 27.200 & 1.360 & 0.092 & 6.600 & 0.469 & 16.508 & 0.141 & 4.306 & 0.805 & 14.053 & 0.896 & 43.200 & 3.200 & 9.341 & 0.819 & 0.000 & 0.466 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 4 & 150 & 82.873 & 4.923 & 29.400 & 1.418 & 0.105 & 5.300 & 0.467 & 20.425 & 0.076 & 5.250 & 0.776 & 13.885 & 0.936 & 45.100 & 3.000 & 9.136 & 0.847 & 0.000 & 0.494 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 4 & 150 & 47.567 & 4.949 & 26.400 & 1.353 & 0.109 & 4.700 & 0.439 & 11.499 & 0.077 & 4.102 & 0.768 & 13.941 & 0.901 & 40.200 & 3.700 & 8.797 & 0.768 & 0.000 & 0.401 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 4 & 150 & 27.115 & 5.055 & 23.600 & 1.350 & 0.083 & 3.500 & 0.448 & 8.346 & 0.074 & 3.031 & 0.777 & 13.763 & 0.889 & 33.300 & 2.600 & 8.742 & 0.717 & -0.000 & 0.320 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 4 & 150 & 45.635 & 4.989 & 22.500 & 1.379 & 0.114 & 4.900 & 0.443 & 11.629 & 0.096 & 3.901 & 0.780 & 13.904 & 0.870 & 34.600 & 2.100 & 8.785 & 0.765 & 0.000 & 0.395 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 4 & 150 & 44.850 & 4.983 & 23.700 & 1.375 & 0.081 & 4.100 & 0.499 & 13.261 & 0.085 & 3.459 & 0.798 & 13.837 & 0.894 & 35.000 & 1.900 & 8.627 & 0.716 & 0.000 & 0.374 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 4 & 150 & 44.859 & 4.901 & 26.300 & 1.380 & 0.070 & 5.000 & 0.470 & 10.916 & 0.075 & 3.912 & 0.803 & 13.947 & 0.862 & 40.900 & 3.600 & 8.410 & 0.760 & -0.000 & 0.365 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 150 & 102.911 & 4.385 & 39.400 & 1.256 & 0.128 & 3.200 & 0.302 & 10.511 & 0.166 & 3.824 & 0.593 & 14.596 & 0.749 & 49.200 & 3.600 & 9.345 & 0.775 & 0.000 & 0.387 \\
mamba-sam-seqlen-2048-original & 4 & 150 & 98.532 & 4.918 & 35.000 & 1.435 & 0.075 & 8.300 & 0.470 & 20.364 & 0.081 & 6.956 & 0.766 & 14.073 & 0.906 & 55.800 & 5.500 & 9.043 & 0.816 & -0.000 & 0.484 \\
opt-sam-orpo-mamba-2048-step448 & 4 & 150 & 81.335 & 4.880 & 39.800 & 1.384 & 0.073 & 11.200 & 0.470 & 18.986 & 0.106 & 6.443 & 0.818 & 14.149 & 0.870 & 64.800 & 7.600 & 9.414 & 0.783 & -0.000 & 0.502 \\
opt-sam-orpo-seqlen-2048-step559 & 4 & 150 & 40.771 & 4.910 & 31.900 & 1.371 & 0.069 & 4.700 & 0.473 & 11.898 & 0.095 & 4.271 & 0.808 & 13.991 & 0.921 & 47.300 & 3.500 & 8.704 & 0.787 & -0.000 & 0.409 \\
opt-sam-seqlen-2048-original & 4 & 150 & 55.269 & 4.998 & 28.900 & 1.416 & 0.117 & 6.100 & 0.466 & 14.362 & 0.122 & 4.435 & 0.814 & 13.753 & 0.913 & 45.500 & 1.800 & 9.115 & 0.789 & 0.000 & 0.455 \\
orpo\_opt\_100M\_2048\_preprocess & 4 & 150 & 45.304 & 5.169 & 24.900 & 1.432 & 0.109 & 3.200 & 0.473 & 12.655 & 0.122 & 4.215 & 0.794 & 13.519 & 0.766 & 33.300 & 1.600 & 8.092 & 0.722 & 0.000 & 0.372 \\
orpo\_opt\_cosmos & 4 & 150 & 41.515 & 5.284 & 19.500 & 1.489 & 0.102 & 2.900 & 0.507 & 14.017 & 0.092 & 3.589 & 0.806 & 13.375 & 0.847 & 27.000 & 1.500 & 8.097 & 0.797 & -0.000 & 0.380 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 150 & 67.041 & 5.077 & 51.500 & 1.395 & 0.076 & 6.400 & 0.474 & 17.192 & 0.103 & 4.861 & 0.793 & 13.884 & 0.825 & 69.600 & 4.500 & 8.858 & 0.815 & -0.000 & 0.429 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 150 & 39.839 & 4.732 & 30.600 & 1.301 & 0.078 & 3.500 & 0.391 & 7.168 & 0.071 & 3.140 & 0.730 & 14.165 & 0.855 & 37.700 & 2.500 & 8.890 & 0.724 & -0.000 & 0.325 \\
babylm-seqlen-opt-1024-warmup-v2 & 4 & 150 & 116.109 & 4.778 & 33.300 & 1.351 & 0.098 & 7.400 & 0.441 & 22.476 & 0.131 & 7.351 & 0.807 & 14.157 & 0.903 & 55.800 & 4.300 & 9.446 & 0.820 & -0.000 & 0.497 \\
babylm-seqlen-opt-4096-warmup-v2 & 4 & 150 & 80.458 & 4.473 & 41.100 & 1.222 & 0.032 & 3.900 & 0.355 & 8.615 & 0.086 & 2.775 & 0.677 & 14.348 & 0.900 & 50.300 & 3.200 & 9.304 & 0.779 & 0.000 & 0.335 \\
cpo\_opt\_100M\_2048\_preprocess & 4 & 200 & 47.506 & 5.171 & 28.000 & 0.932 & 0.108 & 4.900 & 0.432 & 14.398 & 0.103 & 4.454 & 0.783 & 13.663 & 0.904 & 40.300 & 3.100 & 8.410 & 0.767 & -0.000 & 0.370 \\
cpo\_opt\_base & 4 & 200 & 24.663 & 5.378 & 30.600 & 1.506 & 0.099 & 4.500 & 0.433 & 9.025 & 0.047 & 2.724 & 0.794 & 13.324 & 0.882 & 41.500 & 0.900 & 7.803 & 0.738 & -0.000 & 0.334 \\
cpo\_opt\_cosmos & 4 & 200 & 68.586 & 5.191 & 33.000 & 1.270 & 0.130 & 7.900 & 0.435 & 15.983 & 0.121 & 3.610 & 0.793 & 13.749 & 0.933 & 50.800 & 3.500 & 8.165 & 0.868 & -0.000 & 0.440 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 200 & 133.245 & 4.960 & 45.300 & 1.394 & 0.105 & 8.100 & 0.427 & 27.561 & 0.115 & 8.904 & 0.732 & 13.997 & 0.891 & 67.500 & 4.300 & 9.388 & 0.823 & -0.000 & 0.526 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 4 & 200 & 97.072 & 4.827 & 41.000 & 1.345 & 0.113 & 5.800 & 0.430 & 19.744 & 0.153 & 6.578 & 0.763 & 14.008 & 0.946 & 59.900 & 5.300 & 9.482 & 0.862 & -0.000 & 0.513 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 4 & 200 & 97.373 & 4.952 & 40.200 & 1.391 & 0.061 & 7.200 & 0.419 & 19.274 & 0.068 & 6.760 & 0.746 & 13.959 & 0.874 & 58.100 & 3.200 & 9.061 & 0.795 & 0.000 & 0.452 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 4 & 200 & 97.831 & 5.184 & 40.000 & 1.474 & 0.115 & 8.200 & 0.434 & 20.974 & 0.091 & 5.105 & 0.781 & 13.664 & 0.873 & 60.400 & 3.500 & 8.268 & 0.800 & -0.000 & 0.455 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 4 & 200 & 35.098 & 4.899 & 29.400 & 1.337 & 0.071 & 6.500 & 0.469 & 10.400 & 0.096 & 3.705 & 0.795 & 13.860 & 0.872 & 44.300 & 3.200 & 8.790 & 0.730 & -0.000 & 0.366 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 4 & 200 & 46.844 & 5.025 & 35.000 & 1.387 & 0.093 & 4.400 & 0.441 & 11.659 & 0.085 & 4.477 & 0.798 & 13.840 & 0.904 & 50.500 & 3.700 & 8.466 & 0.833 & -0.000 & 0.417 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 4 & 200 & 29.901 & 5.006 & 31.600 & 1.444 & 0.068 & 3.900 & 0.454 & 9.793 & 0.060 & 3.258 & 0.798 & 13.721 & 0.887 & 43.300 & 3.200 & 7.894 & 0.706 & -0.000 & 0.325 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 4 & 200 & 34.534 & 5.163 & 36.100 & 1.257 & 0.083 & 4.200 & 0.453 & 11.543 & 0.123 & 3.777 & 0.794 & 13.467 & 0.875 & 50.100 & 4.400 & 7.789 & 0.786 & 0.000 & 0.381 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 200 & 188.465 & 4.367 & 89.200 & 1.188 & 0.082 & 7.600 & 0.245 & 14.528 & 0.173 & 3.708 & 0.525 & 14.752 & 0.770 & 102.700 & 3.000 & 9.584 & 0.875 & -0.000 & 0.409 \\
mamba-sam-seqlen-2048-original & 4 & 200 & 174.490 & 4.967 & 52.300 & 1.547 & 0.108 & 7.700 & 0.430 & 34.877 & 0.116 & 5.895 & 0.731 & 13.880 & 0.819 & 73.800 & 8.200 & 8.868 & 0.779 & 0.000 & 0.530 \\
opt-sam-orpo-mamba-2048-step448 & 4 & 200 & 164.789 & 5.049 & 47.100 & 1.435 & 0.095 & 11.300 & 0.438 & 30.892 & 0.145 & 6.019 & 0.772 & 13.997 & 0.853 & 76.100 & 7.200 & 9.044 & 0.839 & 0.000 & 0.569 \\
opt-sam-orpo-seqlen-2048-step559 & 4 & 200 & 105.132 & 4.825 & 41.200 & 1.152 & 0.090 & 8.100 & 0.456 & 23.545 & 0.104 & 5.306 & 0.784 & 13.945 & 0.829 & 62.500 & 5.100 & 9.511 & 0.872 & 0.000 & 0.479 \\
opt-sam-seqlen-2048-original & 4 & 200 & 91.975 & 4.947 & 36.600 & 1.384 & 0.073 & 8.500 & 0.456 & 21.103 & 0.086 & 5.612 & 0.793 & 14.027 & 0.841 & 59.800 & 3.300 & 9.724 & 0.825 & 0.000 & 0.465 \\
orpo\_opt\_100M\_2048\_preprocess & 4 & 200 & 29.878 & 5.080 & 27.500 & 1.198 & 0.100 & 5.600 & 0.463 & 10.060 & 0.100 & 3.136 & 0.795 & 13.530 & 0.928 & 39.000 & 3.600 & 8.636 & 0.797 & -0.000 & 0.385 \\
orpo\_opt\_cosmos & 4 & 200 & 33.851 & 5.417 & 31.300 & 1.546 & 0.074 & 4.300 & 0.478 & 12.225 & 0.065 & 3.291 & 0.811 & 13.412 & 0.854 & 43.100 & 3.200 & 7.906 & 0.842 & -0.000 & 0.388 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 200 & 89.349 & 5.047 & 49.400 & 0.888 & 0.094 & 8.100 & 0.438 & 20.531 & 0.101 & 5.535 & 0.784 & 13.947 & 0.948 & 71.000 & 4.000 & 8.855 & 0.854 & -0.000 & 0.452 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 200 & 76.995 & 4.533 & 56.700 & 1.340 & 0.122 & 4.300 & 0.306 & 9.178 & 0.145 & 2.711 & 0.612 & 14.225 & 0.808 & 65.100 & 2.600 & 8.758 & 0.788 & 0.000 & 0.368 \\
babylm-seqlen-opt-1024-warmup-v2 & 4 & 200 & 103.452 & 5.010 & 53.700 & 1.410 & 0.072 & 7.900 & 0.436 & 21.011 & 0.080 & 5.224 & 0.772 & 13.869 & 0.952 & 75.800 & 4.400 & 9.447 & 0.804 & -0.000 & 0.478 \\
babylm-seqlen-opt-4096-warmup-v2 & 4 & 200 & 153.182 & 4.418 & 60.000 & 1.164 & 0.042 & 6.100 & 0.268 & 12.451 & 0.105 & 3.435 & 0.507 & 14.641 & 0.750 & 70.400 & 1.900 & 8.675 & 0.764 & 0.000 & 0.315 \\
cpo\_opt\_100M\_2048\_preprocess & 4 & 250 & 76.486 & 5.054 & 41.900 & 1.393 & 0.125 & 8.300 & 0.396 & 17.633 & 0.135 & 5.052 & 0.733 & 13.711 & 0.950 & 57.700 & 2.500 & 8.453 & 0.827 & 0.000 & 0.476 \\
cpo\_opt\_base & 4 & 250 & 37.526 & 5.655 & 34.600 & 1.647 & 0.108 & 3.900 & 0.411 & 11.165 & 0.092 & 3.200 & 0.748 & 13.392 & 0.835 & 47.300 & 3.000 & 7.798 & 0.780 & -0.000 & 0.391 \\
cpo\_opt\_cosmos & 4 & 250 & 80.139 & 5.124 & 42.200 & 1.435 & 0.104 & 6.400 & 0.419 & 18.616 & 0.104 & 5.100 & 0.769 & 13.702 & 0.855 & 61.500 & 5.500 & 8.321 & 0.752 & -0.000 & 0.432 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 250 & 109.418 & 4.932 & 53.400 & 1.391 & 0.103 & 8.900 & 0.411 & 23.573 & 0.125 & 7.233 & 0.794 & 14.018 & 0.819 & 80.200 & 7.300 & 9.086 & 0.855 & 0.000 & 0.532 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 4 & 250 & 66.742 & 5.149 & 43.100 & 1.467 & 0.104 & 6.000 & 0.399 & 15.570 & 0.087 & 5.694 & 0.756 & 13.580 & 0.910 & 60.400 & 2.900 & 8.551 & 0.805 & -0.000 & 0.432 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 4 & 250 & 29.468 & 4.927 & 38.300 & 1.378 & 0.099 & 5.800 & 0.396 & 8.501 & 0.106 & 3.049 & 0.753 & 13.931 & 0.840 & 55.800 & 5.800 & 9.602 & 0.653 & 0.000 & 0.386 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 4 & 250 & 81.728 & 4.898 & 42.000 & 1.375 & 0.140 & 7.600 & 0.409 & 16.024 & 0.149 & 4.004 & 0.733 & 13.995 & 0.805 & 60.800 & 4.900 & 9.658 & 0.855 & 0.000 & 0.474 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 4 & 250 & 62.019 & 5.029 & 44.900 & 1.427 & 0.092 & 10.700 & 0.387 & 14.662 & 0.086 & 3.914 & 0.780 & 13.896 & 0.887 & 66.900 & 5.800 & 8.251 & 0.719 & -0.000 & 0.423 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 4 & 250 & 53.963 & 5.183 & 41.600 & 1.434 & 0.095 & 7.400 & 0.419 & 13.664 & 0.078 & 3.673 & 0.766 & 13.761 & 0.838 & 59.000 & 3.100 & 8.245 & 0.761 & 0.000 & 0.412 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 4 & 250 & 28.966 & 5.007 & 33.700 & 1.391 & 0.101 & 5.200 & 0.409 & 9.020 & 0.075 & 2.831 & 0.757 & 13.849 & 0.839 & 48.600 & 3.600 & 8.467 & 0.727 & 0.000 & 0.367 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 4 & 250 & 114.437 & 5.016 & 45.200 & 0.910 & 0.155 & 8.400 & 0.370 & 19.417 & 0.147 & 6.853 & 0.719 & 13.841 & 0.911 & 68.100 & 4.700 & 8.382 & 0.860 & 0.000 & 0.490 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 250 & 89.015 & 4.632 & 66.500 & 1.245 & 0.094 & 5.000 & 0.286 & 9.951 & 0.144 & 3.424 & 0.626 & 14.430 & 0.891 & 78.300 & 2.500 & 9.265 & 0.794 & 0.000 & 0.401 \\
mamba-sam-seqlen-2048-original & 4 & 250 & 175.872 & 4.836 & 67.500 & 1.413 & 0.100 & 12.100 & 0.411 & 31.918 & 0.116 & 5.291 & 0.764 & 14.108 & 0.869 & 100.300 & 10.300 & 9.417 & 0.858 & -0.000 & 0.567 \\
opt-sam-orpo-mamba-2048-step448 & 4 & 250 & 219.538 & 4.777 & 68.700 & 1.140 & 0.126 & 17.600 & 0.388 & 37.041 & 0.179 & 5.779 & 0.747 & 14.147 & 0.778 & 108.300 & 12.200 & 8.808 & 0.877 & -0.000 & 0.597 \\
opt-sam-orpo-seqlen-2048-step559 & 4 & 250 & 59.532 & 5.091 & 42.700 & 1.454 & 0.092 & 10.100 & 0.407 & 13.267 & 0.078 & 4.055 & 0.787 & 13.753 & 0.861 & 67.500 & 5.600 & 8.867 & 0.791 & -0.000 & 0.438 \\
opt-sam-seqlen-2048-original & 4 & 250 & 89.471 & 4.997 & 48.400 & 1.439 & 0.116 & 8.700 & 0.401 & 17.007 & 0.113 & 4.923 & 0.781 & 13.776 & 0.907 & 71.200 & 5.900 & 8.697 & 0.834 & 0.000 & 0.492 \\
orpo\_opt\_100M\_2048\_preprocess & 4 & 250 & 55.255 & 5.160 & 35.600 & 1.247 & 0.101 & 5.600 & 0.424 & 16.513 & 0.099 & 4.485 & 0.783 & 13.528 & 0.897 & 47.700 & 4.100 & 8.531 & 0.830 & 0.000 & 0.432 \\
orpo\_opt\_cosmos & 4 & 250 & 37.789 & 5.386 & 33.300 & 1.497 & 0.120 & 5.400 & 0.436 & 11.985 & 0.103 & 3.751 & 0.788 & 13.499 & 0.844 & 47.600 & 3.000 & 7.614 & 0.824 & -0.000 & 0.402 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 4 & 250 & 147.296 & 5.073 & 64.700 & 1.197 & 0.096 & 8.100 & 0.412 & 31.001 & 0.105 & 7.536 & 0.754 & 13.846 & 0.888 & 90.700 & 8.200 & 9.247 & 0.846 & 0.000 & 0.548 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 4 & 250 & 53.894 & 4.741 & 38.200 & 1.391 & 0.117 & 5.700 & 0.318 & 8.424 & 0.144 & 3.100 & 0.676 & 14.188 & 0.810 & 49.500 & 3.900 & 7.859 & 0.794 & -0.000 & 0.357 \\
babylm-seqlen-opt-1024-warmup-v2 & 4 & 250 & 110.928 & 4.977 & 50.300 & 1.426 & 0.077 & 6.400 & 0.429 & 23.477 & 0.087 & 7.182 & 0.762 & 13.686 & 0.905 & 71.000 & 4.000 & 8.592 & 0.823 & 0.000 & 0.493 \\
babylm-seqlen-opt-4096-warmup-v2 & 4 & 250 & 105.623 & 4.549 & 68.000 & 1.223 & 0.070 & 3.500 & 0.266 & 8.857 & 0.148 & 5.175 & 0.532 & 14.537 & 0.922 & 79.400 & 3.300 & 9.127 & 0.816 & 0.000 & 0.408 \\
cpo\_opt\_100M\_2048\_preprocess & 6 & 50 & 24.654 & 5.071 & 12.200 & 1.423 & 0.065 & 2.300 & 0.564 & 8.720 & 0.074 & 2.547 & 0.840 & 13.478 & 0.830 & 19.000 & 2.500 & 8.146 & 0.740 & 0.000 & 0.326 \\
cpo\_opt\_base & 6 & 50 & 25.556 & 5.022 & 11.700 & 1.355 & 0.057 & 2.100 & 0.549 & 8.178 & 0.066 & 2.712 & 0.819 & 13.636 & 0.891 & 18.400 & 1.800 & 8.236 & 0.766 & -0.000 & 0.326 \\
cpo\_opt\_cosmos & 6 & 50 & 29.026 & 5.123 & 14.400 & 1.457 & 0.049 & 2.000 & 0.560 & 9.433 & 0.060 & 2.633 & 0.833 & 13.279 & 0.912 & 20.300 & 2.100 & 7.358 & 0.745 & -0.000 & 0.316 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 50 & 41.064 & 4.947 & 15.100 & 1.405 & 0.050 & 3.400 & 0.563 & 12.358 & 0.041 & 3.686 & 0.859 & 13.936 & 0.911 & 25.900 & 1.800 & 8.552 & 0.745 & 0.000 & 0.373 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 6 & 50 & 33.399 & 4.898 & 14.100 & 1.350 & 0.050 & 3.300 & 0.554 & 9.763 & 0.041 & 3.165 & 0.858 & 14.057 & 0.915 & 23.400 & 2.600 & 8.527 & 0.796 & 0.000 & 0.382 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 6 & 50 & 48.080 & 4.812 & 14.100 & 1.341 & 0.067 & 3.200 & 0.543 & 12.932 & 0.073 & 3.898 & 0.834 & 14.109 & 0.922 & 25.200 & 1.200 & 9.002 & 0.845 & 0.000 & 0.418 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 6 & 50 & 30.366 & 4.812 & 12.600 & 1.337 & 0.083 & 2.600 & 0.531 & 9.063 & 0.096 & 3.148 & 0.839 & 13.883 & 0.893 & 20.300 & 1.100 & 8.223 & 0.722 & 0.000 & 0.352 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 6 & 50 & 33.925 & 4.882 & 14.900 & 1.339 & 0.057 & 2.700 & 0.536 & 9.983 & 0.058 & 3.060 & 0.841 & 13.994 & 0.938 & 22.700 & 2.400 & 9.117 & 0.678 & 0.000 & 0.355 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 6 & 50 & 30.896 & 4.886 & 12.600 & 1.333 & 0.064 & 3.000 & 0.528 & 8.890 & 0.061 & 2.855 & 0.826 & 13.854 & 0.929 & 22.600 & 2.100 & 8.392 & 0.800 & 0.000 & 0.356 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 6 & 50 & 29.773 & 4.846 & 13.400 & 1.331 & 0.036 & 2.900 & 0.557 & 8.992 & 0.061 & 3.073 & 0.850 & 13.996 & 0.916 & 21.300 & 1.700 & 8.521 & 0.740 & 0.000 & 0.346 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 6 & 50 & 30.939 & 4.982 & 15.600 & 1.373 & 0.069 & 2.200 & 0.541 & 9.244 & 0.091 & 3.097 & 0.836 & 13.886 & 0.853 & 23.000 & 2.000 & 7.914 & 0.754 & -0.000 & 0.335 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 50 & 52.442 & 4.525 & 15.700 & 1.231 & 0.094 & 3.100 & 0.411 & 8.287 & 0.123 & 3.166 & 0.752 & 14.379 & 0.921 & 22.500 & 1.600 & 8.597 & 0.787 & -0.000 & 0.348 \\
mamba-sam-seqlen-2048-original & 6 & 50 & 49.566 & 4.881 & 18.700 & 1.325 & 0.059 & 4.100 & 0.558 & 12.501 & 0.085 & 3.403 & 0.853 & 13.962 & 0.969 & 29.200 & 3.100 & 9.034 & 0.832 & -0.000 & 0.419 \\
opt-sam-orpo-mamba-2048-step448 & 6 & 50 & 50.604 & 4.831 & 15.100 & 1.369 & 0.084 & 3.700 & 0.553 & 12.953 & 0.083 & 3.492 & 0.851 & 13.975 & 0.912 & 24.200 & 3.500 & 9.184 & 0.758 & 0.000 & 0.412 \\
opt-sam-orpo-seqlen-2048-step559 & 6 & 50 & 49.101 & 5.072 & 14.900 & 1.382 & 0.055 & 4.500 & 0.576 & 14.237 & 0.075 & 3.843 & 0.852 & 13.900 & 0.868 & 25.400 & 2.300 & 9.109 & 0.778 & 0.000 & 0.420 \\
opt-sam-seqlen-2048-original & 6 & 50 & 42.333 & 4.858 & 14.100 & 1.323 & 0.052 & 3.000 & 0.551 & 12.123 & 0.054 & 3.824 & 0.837 & 14.009 & 0.932 & 24.500 & 2.100 & 8.350 & 0.762 & -0.000 & 0.354 \\
orpo\_opt\_100M\_2048\_preprocess & 6 & 50 & 30.130 & 5.145 & 12.800 & 1.411 & 0.082 & 1.700 & 0.546 & 10.085 & 0.098 & 2.647 & 0.842 & 13.508 & 0.865 & 18.400 & 0.700 & 7.507 & 0.817 & 0.000 & 0.353 \\
orpo\_opt\_cosmos & 6 & 50 & 26.178 & 5.375 & 12.700 & 1.514 & 0.055 & 1.400 & 0.564 & 8.791 & 0.030 & 2.413 & 0.822 & 13.298 & 0.858 & 17.600 & 0.500 & 6.911 & 0.740 & -0.000 & 0.277 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 50 & 37.211 & 4.951 & 17.200 & 1.390 & 0.065 & 3.300 & 0.567 & 11.240 & 0.071 & 3.354 & 0.866 & 13.864 & 0.927 & 26.100 & 2.400 & 8.366 & 0.744 & -0.000 & 0.369 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 50 & 43.884 & 4.612 & 13.600 & 1.234 & 0.061 & 2.600 & 0.419 & 8.086 & 0.132 & 3.602 & 0.741 & 14.326 & 0.907 & 19.000 & 2.000 & 9.567 & 0.793 & -0.000 & 0.354 \\
babylm-seqlen-opt-1024-warmup-v2 & 6 & 50 & 38.328 & 4.864 & 16.100 & 1.339 & 0.038 & 2.400 & 0.543 & 10.812 & 0.071 & 3.794 & 0.841 & 13.939 & 0.901 & 25.300 & 2.500 & 8.834 & 0.774 & -0.000 & 0.353 \\
babylm-seqlen-opt-4096-warmup-v2 & 6 & 50 & 48.956 & 4.478 & 14.800 & 1.197 & 0.029 & 2.400 & 0.408 & 7.644 & 0.115 & 2.742 & 0.734 & 14.430 & 0.803 & 22.100 & 1.300 & 8.928 & 0.643 & -0.000 & 0.254 \\
cpo\_opt\_100M\_2048\_preprocess & 6 & 100 & 33.151 & 5.093 & 24.400 & 1.437 & 0.090 & 5.800 & 0.483 & 10.351 & 0.081 & 3.358 & 0.806 & 13.509 & 0.858 & 36.100 & 1.600 & 8.253 & 0.776 & 0.000 & 0.384 \\
cpo\_opt\_base & 6 & 100 & 28.475 & 5.035 & 26.300 & 1.429 & 0.080 & 5.200 & 0.489 & 8.843 & 0.067 & 2.961 & 0.822 & 13.683 & 0.892 & 38.500 & 2.500 & 8.295 & 0.780 & -0.000 & 0.368 \\
cpo\_opt\_cosmos & 6 & 100 & 70.834 & 5.075 & 26.200 & 1.395 & 0.116 & 7.600 & 0.465 & 18.575 & 0.151 & 5.015 & 0.803 & 13.796 & 0.904 & 43.300 & 4.000 & 8.329 & 0.887 & -0.000 & 0.488 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 100 & 83.186 & 4.904 & 34.300 & 1.364 & 0.094 & 7.500 & 0.456 & 19.969 & 0.120 & 6.287 & 0.813 & 14.075 & 0.932 & 55.000 & 5.000 & 9.643 & 0.883 & 0.000 & 0.526 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 6 & 100 & 50.005 & 4.843 & 31.600 & 1.325 & 0.099 & 7.800 & 0.453 & 13.036 & 0.097 & 5.071 & 0.803 & 14.099 & 0.901 & 51.400 & 3.500 & 9.253 & 0.783 & 0.000 & 0.442 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 6 & 100 & 65.308 & 4.805 & 30.600 & 1.323 & 0.092 & 7.700 & 0.460 & 15.604 & 0.118 & 4.669 & 0.803 & 14.082 & 0.892 & 49.000 & 4.000 & 9.001 & 0.787 & 0.000 & 0.452 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 6 & 100 & 32.271 & 4.916 & 26.500 & 1.107 & 0.112 & 6.800 & 0.465 & 9.613 & 0.132 & 3.587 & 0.797 & 13.860 & 0.876 & 42.900 & 2.400 & 8.827 & 0.810 & -0.000 & 0.395 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 6 & 100 & 44.409 & 4.943 & 26.300 & 1.127 & 0.078 & 5.100 & 0.486 & 13.444 & 0.080 & 3.534 & 0.805 & 13.817 & 0.888 & 40.100 & 3.700 & 8.228 & 0.743 & 0.000 & 0.368 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 6 & 100 & 33.523 & 4.845 & 27.300 & 1.366 & 0.095 & 6.800 & 0.469 & 9.840 & 0.097 & 3.465 & 0.798 & 13.981 & 0.912 & 45.600 & 3.200 & 8.514 & 0.796 & -0.000 & 0.396 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 6 & 100 & 47.190 & 4.953 & 29.700 & 1.363 & 0.068 & 5.800 & 0.469 & 14.254 & 0.041 & 3.716 & 0.811 & 13.817 & 0.915 & 44.500 & 3.600 & 8.648 & 0.744 & -0.000 & 0.377 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 6 & 100 & 39.052 & 4.974 & 28.800 & 1.394 & 0.075 & 4.800 & 0.483 & 10.276 & 0.092 & 3.918 & 0.805 & 13.917 & 0.858 & 42.800 & 3.900 & 8.832 & 0.723 & 0.000 & 0.387 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 100 & 115.270 & 4.430 & 43.900 & 1.320 & 0.129 & 5.300 & 0.299 & 12.640 & 0.214 & 3.048 & 0.641 & 14.556 & 0.764 & 55.700 & 3.000 & 8.628 & 0.791 & 0.000 & 0.402 \\
mamba-sam-seqlen-2048-original & 6 & 100 & 96.530 & 4.838 & 35.000 & 1.429 & 0.105 & 10.900 & 0.474 & 19.013 & 0.145 & 4.302 & 0.824 & 14.020 & 0.840 & 59.100 & 5.600 & 9.590 & 0.811 & -0.000 & 0.485 \\
opt-sam-orpo-mamba-2048-step448 & 6 & 100 & 100.494 & 4.959 & 38.500 & 1.411 & 0.066 & 8.900 & 0.478 & 21.334 & 0.085 & 4.726 & 0.822 & 13.985 & 0.962 & 60.700 & 6.500 & 8.757 & 0.757 & -0.000 & 0.473 \\
opt-sam-orpo-seqlen-2048-step559 & 6 & 100 & 46.084 & 4.912 & 26.300 & 1.352 & 0.080 & 6.200 & 0.508 & 13.015 & 0.085 & 5.115 & 0.801 & 14.013 & 0.944 & 44.600 & 3.800 & 8.853 & 0.841 & -0.000 & 0.439 \\
opt-sam-seqlen-2048-original & 6 & 100 & 80.222 & 4.861 & 33.200 & 1.384 & 0.071 & 8.000 & 0.465 & 18.112 & 0.086 & 5.115 & 0.808 & 13.923 & 0.838 & 52.600 & 4.700 & 9.464 & 0.822 & 0.000 & 0.452 \\
orpo\_opt\_100M\_2048\_preprocess & 6 & 100 & 40.484 & 4.984 & 30.300 & 1.399 & 0.093 & 5.500 & 0.479 & 12.577 & 0.109 & 3.275 & 0.803 & 13.602 & 0.853 & 41.800 & 3.200 & 8.917 & 0.748 & -0.000 & 0.384 \\
orpo\_opt\_cosmos & 6 & 100 & 47.905 & 5.155 & 25.400 & 1.512 & 0.111 & 6.700 & 0.509 & 13.311 & 0.092 & 3.075 & 0.802 & 13.448 & 0.917 & 38.800 & 2.700 & 7.380 & 0.818 & 0.000 & 0.423 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 100 & 54.634 & 4.965 & 36.800 & 1.382 & 0.069 & 7.800 & 0.467 & 14.747 & 0.067 & 4.560 & 0.824 & 14.039 & 0.888 & 57.200 & 5.100 & 9.444 & 0.759 & -0.000 & 0.426 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 100 & 43.797 & 4.626 & 26.000 & 1.274 & 0.060 & 3.600 & 0.362 & 8.278 & 0.099 & 3.196 & 0.741 & 14.196 & 0.937 & 34.500 & 2.900 & 8.691 & 0.778 & 0.000 & 0.359 \\
babylm-seqlen-opt-1024-warmup-v2 & 6 & 100 & 79.831 & 4.895 & 35.300 & 1.365 & 0.080 & 6.600 & 0.467 & 19.934 & 0.097 & 6.413 & 0.792 & 14.010 & 0.955 & 55.600 & 2.300 & 10.311 & 0.825 & 0.000 & 0.503 \\
babylm-seqlen-opt-4096-warmup-v2 & 6 & 100 & 68.903 & 4.709 & 37.500 & 1.256 & 0.049 & 3.400 & 0.317 & 8.270 & 0.114 & 2.911 & 0.645 & 14.248 & 0.842 & 48.900 & 2.800 & 8.554 & 0.710 & -0.000 & 0.303 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 150 & 57.867 & 5.236 & 53.000 & 1.493 & 0.075 & 7.100 & 0.460 & 18.232 & 0.080 & 5.634 & 0.806 & 13.678 & 0.954 & 75.800 & 4.900 & 8.650 & 0.882 & -0.000 & 0.484 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 6 & 150 & 76.770 & 4.859 & 50.100 & 1.371 & 0.090 & 9.900 & 0.414 & 17.024 & 0.095 & 5.429 & 0.788 & 14.073 & 0.912 & 76.200 & 5.500 & 9.054 & 0.800 & -0.000 & 0.463 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 6 & 150 & 41.940 & 5.048 & 38.500 & 1.427 & 0.088 & 8.200 & 0.438 & 12.654 & 0.090 & 4.002 & 0.806 & 13.829 & 0.918 & 60.700 & 5.000 & 8.728 & 0.723 & 0.000 & 0.427 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 6 & 150 & 40.468 & 5.091 & 37.100 & 0.960 & 0.086 & 8.000 & 0.420 & 12.080 & 0.084 & 3.377 & 0.790 & 13.684 & 0.897 & 62.100 & 4.800 & 8.118 & 0.759 & 0.000 & 0.382 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 6 & 150 & 65.959 & 5.128 & 49.300 & 1.419 & 0.088 & 7.400 & 0.420 & 15.683 & 0.104 & 3.999 & 0.784 & 13.844 & 0.870 & 71.100 & 4.800 & 8.799 & 0.756 & 0.000 & 0.440 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 6 & 150 & 37.495 & 5.011 & 42.800 & 1.397 & 0.092 & 10.200 & 0.429 & 10.758 & 0.107 & 3.888 & 0.789 & 13.915 & 0.902 & 67.300 & 5.300 & 8.373 & 0.835 & 0.000 & 0.456 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 6 & 150 & 44.770 & 5.152 & 46.100 & 1.473 & 0.093 & 7.400 & 0.450 & 14.140 & 0.076 & 4.278 & 0.801 & 13.694 & 0.888 & 66.200 & 5.000 & 8.070 & 0.731 & 0.000 & 0.429 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 6 & 150 & 94.854 & 4.943 & 45.900 & 1.375 & 0.165 & 7.200 & 0.390 & 17.234 & 0.169 & 4.676 & 0.716 & 13.974 & 0.908 & 64.800 & 4.600 & 8.833 & 0.822 & 0.000 & 0.527 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 150 & 152.782 & 4.410 & 67.400 & 1.191 & 0.070 & 4.500 & 0.252 & 12.903 & 0.131 & 3.624 & 0.591 & 14.621 & 0.885 & 78.400 & 5.300 & 9.609 & 0.793 & 0.000 & 0.407 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 6 & 150 & 88.099 & 5.056 & 52.600 & 1.165 & 0.086 & 8.100 & 0.437 & 22.341 & 0.097 & 6.008 & 0.804 & 13.928 & 0.827 & 75.800 & 6.200 & 8.885 & 0.886 & -0.000 & 0.475 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 150 & 46.760 & 4.621 & 44.800 & 1.283 & 0.077 & 4.400 & 0.306 & 8.345 & 0.114 & 3.171 & 0.682 & 14.368 & 0.876 & 58.000 & 4.400 & 8.878 & 0.763 & -0.000 & 0.355 \\
babylm-seqlen-opt-1024-warmup-v2 & 6 & 150 & 70.947 & 5.060 & 43.500 & 1.429 & 0.076 & 7.800 & 0.439 & 17.958 & 0.066 & 4.506 & 0.802 & 13.922 & 0.858 & 66.000 & 4.600 & 8.523 & 0.724 & 0.000 & 0.429 \\
babylm-seqlen-opt-4096-warmup-v2 & 6 & 150 & 143.764 & 4.537 & 76.200 & 1.213 & 0.063 & 4.800 & 0.266 & 14.012 & 0.138 & 3.547 & 0.576 & 14.515 & 0.890 & 89.300 & 3.700 & 8.916 & 0.802 & -0.000 & 0.390 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 6 & 200 & 164.283 & 5.023 & 65.000 & 1.419 & 0.089 & 11.800 & 0.412 & 33.135 & 0.119 & 7.077 & 0.743 & 14.009 & 0.898 & 91.200 & 5.600 & 8.917 & 0.861 & 0.000 & 0.572 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 6 & 200 & 107.791 & 4.785 & 87.200 & 1.297 & 0.122 & 12.900 & 0.363 & 22.308 & 0.147 & 4.927 & 0.718 & 14.186 & 0.776 & 117.700 & 6.500 & 8.964 & 0.821 & 0.000 & 0.506 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 6 & 200 & 114.583 & 4.934 & 63.200 & 1.398 & 0.120 & 9.000 & 0.369 & 22.194 & 0.125 & 5.512 & 0.753 & 13.996 & 0.832 & 88.800 & 6.200 & 9.136 & 0.832 & -0.000 & 0.500 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 6 & 200 & 51.652 & 4.947 & 54.500 & 1.363 & 0.142 & 9.100 & 0.378 & 12.861 & 0.162 & 4.317 & 0.745 & 13.952 & 0.888 & 79.700 & 6.100 & 8.782 & 0.816 & 0.000 & 0.485 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 6 & 200 & 62.904 & 4.964 & 50.500 & 1.372 & 0.090 & 7.600 & 0.411 & 14.895 & 0.091 & 4.313 & 0.765 & 13.857 & 0.889 & 71.100 & 6.700 & 8.708 & 0.782 & 0.000 & 0.461 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 6 & 200 & 40.390 & 5.100 & 51.100 & 1.431 & 0.088 & 13.200 & 0.382 & 10.987 & 0.083 & 3.869 & 0.761 & 13.687 & 0.915 & 77.400 & 5.000 & 8.313 & 0.808 & -0.000 & 0.434 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 200 & 139.700 & 4.510 & 83.900 & 1.267 & 0.084 & 6.300 & 0.244 & 12.946 & 0.140 & 3.770 & 0.590 & 14.449 & 0.809 & 98.300 & 3.700 & 9.394 & 0.811 & 0.000 & 0.424 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 200 & 110.414 & 4.456 & 100.500 & 1.293 & 0.120 & 8.500 & 0.245 & 9.865 & 0.191 & 4.011 & 0.557 & 14.601 & 0.909 & 118.600 & 5.200 & 9.021 & 0.796 & 0.000 & 0.484 \\
babylm-seqlen-opt-1024-warmup-v2 & 6 & 200 & 123.525 & 4.897 & 68.000 & 1.397 & 0.110 & 14.700 & 0.376 & 22.660 & 0.132 & 6.588 & 0.759 & 13.999 & 0.946 & 100.700 & 6.800 & 9.551 & 0.816 & 0.000 & 0.574 \\
babylm-seqlen-opt-4096-warmup-v2 & 6 & 200 & 177.000 & 4.402 & 95.500 & 1.181 & 0.047 & 10.000 & 0.227 & 13.033 & 0.085 & 3.010 & 0.525 & 14.600 & 0.870 & 113.300 & 3.100 & 9.030 & 0.773 & 0.000 & 0.380 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 250 & 162.039 & 4.375 & 113.800 & 1.179 & 0.104 & 9.100 & 0.212 & 13.378 & 0.192 & 4.009 & 0.534 & 14.653 & 0.857 & 132.200 & 3.300 & 9.918 & 0.816 & -0.000 & 0.453 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 6 & 250 & 151.749 & 4.498 & 113.700 & 1.226 & 0.151 & 6.800 & 0.214 & 10.704 & 0.212 & 4.198 & 0.515 & 14.631 & 0.932 & 130.800 & 5.000 & 10.981 & 0.817 & 0.000 & 0.526 \\
babylm-seqlen-opt-4096-warmup-v2 & 6 & 250 & 342.416 & 4.298 & 164.700 & 1.118 & 0.070 & 6.800 & 0.168 & 21.173 & 0.181 & 4.993 & 0.423 & 14.846 & 0.780 & 182.400 & 2.700 & 9.331 & 0.820 & 0.000 & 0.469 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 8 & 50 & 42.823 & 4.917 & 25.600 & 1.346 & 0.058 & 4.300 & 0.523 & 13.036 & 0.054 & 3.717 & 0.851 & 13.877 & 0.893 & 40.100 & 2.800 & 8.185 & 0.818 & 0.000 & 0.398 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 8 & 50 & 39.586 & 4.786 & 15.500 & 1.307 & 0.063 & 3.100 & 0.507 & 10.766 & 0.067 & 3.147 & 0.831 & 14.022 & 0.894 & 27.500 & 3.000 & 9.427 & 0.715 & -0.000 & 0.357 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 8 & 50 & 39.688 & 5.018 & 19.100 & 1.400 & 0.063 & 4.300 & 0.524 & 11.439 & 0.069 & 3.404 & 0.843 & 13.855 & 0.881 & 30.600 & 2.700 & 8.512 & 0.766 & 0.000 & 0.379 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 8 & 50 & 37.096 & 4.790 & 17.400 & 1.324 & 0.066 & 5.000 & 0.489 & 10.125 & 0.091 & 3.265 & 0.827 & 14.087 & 0.842 & 30.500 & 2.400 & 9.141 & 0.725 & -0.000 & 0.349 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 8 & 50 & 40.788 & 4.858 & 20.000 & 1.346 & 0.075 & 5.800 & 0.510 & 11.094 & 0.071 & 3.509 & 0.835 & 14.080 & 0.885 & 34.000 & 2.900 & 8.717 & 0.788 & 0.000 & 0.397 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 8 & 50 & 38.565 & 4.874 & 17.900 & 1.345 & 0.070 & 4.100 & 0.500 & 11.086 & 0.090 & 3.297 & 0.835 & 13.990 & 0.948 & 29.700 & 2.200 & 8.792 & 0.789 & 0.000 & 0.394 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 8 & 50 & 50.151 & 4.889 & 18.400 & 1.355 & 0.070 & 4.500 & 0.519 & 13.028 & 0.072 & 3.610 & 0.824 & 13.963 & 0.856 & 29.700 & 2.800 & 8.579 & 0.767 & 0.000 & 0.378 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 8 & 50 & 33.195 & 4.868 & 19.500 & 1.337 & 0.059 & 4.100 & 0.508 & 9.969 & 0.059 & 2.917 & 0.831 & 13.919 & 0.850 & 30.200 & 2.900 & 8.428 & 0.723 & 0.000 & 0.352 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 50 & 64.514 & 4.495 & 22.300 & 1.193 & 0.073 & 3.500 & 0.363 & 9.533 & 0.133 & 3.866 & 0.738 & 14.479 & 0.941 & 31.100 & 2.000 & 9.187 & 0.745 & 0.000 & 0.376 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 8 & 50 & 49.000 & 4.958 & 25.000 & 1.359 & 0.076 & 6.100 & 0.511 & 13.795 & 0.072 & 4.322 & 0.852 & 13.990 & 0.930 & 40.000 & 3.800 & 9.058 & 0.807 & 0.000 & 0.463 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 50 & 65.527 & 4.437 & 24.900 & 1.186 & 0.059 & 4.000 & 0.359 & 9.285 & 0.092 & 3.188 & 0.723 & 14.447 & 0.858 & 32.700 & 4.500 & 8.461 & 0.701 & 0.000 & 0.319 \\
babylm-seqlen-opt-1024-warmup-v2 & 8 & 50 & 53.219 & 4.845 & 20.900 & 1.344 & 0.063 & 3.700 & 0.504 & 13.762 & 0.067 & 3.845 & 0.832 & 13.982 & 0.937 & 33.400 & 3.000 & 9.526 & 0.782 & 0.000 & 0.410 \\
babylm-seqlen-opt-4096-warmup-v2 & 8 & 50 & 75.174 & 4.458 & 29.900 & 1.170 & 0.036 & 3.300 & 0.337 & 9.767 & 0.114 & 3.604 & 0.686 & 14.552 & 0.897 & 38.300 & 1.300 & 8.458 & 0.663 & 0.000 & 0.304 \\
cpo\_opt\_seqlen\_1024\_final\_checkpoint & 8 & 100 & 78.090 & 4.956 & 44.300 & 1.406 & 0.113 & 8.500 & 0.421 & 18.996 & 0.128 & 5.192 & 0.793 & 13.975 & 0.953 & 69.300 & 4.300 & 8.717 & 0.882 & 0.000 & 0.520 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration1 & 8 & 100 & 91.858 & 4.938 & 44.100 & 1.389 & 0.081 & 8.500 & 0.436 & 21.904 & 0.065 & 5.228 & 0.784 & 13.959 & 0.863 & 69.200 & 4.700 & 8.739 & 0.780 & 0.000 & 0.462 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration2 & 8 & 100 & 53.447 & 4.954 & 43.200 & 1.402 & 0.083 & 7.000 & 0.435 & 14.739 & 0.104 & 4.041 & 0.799 & 13.887 & 0.898 & 63.500 & 5.600 & 8.987 & 0.758 & -0.000 & 0.415 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration3 & 8 & 100 & 52.003 & 5.062 & 40.400 & 1.417 & 0.090 & 9.300 & 0.440 & 14.185 & 0.090 & 3.883 & 0.793 & 13.795 & 0.917 & 63.100 & 4.400 & 8.401 & 0.739 & -0.000 & 0.424 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration4 & 8 & 100 & 102.745 & 4.939 & 38.000 & 1.116 & 0.102 & 8.400 & 0.437 & 23.938 & 0.111 & 5.030 & 0.802 & 13.850 & 0.893 & 60.400 & 5.300 & 8.821 & 0.862 & 0.000 & 0.481 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_parlai\_iteration5 & 8 & 100 & 51.006 & 5.110 & 36.900 & 1.419 & 0.084 & 6.100 & 0.431 & 13.309 & 0.075 & 3.807 & 0.748 & 13.767 & 0.930 & 55.600 & 4.000 & 7.904 & 0.844 & 0.000 & 0.420 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration4 & 8 & 100 & 38.790 & 5.052 & 38.800 & 1.159 & 0.085 & 6.700 & 0.448 & 11.696 & 0.099 & 3.619 & 0.798 & 13.896 & 0.940 & 56.200 & 5.600 & 8.342 & 0.755 & 0.000 & 0.435 \\
cpo\_opt\_seqlen\_1024\_progressive\_cefr\_reverse\_parlai\_iteration5 & 8 & 100 & 73.983 & 4.903 & 36.900 & 1.104 & 0.108 & 9.300 & 0.431 & 17.744 & 0.099 & 4.188 & 0.779 & 14.020 & 0.879 & 58.300 & 4.400 & 9.010 & 0.794 & 0.000 & 0.438 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 100 & 101.535 & 4.493 & 72.500 & 1.187 & 0.073 & 8.800 & 0.273 & 10.498 & 0.125 & 3.883 & 0.651 & 14.545 & 0.832 & 89.500 & 4.300 & 9.361 & 0.808 & -0.000 & 0.390 \\
orpo\_opt\_seqlen\_1024\_final\_checkpoint & 8 & 100 & 60.045 & 5.052 & 49.500 & 1.424 & 0.072 & 8.800 & 0.443 & 17.114 & 0.078 & 4.587 & 0.805 & 13.865 & 0.957 & 74.700 & 5.800 & 8.705 & 0.847 & 0.000 & 0.493 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 100 & 82.047 & 4.482 & 38.200 & 1.315 & 0.120 & 5.300 & 0.294 & 10.086 & 0.120 & 3.348 & 0.665 & 14.341 & 0.903 & 51.900 & 4.100 & 8.326 & 0.807 & -0.000 & 0.361 \\
babylm-seqlen-opt-1024-warmup-v2 & 8 & 100 & 96.315 & 5.002 & 40.000 & 1.432 & 0.084 & 6.000 & 0.447 & 23.534 & 0.094 & 4.797 & 0.795 & 13.771 & 0.829 & 59.200 & 4.600 & 8.566 & 0.799 & 0.000 & 0.443 \\
babylm-seqlen-opt-4096-warmup-v2 & 8 & 100 & 105.409 & 4.485 & 56.200 & 1.215 & 0.066 & 4.900 & 0.279 & 11.872 & 0.109 & 3.486 & 0.612 & 14.543 & 0.914 & 70.000 & 2.900 & 8.584 & 0.766 & -0.000 & 0.357 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 150 & 232.080 & 4.408 & 101.300 & 1.170 & 0.068 & 7.000 & 0.201 & 16.174 & 0.128 & 4.299 & 0.501 & 14.769 & 0.900 & 115.300 & 3.100 & 9.759 & 0.798 & 0.000 & 0.442 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 150 & 100.032 & 4.481 & 69.700 & 1.202 & 0.070 & 8.800 & 0.248 & 9.962 & 0.141 & 3.936 & 0.610 & 14.511 & 0.890 & 85.200 & 3.000 & 8.217 & 0.825 & 0.000 & 0.393 \\
babylm-seqlen-opt-4096-warmup-v2 & 8 & 150 & 115.660 & 4.505 & 85.600 & 1.218 & 0.036 & 5.100 & 0.251 & 11.382 & 0.133 & 2.960 & 0.589 & 14.418 & 0.856 & 100.000 & 2.500 & 8.419 & 0.828 & -0.000 & 0.341 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 200 & 185.814 & 4.366 & 178.900 & 1.223 & 0.109 & 10.300 & 0.196 & 15.133 & 0.194 & 3.201 & 0.530 & 14.614 & 0.934 & 198.200 & 4.000 & 9.354 & 0.851 & -0.000 & 0.495 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 200 & 88.959 & 4.663 & 92.100 & 1.284 & 0.107 & 11.200 & 0.247 & 10.933 & 0.142 & 3.371 & 0.626 & 14.316 & 0.830 & 113.100 & 5.400 & 8.748 & 0.794 & 0.000 & 0.429 \\
babylm-seqlen-opt-4096-warmup-v2 & 8 & 200 & 219.890 & 4.446 & 136.700 & 1.166 & 0.114 & 5.400 & 0.183 & 15.693 & 0.154 & 3.967 & 0.453 & 14.739 & 0.841 & 154.400 & 3.300 & 8.978 & 0.781 & 0.000 & 0.434 \\
cpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 250 & 355.466 & 4.366 & 221.700 & 1.207 & 0.129 & 8.900 & 0.159 & 22.153 & 0.182 & 5.127 & 0.442 & 14.780 & 0.838 & 245.300 & 5.200 & 9.399 & 0.865 & 0.000 & 0.571 \\
orpo\_opt\_seqlen\_4096\_final\_checkpoint & 8 & 250 & 245.333 & 4.434 & 232.200 & 1.283 & 0.141 & 11.400 & 0.181 & 15.772 & 0.188 & 4.189 & 0.485 & 14.648 & 0.938 & 254.000 & 5.700 & 9.094 & 0.863 & 0.000 & 0.605 \\
babylm-seqlen-opt-4096-warmup-v2 & 8 & 250 & 260.688 & 4.531 & 141.000 & 1.193 & 0.063 & 10.700 & 0.171 & 19.532 & 0.112 & 7.334 & 0.426 & 14.737 & 0.715 & 162.200 & 4.800 & 8.916 & 0.751 & -0.000 & 0.418 \\
\bottomrule
\end{tabular}
\caption{Average metrics per BabyLM setting with min--max normalized aggregate (NormAvg) across metrics.}
\label{tab:dialogue-metrics}
\end{table*}

